Tree exploration in dual-memory model

We study the problem of online tree exploration by a deterministic mobile agent. Our main objective is to establish what features of the model of the mobile agent and the environment allow linear exploration time. We study agents that, upon entering to a node, do not receive as input the edge via which they entered. In such a model, deterministic memoryless exploration is infeasible, hence the agent needs to be allowed to use some memory. The memory can be located at the agent or at each node. The existing lower bounds show that if the memory is either only at the agent or only at the nodes, then the exploration needs superlinear time. We show that tree exploration in dual-memory model, with constant memory at the agent and logarithmic at each node is possible in linear time when one of two additional features is present: fixed initial state of the memory at each node (so called clean memory) or a single movable token. We present two algorithms working in linear time for arbitrary trees in these two models. On the other hand, in our lower bound we show that if the agent has a single bit of memory and one bit is present at each node, then exploration may require quadratic time on paths, if the initial memory at nodes could be set arbitrarily (so called dirty memory). This shows that having clean node memory or a token allows linear exploration of trees in the model with two types of memory, but having neither of those features may lead to quadratic exploration time even on a simple path.

==> sections/00-abstract.tex <==
We consider the following problem -- ...
The abstract should briefly summarize the contents of the paper in
150--250 words.



==> sections/10-intro.tex <==
\section{Introduction}\label{sec:intro}

In this paper we investigate ...

\subsubsection*{Organization of the Paper.}
In Section \ref{sec:model} we describe the problem and the formal model. An overview of the most important related work is mentioned in Sect. \ref{sec:relatedWork}.
... We conclude in Sect. \ref{sec:conclusion}.

      




==> sections/20-model.tex <==
% !TEX root = ../asyncExploration.tex
\section{Model}
\label{sec:model}

\subsubsection*{The Agents in the Network.}
We model the network as a simple, undirected, connected graph $G(V,E)$ with $n$ vertices, $m$ edges and diameter $D$.
The nodes of the graph are uniquely labelled with numbers $\{1,2,\dots,n\}$.
We have also $k\geq 1$, $k \ll n$ agents representing mobile devices, where the value of $k$ may or may not be \mk{Istotne, ze nie wiedza gdzie sa ...}
Agents know the topology of $G$ and their objective is to explore jointly every node of $G$ with the least possible complexity measure.
\mk{Trzeba by juz tu okreslic jakie measures ...}
We may model it as follows:
Every node has its exploration flag, initially set to $0$. Every agent starts at some node, which flag is automatically set to $1$. At every moment the agent decides how to make a next step across one of the edges connected to his actual position. 
\mk{Istotne, ze nie wiedza gdzie sa w grafie ...}
When he crosses the link, he automatically checks, if the exploration flag of a destination point is set to $1$, and if it is not, then it is changed automatically to $1$. Every agent is aware of a presence of other agents in his actual position and may know which edges all of these agents used (he knows where they came from and where they went to). When agents meet in some vertex, they may eventually compare theirs information. Otherwise, agents cannot communicate. An agent may change his destination, when some agents go in or outside his position. Moreover vertex' flag may be saved in the particular node and read automatically by 
\mk{Nie bardzo rozumiem. Poza tym raz mowimy o flag, raz o pebbles, raz o bitach ...}
The exploration of the network is done when all exploration flags are set to $1$ and it is terminated automatically then.

Depending on a model, agents may or may not use the information from different types of oracles:
\begin{itemize}
\item[geometric oracle] shows directions of adjacent vertices or directions of positions of other agents.
\item[own position] shows agent's actual position in the network.
\item[all positions] shows positions of all agents in the network.
\item[online] agents may request oracle at any time.
\item[offline] agents only request oracle at start of an algorithm.
\end{itemize}
\mk{Tutaj chyba byloby rozsadniej opisac to jako taksonomie roznych modeli. Poza tym te kategorie nie sa rozlaczne. }
%Time is divided into synchronous rounds. At the beginning of
%each round each agent is located in a single vertex. In each round the agent can change its position to any of
%neighboring vertices.  We allow many agents to be in a single vertex in the same round. The agents need to locally
%distinguish the edges in order to navigate in the graph hence we assume that the edges outgoing from a node with degree
%$d$ are uniquely labeled with numbers $\{1,2,\dots,d\}$. We assume no correlation between the labels on two endpoints of
%any node. A graph with such a labeling is sometimes called {\em port-labeled}.
%
%When an agent is located in a vertex we assume that it has access to the degree of the node and possibly the value or
%the estimate of $n$ and to some internal memory sufficient for local computations it performs.
%In our paper we consider various models of mobile agents depending on the resources at their disposal. This will involve 
%settings where the devices have or have not an access to a source of random bits and they are given a priori the topology
%of the network or they have no such knowledge. In the latter case we will consider two different scenarios depending on
%whether the agent has an access to operational memory that remains intact when it traverses an edge or its memory is very
%limited and does not allow to store any information about the network gathered while it moves from one vertex to another. 
%
%Our primary motivation is the problem of physical hiding of mobile devices performing tasks in some terrain.
%Nevertheless, our work aims for formalizing the problem of losing information on agents' initial placement
%in a given network. Thus, we focus on proposing a theoretical model related to the logical topology.

\subsubsection*{Model of the Adversary.}
%We consider various models of the adversary...
An adversary has full information about the network, actual agents positions and decisions and a type of exploited oracle.\db{tutaj nie jestem pewien, czy nie ma innych opcji}
The adversary can choose the initial positions of all agents and make some part of agents temporarily idle (but never all of them)
\mk{nieprecyzyjnie }
during the exploration process. Every idle agent stays still and does not change his decision until the local situation of this agent does not change (no other agent moves in or out his position), whilst the rest of them move as they decided previously. Agents have no sense of time, but he is awared of chronology (especially, when he is idle, then he is able to order the situations that take place in the vertex he is actually in).\db{sa achronometryczni?} 
Although the process of exploration is asynchronous, we may easily interpret it in a synchronous rounds arrangement. Indeed, we may assume that every move takes one round (we assume that either all moves are instant)\db{inaczej to stwarza problemy, ze ktos ktos moze byc wstrzymywany do polowy ruchu ktoregos z agentow, co moze dac dodatkowa sile adwersarzowi} 
and if an agent does not make any move, then it is idle during this round, but he is not aware of this.
A goal of the adversary is to maximally increase the value of complexity measure of the exploration.
\mk{wazne ze NIE zna bitow losowych lokalnie wygenerowanych przez stacje  }
%From the adversary's point of view, the agents are indistinguishable and the nodes of the underlying graph are labeled.
%The assumption on indistinguishability is adequate for systems with very similar devices. 
%Thus the state of the system in a given round $t$ can be seen as a graph $G$ and a function $n_t(v)$ denoting the number
%of agents located at node $v$.
%Let $X_t$, $t \in \{ 0,1, \ldots \}$, represents the state of the network at the beginning of $t^{\mathrm{th}}$ round.
%
%We assume that in round $0$ the agents complete (or interrupt due to approaching adversary) their actual tasks and run
%{\em hiding algorithm} $\AAA$ that takes $T$ rounds. Just after the round $T$ the adversary is given  the final state $X_T$ and, 
%roughly speaking, its aim is to learn as much as possible about the initial state $X_0$. That is, the adversary gets an access to 
%a single configuration (representing a single view of the system). 
%Note that the adversary may have some {\em a priori} knowledge that is modeled as a distribution
%of $X_0$. In randomized settings the adversary has no information about agents'
%local random number generators. On the
%other hand, the aim of agents is to make learning  the adversary $X_0$ from $X_T$ impossible  for {\bfseries any}
%initial state (or distributions of states).\footnote{That is, we consider the worst case scenario implying
%strongest security guarantees.} Moreover the number of rounds $T$ should be as small as possible (we need to hide the
%location quickly). We also consider {\em energy complexity} understood as the maximal number of moves (i.e. moving to
%a neighboring vertex) over all agents in the execution of $\AAA$. Such definition follows from the fact that we need to
%have all agents working and consequently we need to protect the most loaded agent against running out of batteries.
%As we shall see, in all cases considered in this paper the energy complexity is very closely related to the time of
%getting to the ``safe'' configuration by all devices, namely it is asymptotically equal $T$.

\subsubsection*{Measures of the algorithm's complexity.}\db{czy sa jakies inne miary w tym przypadku?}
We will evaluate the efficiency of constructed protocols for asynchronous graph exploration in terms of total work performed by all devices in the network.
Thus, the {\em energy complexity} of the algorithms will be defined as the total number of moves over all agents during the execution of the protocol.
We will be also interested in {\em energy complexity per node}. Realize that concerning the {\em maximal energy complexity} over all agents is ponitless, becasue adversary may stop all agents excluding one of them.

%By a single move of an agent we mean traversing an edge between two neighboring vertices.

Realize that the state of an agent $a$ may be described by $(t,V,v,A)$, where $t$ is the number of moves that $a$ did, $V$ is a set of vertices of the network that $a$ visited or he knows that the other agents have visited, $v$ is an actual position of $a$ and $A$ is an additional information given by the observation and communication with other agents like port the specific agent came from and eventually went to and in what order (the other agent may came to went out and back again). 
\mk{Co to jest $A$? W jaki posob sie odbywa ta communication? Czy to co wie agent to po prostu graf indukowany przez te odwiedzone? Etykiety na krawedziach ...}
In case of the online oracle we may introduce additional cost of a request.
\mk{Swoja droga trzeba tez jasno opisac jak wyglada ten asynchronizm, szczegolnie co sie dzieje jak dwa agenty wchodza do tego samego wierzcholka jednoczesnie }
\mk{Kolejna sprawa: czy maja swoje unikalne ID? Czy możemy zrobic tak by jeden szedl w prawo, drui w lewo? Czy protokol jest symetryczny, t.j. czy wszystkie agenty wykonuja ten sam kod?}

==> sections/30-related.tex <==
% !TEX root = ../asyncExploration.tex
\section{Previous and Related Work}
\label{sec:relatedWork}

The problem of graph exploration by a set of agents is one of the classical problems in distributed computing.
In the vast body of literature various models and scenarios have been extensively discussed and a lot of efficient
algorithms have been proposed over the past decades...[In particular there exist polynomial
deterministic algorithms (using Universal Sequences) that need only logarithmic memory~\cite{AleliunasKLLR79,Reingold08}.]
...
A thorough survey on algorithmic aspects of distributed computing by mobile agents and robots, including a comprehensive overview
of common formal models and the state-of-the-art algorithms for many classical problems like graph exploration,
gathering and patrolling can be found in \cite{Flocchini:2019:DistCompSurv}.
\mk{Mysle, ze tu bardzo zgrubny szkielet Previous Work - jakie tematy moglby zaproponowac Dominik lub Darek, a reszte wypelnimy my }

==> sections/40-alg.tex <==
\section{Algorithms for asynchronous graph exploration}
\label{sec:alg}

In this section we present and analyze distributed algorithms for asynchronous graph exploration in the presence of an adversary
for a wide range of scenarios, including the settings where...


==> sections/41-circle2.tex <==
% !TEX root = ../asyncExploration.tex

\subsection{Two agents on a circle}
\label{sec:alg:2circle}

We will analyze in details the task of asynchronous exploration of a circle by two agents. This will serve as a simple introductory 
example for our further discussion, showing various aspects of the problem studied in this paper for different settings.
\mk{}
Let us consider the following simple scenario. There are two agents, say $a_1$ and $a_2$ located in some two vertices $v_1$ and $v_2$
(not necessarily distinct) on a circle of size $n$, i.e. a simple undirected graph $C_n = (V, E)$ with $n$ vertices $V = \{0,\dotsc,n-1\}$
and the set of edges $E = \{\{(i, i + 1) \mod n\} \colon i \in V \}$. Each active agent $a_i$ (i.e. not suspended by the adversary), $i \in \{1,2\}$, 
located in some vertex $v \in V$, in a single step can move along an edge incident to $v$ either to $(v+1) \mod n$ or to $(v-1) \mod n$. After entering
some vertex $v$, which has not been visited yet, an agent puts a pebble on $v$ marking it as explored (the vertices $v_1$ and $v_2$, i.e. the agents'
initial positions, are pebbled at the beginning of the algorithm). For the sake or brevity, in our discussion we will use the following simplified notation.
For $v \in V = \{0,\dotsc,n-1\}$ and $x \in ZZ$, by $u + x$ we will denote a vertex $v \in V$ such that $v = (u + x) \mod n$ (in other words,
$+$ and $-$ will denote the operations modulo $n$ on the set of vertices). 

The goal of the protocol is to explore the whole graph $C_n$ by the agents, so that each vertex in $V$ will be pebbled. This means that each of the
vertices has to be visited at least once by some agent. We will assume that the algorithm terminates immediately after pebbling all vertices and its
cost (i.e. algorithm's energetic complexity) is the total number of moves performed by all agents in the graph during the execution of the protocol.

Given the set of agents $A$, the adversary $\AAA$ controls them by arbitrarily choosing the subset of agents which are active in a given time instant.
In other words, at any moment only the agents not suspended by $\AAA$ can move to another vertex. All remaining agents become idle and stay in their
current positions (we may assume e.g. that each agent has one control bit governed solely by $\AAA$). The only requirement is that at least one agent has to be
active in every time instant (the slots in which all agents are inactive have no impact on the overall cost of the algorithm, so we may ignore them).
In this example we will consider an adaptive adversary which knows both the protocols executed by devices and their state (including their current positions and
access to their memory). We also assume that the adversary has knowledge of all random choices made by the agents. Based on all these observations the adversary
can adaptively make choices about his strategy (which agents are active in next slots).

Fix an agent $a \in A$. The set of vertices visited by $a$ during the execution of the algorithm always induces a connected subgraph of the original graph
(in this example $C_n$). Hence, we may split the set $V$ of vertices into four subsets $C_1$, $C_2$, $U_1$, $U_2$, where $C_i$ is the
set covered by $a_i$, $i \in \{1,2\}$, and $U_1$, $U_2$ consist of not yet visited vertices. More precisely, letting $v_{1}^{m} = \min\{C_1\}$, $v_{1}^{M} = \max\{C_1\}$,
$v_{2}^{m} = \min\{C_2\}$, $v_{2}^{M} = \max\{C_2\}$ we define $U_1 = \{v_{1}^{M} + 1, v_{1}^{M} + 2, \dotsc, v_{2}^{m} - 1\}$
and $U_1 = \{v_{2}^{M} + 1, v_{2}^{M} + 2, \dotsc, v_{1}^{m} - 1\}$. Obviously $C_1$ and $C_2$ are nonempty, whereas $U_1$ and $U_2$ may be empty.

\paragraph{Deterministic algorithm.}
Suppose that the agents know the topology of the network described by a circle graph $C_n$ with $n$ vertices, but they do not necessarily know its size $n$.
Then, asynchronous exploration of $C_n$ by two agents can be done deterministically in at most $2n$ steps regardless of their initial positions. The following
simple procedure executed by each of the agents allows for achieving this.\kg{lepiej zapisac ten alg.} In the beginning the agents choose the outgoing edge with 
the smallest index. Then, upon entering a vertex $v$ through a port $p$, the agent marks $v$ as visited and moves to the next vertex using the other port
(we assume that agents can distinguish between the edges outgoing from a given vertex).\kg{wspomniec o port-labelled graphs} It is clear that if a single agent
will preform $n-1$ steps, then all vertices will be marked as visited and the protocol will terminate. Hence, since at least one agent must be active in every
time instant, the worst case scenario for this simple protocol (with respect to the total amount of energy used by the agents) is when both agents are initially
located in the same vertex $v^{*}$ and the adversary lets them both to be active. As we can easily see, in this scenario each agent will make $n-1$ moves until
all vertices will be pebbled at least once, thus leading to the energetic complexity $2(n-1)$. The same cost is when the adversary will block them alternately,
but they will eventually meet up in some vertex $v'$ before one of them will reach $v^{*} - 1$.
\mk{nie jest jasne, kiedy konczy sie algorytm. zadsadniczo nikt nie musi wiedzuec, ze wszystkie stacje sa odwiedzone}


\paragraph{Algorithm with an advice.}
Observe that the worst-case cost of the previous simple algorithm of $2(n-1)$ is partially due to the fact, that the agents are unaware of each other's initial
positions and traverse the graph ``independently'', taking no advantage from the information if some vertices have already been explored. Let us assume now that
at the beginning the agent $a_i$, $i \in \{1,2\}$ is given an one bit $b_i$ of information about the starting position of the other agent. This advice
tells $a_i$ in which direction (clockwise or counterclockwise) it should go, to reach the vertex in which $a_2$ was located initially in fewer steps (in other words,
which port should it choose in the first step). More formally, let $v_i$ be the starting position of $a_i$, $\tilde{i} = 3-i$ (i.e. for $i=1$, $\tilde{i} = 2$,
and conversely)\kg{ta uwage wywalic} and denote by $d = d(v_1,v_2)$ the distance between $v_1$ and $v_2$ in $C_n$, i.e. the number of edges on a shortest path between
$v_1$ and $v_2$. Then, $b_i = 0$ means that $v_{\tilde{i}} = v_i + d$, otherwise $v_{\tilde{i}} = v_i - d$. In case of a tie, i.e. when $v_i + d = v_i - d$, we put e.g. $b_1 = 0$,
$b_2 = 1$. Having this information, we may modify the first step of the simple deterministic procedure for asynchronous exploration of $C_n$ from previous paragraph
by letting the agents make the first move according the advice. It is easy to see, that the worst-case energetic complexity of such modified procedure is $1.5 n + \BigO{\frac{1}{n}}$
\mk{nie bardzo rozumim skad sie $\BigO{\frac{1}{n}}$ wzielo ...}.
Indeed, assume wlog that $v_2 = v_1 + d$. Then, the set of vertices $V$ can be partitioned into $V_1 = \{v_1, v_1 + 1, \dotsc, v_2\}$ and $V_2 = \{v_2 + 1, v_2 + 2, \dotsc, v_1 - 1\}$.
Observe that the vertices in $V_1$ may be explored by both agents, whereas $V_2$ consists of vertices visited only once. Since $d \leq \frac{n}{2}$, we have
$|V_1| \leq \frac{n}{2} + 1$ and the upper bounds on the total cost follows.

There is also another variant of the procedure, for which the total number of agents' moves in worst case is $1.5 n + \BigO{1}$. The only difference is that if an agent
will enter some vertex which was already pebbled (or the devices meet up in some common vertex), it will ``turn back'', changing the direction, in which it traverses the edges of $C_n$.
Again, regardless of the adversary's strategy, at most $\frac{n}{2} + 1$ vertices will be explored more than once (it can happen, that two vertices will be visited three times
in this algorithm, if the agents pass each other while traversing some edge), thus leading to the same upper bound on the energetic complexity.

\paragraph{Guessing the advice.}
If the agents are not given such one-bit advice, but they have an access to some source of randomly generated, independent uniform bits, they may try to ``guess'' the advice
by independently letting $b_i$ to be $0$ or $1$ with equal probability. The devices will then execute the variant of the algorithm, in which they change the direction
of exploration after entering some already pebbled vertex. Suppose that $d(v_1,v_2) = d$. If the bits $b_i$ were ``guessed correctly'' (i.e. they have the same values as in the algorithm
with an advice from previous paragraph), then the worst-case energetic complexity is $n + d + \BigO{1}$. This will happen with probability $\frac{1}{4}$.
In all remaining cases the adversary can choose his strategy so that the agents will perform $2(n-d) + d + \BigO{1}$\kg{uporzadkowac to O(1) - tam siedzi cos typu +/- 1} moves in total. 
If $b_1 = b_2$ (the agents move in the same direction), then  in order to reach the initial position of the other agent, one of them (say, $a_i$) needs to make $d$ steps,
and the second one (say, $a_{\tilde{i}}$) -- $n-d$ steps. The adversary can then block $a_i$ so that $a_{\tilde{i}}$ will traverse the longer path (of length $n-d$) twice.
Otherwise, if $b_1 \neq b_2$, then each agent will encounter the vertices visited by the other one somewhere on the longer path between $v_1$ and $v_2$. Thus, the set of
vertices explored by both agents will be of size $n - d + \BigO{1}$. Hence, the total energetic expenditure is on average 
$$ \frac{1}{4} \left(n + d + \BigO{1} \right) + \frac{3}{4} \left(2(n - d) + d + \BigO{1} \right) = \frac{7n}{4} - \frac{d}{2} + \BigO{1}~,$$
where $0 \leq d \leq \frac{n}{2}$. From this we conclude, that the expected energetic complexity of the considered randomized algorithm for the worst-case choice of agents'
initial positions is $1.75 n + \BigO{1}$.

\paragraph{Lower bound for deterministic protocols.}
As we shall see, if there is no additional information available to the agents at the beginning of the procedure, then the total energetic expenditure of both agents
in any deterministic algorithm for asynchronous graph exploration will be at least $2(n-1)$ in worst case. Suppose, that the agents cannot distinguish the directions (clockwise,
counterclockwise) in which they should go, to reach the other's agent initial position in fewer steps. Then, ...
...\kg{TODO: spisac dowod DP}


==> sections/90-conclusion.tex <==
\section{Conclusions and Further Research}\label{sec:conclusion}
In the paper we considered the problem of asynchronous graph exploration by a set of mobile agents in the adversarial setting.
We discussed various scenarios depending on ..., proposed some efficient algorithms and provided lower bounds for []some of the
considered settings]...








==> sections/app_line.tex <==
\section{Missing proofs from Section~\ref{sec:line}}
\label{app_line}
In the following series of facts we will prove some properties that $\mathcal{A}$ has to satisfy. 
%dwa pierwsze fakty przeniesione do glownej czesci
\begin{lem}
\label{lem:vconst}
Fix any $a \in \As$ and $v\in \Vs$. Algorithm $\mathcal{A}$ does \textbf{not} satisfy the following condition:
\[
%(\forall\;a,x\in \As)(\forall\;v,y,z\in Vs)\;R_2(a,v)=(a',v) \land R_2(a',v)=(x,y)\land R_2(a',v')=(x,z).
R_2(a,v)=(a',v) \land A(a',v) = A(a',v')~.
\]
%Then the adversary can initialize the algorithm in such the way, to either produce infinite loop either reduce the algorithm to RR.
\end{lem}
\begin{proof}
%CASE 3. 
Assume that the formula holds for some $a \in \As$ and $v\in \Vs$ and we will show that in such a case $\mathcal{A}$ would fall into an infinite loop for some initializations of the path. 
From Fact \ref{wn1}, we obtain, that $A(a',v) = A(a',v') = a$. Denote $P(a,v)=p$ and $V(a',v)= y$.
%CASE 3.1. 

If $y=v$, then let $P(a',v)=p'$, and the following initial state of the path results in an infinite loop: 
%$\underline{(a,v)}\stackrel{p\;q}{\leftrightarrow}(a',v)$ 
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (Y);
  \path	 (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\end{center}

%so only two vertices will be visited.\\
%CASE 3.2. 
In the opposite case, where $y = v'$, the agent would fall into an infinite loop on the following gadget:
%$$
%(a,v)\stackrel{p\;p}{\leftrightarrow}(a',v')\stackrel{p'\;p}{\leftrightarrow}(a,v)~,
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v'$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (3,0) {$v$};
  \node (Y) at (4,0) { };
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (Z)
		(Z) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\end{center}

%which leads to infinite loop.\\
Indeed, $R_3(a,v) = (a',v,p)$, hence in the first step, the agent moves to the middle vertex, changes its state to $a'$, and keeps $v$ as the state of the first vertex.
At the middle vertex when the agent state is $a'$, then it always changes its state to $a$ and moves to one of the outer vertices (independent on the vertex state of the middle node). But since the outer vertices are both in state $v$, the agent returns to the middle vertex, and so on, which is an infinite loop.
%and, hence we always return to the middle vertex from the entering state $(a,v)$, hence the outer vertices' states won't change as well, so we never visit any of the positions excluding these 3.
\end{proof}

The following fact characterises features of an algorithm, in which some state $a$ of the agent is flipped for both states of a vertex.
\begin{fact}
\label{wn3}
Fix any $a\in\As$. %\marginpar{DB: Wybieramy dowolne a. Ale obydwa fakty dotycza tego samego a; Innymi s³owy: jak pewne a spe³nia warunek ifa, to zachodza dla niego te dwie wlasnosci. Jesli a' tez spelnia analogiczny warunek z ifa, to dla niego tez beda zachodzily analogiczne wlasnosci z primami przy stanach agentow; To wynika z Lematu 1. dla $a'=a$, $x=a'$, raz przy $v=v$, a raz przy $v=v'$.} 
If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then:
%$(\forall\; w\in \Vs)\; R_2(a',w)\neq(a,w)$ and moreover, from Fact \ref{wn2}, then 
%$(\forall\; w\in \Vs)\; V(a',w)=w'$.
\begin{enumerate}[label=\roman*.,ref=\roman*.]
\item\label{fct:31} $(\forall\; w\in \Vs)\; R_2(a',w)\neq(a,w)$,
\item\label{fct:32} $(\forall\; w\in \Vs)\; V(a',w)=w'$,
\item\label{fct:33} $(\exists\; w\in \Vs)\; R_2(a',w)=(a,w')$.
\end{enumerate}
\end{fact}
\begin{proof}
For each $w\in\Vs$, Claim~\ref{fct:31} follows from Lemma~\ref{lem:vconst} for $a', w$.
Claim~\ref{fct:32} follows from Fact~\ref{wn2} and Claim~\ref{fct:31}.
Claim~\ref{fct:33} follows from Fact~\ref{wn1} and Claims~\ref{fct:31},~\ref{fct:32}.
\end{proof}
%\marginpar{DB: dlatego moze wartop rozbic to na 2 fakty}
%\begin{fact}
%\label{wn4}
%Fix any $a\in\As$. If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then, from facts \ref{wn1} and \ref{wn3}, 
%$(\exists\; w\in \Vs)\; R_2(a',w)=(a,w')$.
%\marginpar{DB: tutaj mogloby byc z faktu 3. tylko $R_2(a',w)=(a,w')$ albo $R_2(a',w)=(a',w')$, ale z faktu 1. musi choc raz zmieniac stan agenta.}
%\end{fact}
\begin{fact}
\label{fac:CASE4}
%CASE 4\dpa{CASE 4 -- to jest do któregoœ z faktów?}. 
%Assume that for some $v$, $R_3(a,v)=(a',v,p)$ and $R_3(a',v)=(a,v,q)$. Then $(a',v)\stackrel{q\;p}{\leftrightarrow}(a,v)$ gives the 2-loop.
For any $v \in \Vs$, $R_2(a,v) \neq (a',v)$ or $R_2(a',v) \neq (a,v)$. 
\end{fact}
\begin{proof}
Let $P(a,v)=p$ and $P(a'v)=q$.
Observe that if $(\exists\; v\in\Vs)\; R_3(a,v) = (a',v,p)\ \land\ R_3(a',v) = (a,v,q)$, then the agent would fall into an infinite loop on the following gadget:
%Then $(a',v)\stackrel{q\;p}{\leftrightarrow}(a,v)$ gives the 2-loop.
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$q'$} (Y);
  \path  (B) edge [below, bend left] node {$q$} (A)
	   (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\end{center}
Indeed, if the agent's starting state is $a$ (respectively $a'$), the adversary chooses its starting position as the right (respectively left) vertex and the agent never exits from the gadget.
\end{proof}
\begin{lem}
\label{lem:ports}
Let $a\in \As$. If $(\forall\; v\in\Vs)\; P(a,v)=p$, then 
$
(\exists\; w\in \Vs)\; A(a',w)=a' \land P(a',w)=p'~.
$
\end{lem}
\begin{proof}
First observe that $(\exists\; w\in \Vs) P(a',w)=p'$, since otherwise the algorithm always takes the same port $p$ in every node with degree $2$ and thence can be trivially looped.
%Fix $w^*  \in \Vs$ such that $P(a',w^*) = p'$. 

%CASE 5.1. If all the outports are the same, then there is no way to change the direction, hence 2-loop can be trivially obtained.\\
%CASE 5.2.  
Observe that, if $(\forall\;w\in \Vs)\;P(a',w)=p' \Rightarrow A(a',w)=a$, then the agent always changes its state to $a$ whenever we takes port $p'$ and from the assumption, it always takes port $p$ in state $a$. Consider the following gadget (where $\ast$ denotes any vertex state, possibly different at each vertex):

\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (1,0) {$*$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$\ast$};
 \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$\ast$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$\ast$};
  \node (Y) at (5,0) { };
 \path 	(X) edge [above, bend left] node {$p'$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	        (B) edge [above, bend left] node {$p$} (C)
	  	(C) edge [above, bend left] node {$p'$} (D)
		(D) edge [above, bend left] node {$p'$} (Y);
  \path	 (Y) edge [below, bend left] node {$p'$} (D)
	         (D) edge [below, bend left] node {$p$} (C)
		(C) edge [below, bend left] node {$p$} (B)
		(B) edge [below, bend left] node {$p'$} (A)
		(A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\end{center}
After entering to any of the outer vertices, the agent is certainly in state $a$, because it can only enter it via port $p'$.
Hence in the next step it takes port $p$. Thus it cannot exit from such a gadget. We obtain a contradiction, so the implication cannot be true, what completes the proof of the lemma.
%then we can construct the sequence of ports:
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow}B \stackrel{p\; p}{\leftrightarrow}C\stackrel{p'\; p}{\leftrightarrow} (a,v)~,
%$$
%which blocks the opportunity to change the direction both in A and D.
%Indeed, in order to get to those vertices, we have to use port $p'$, but then the agent's bit changes to $a$. However the adversary initializes terminal positions with vertex's state $v$, then the agent has to use $P(a,v)=p$, so it goes always either to B or C.
\end{proof}
The following fact is a direct conclusion of Lemma~\ref{lem:ports}:
\begin{fact}
\label{wn5}
Let $a\in\As$. If $(\forall\; v\in\Vs)\; A(a',v)=a$, then $P(a,v)\neq P(a,v')$.
\end{fact}
%\paragraph{CASE 6. Assume that 
%$$
%(\forall\; a\in\As)(\forall\; v\in\Vs) A(a,v)=a' \lor (\exists\;a\in\As)\; V(a,v)=v~.
%$$}

% \marginpar{DB: ewentualnie to mozna rozbic na osobne przypadki 6. i 7. zamiast 6.1 i 6.2}
The next lemma shows that the agent does not change its internal state in every step.

\begin{lem}
\label{fact:1}
Fix any $a\in \As$. If $(\forall\;v\in \Vs)\;A(a,v)=a'$, then $(\exists\; w\in \Vs)\;R_2(a',w)=(a,w')\ \land\ R_2(a',w')=(a',w)$. % or the algorithm is equivalent with RR.
\end{lem}
\begin{proof}
%CASE 6.1.
By Fact \ref{wn3} we know that
\[
(\exists\; w\in \Vs)\;R_2(a',w)=(a,w')\ \land\ \left(R_2(a',w')=(a',w)\ \lor\ R_2(a',w')=(a,w)\right)~.
\]
In order to prove \autoref{fact:1}, let us assume that $R_2(a',w')=(a,w)$, what implies that the agent changes its internal state in each step (i.e. $(\forall\; a\in\As)(\forall\; v\in\Vs)\; A(a,v)=a'$).
A symmetric application of Fact \ref{wn3} shows that $(\exists\; v\in\Vs)\; R_2(a,v)=(a',v')\ \land\ R_2(a,v')=(a',v)$ (because $A(a,v')=a'$).
Hence we obtained that $(\forall\; a\in\As)(\forall\; v\in\Vs)\; R_2(a,v)=(a',v')$, what means that the states of vertices are changed upon each visit of the agent as well.
\begin{center}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge [above, bend left] (m-2-2);
    \draw[->] (m-1-2) edge [above, bend left] (m-2-1);
    \draw[->] (m-2-1) edge [above, bend left] (m-1-2);
    \draw[->] (m-2-2) edge [above, bend left] (m-1-1);
\end{tikzpicture}
\end{center}
%\db{moze narysowac ten rozwazany algorytm?}
We want to show that for such an algorithm:
\begin{equation}
  \label{eqn:differences}
   (\forall\; a\in\As)(\forall\; v\in\Vs)\; P(a,v)\neq P(a,v'). 
\end{equation}
Assume for contradition that for some $a \in \As,\ v \in \Vs,\ p \in \Ps$ we have $P(a,v) = P(a,v') = p$.
Observe that, in this case, in every step at a node with degree $2$ the agent changes its state, so at least one of every two consecutive steps at nodes with degree $2$ is via port $p$.
This shows, that on a path, where port $p$ always points towards the starting position of the agent, the agent cannot reach more than $2$ steps away from its starting position, hence it cannot explore the whole path. Thence Equation~\ref{eqn:differences} is proved for such the algorithm.

%Since we are not able to change the agent's bit at entering state of any particular position, then $(\forall\; a\in\As)(\forall\; v\in\Vs) P(a,v)\neq P(a,v')$, because otherwise there won't be possibility to change the direction at some positions, because of parity argument, which blocks the possibility to visit all the vertices.\\
Now, let us consider the following two cases:

\noindent
%CASE 6.1.1. 
\textbf{Case A: $P(a,v)=P(a',v)$}. Then, by Equation~\ref{eqn:differences}, $P(a,v')=P(a',v')$, so the outports chosen by the agent depend only on states of vertices (the agent does not use its internal state). 
Hence this algorithm is equivalent to Rotor-Router on vertices with degree $2$ and requires $\Omega(n^2)$ steps to explore the path, starting from a vertex in the middle of the path (at distance at least $\lfloor n/2 \rfloor$ from each endpoint).\\
%CASE 6.1.2. 
\textbf{Case B: $P(a,v)\neq P(a',v)$}. Again from Equation~\ref{eqn:differences} we attain $P(a',v)=P(a,v')$ and $P(a,v)=P(a',v')$.
Let us think about an equivalence relation, where $W:=(a,v)\equiv(a',v')$ and $W':=(a,v')\equiv(a',v)$.
Note that the outports of $W$ and $W'$ are different. Moreover, since the agent changes its internal state at each step, then after an even number of steps on nodes with degree $2$, the agent is always in the same state.
Consider an agent starting in the middle of the path and analyze its walk until it reaches some of the endpoints. Between successive visits to any of the vertices $x$, the agent makes an even number of steps, hence the agent always visits $x$ in the same state, but each time the state of the vertex $x$ changes to opposite.
Thus upon consecutive visits, it chooses different outports. Hence the walk performed by the agent is equivalent to Rotor-Router and for some initialization of port labels it takes $\Omega(n^2)$ steps to reach any endpoint of the path.

We obtained a contradiction in both cases, which proves that $R_2(a',w')=(a',w)$.
%Realize that after exit of some position, the vertex state changes, but the future agent's state cannot be another, so it may  be seen as changing the state from $W$ to $W'$ and viceversa. Hence this algorithm is isomorphic with RR.\\
%CASE 6.1 provides the following result:
\end{proof}
The following lemma shows that the agent changes the state of the vertex in each step at a node of degree $2$.
\begin{lem}
\label{lem:vchange}
$(\forall\; a\in\As)(\forall\; v\in\Vs)\; V(a,v)=v'$.
\end{lem}
\begin{proof}
%CASE 6.2. 
Assume, that the algorithm does not satisfy the claim, so consider such $a\in\As,\ v\in\Vs$, that $V(a,v) = v$ and denote $P(a,v)=p$.
Then from Fact~\ref{wn2} we get $R_2(a,v) = (a',v)$. Moreover from Fact~\ref{fac:CASE4}, $R_2(a',v) \neq (a,v)$ and again from Fact~\ref{wn2}, $R_2(a',v) \neq (a',v)$, hence $V(a',v) = v'$.
%. Moreover, from CASE 4. and CASE 2. we know that $(\exists\; a\in \As)\; R_2(a,v)=(a',v) \land V(a',v)=v'$.\\

We consider two cases:\\
\textbf{Case A: $R_2(a',v)=(a',v')$}. Observe that in this case from Lemma \ref{lem:vconst} we obtain $A(a',v)\neq A(a',v')=a$. Moreover, if $q = P(a',v) \neq P(a',v')=q'$, then the agent falls into infinite loop on the following gadget:

%CASE 6.2.1. Assume that $R_2(a',v)=(a',v')$. From .\\
%CASE 6.2.1.1. Realize that if $P(a,v)=p$, $P(a',v)=q$ and $P(a',v')=q'$, then we can construct a sequence:
%$$
%(a,v)\stackrel{p\; q'}{\leftrightarrow}(a',v)\stackrel{q\; q}{\leftrightarrow}(a',v)\stackrel{q'\; p}{\leftrightarrow}(a,v)~,
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (B) at (2,0) {$*$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (C) at (3,0) {$*$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
		(B) edge [above, bend left] node {$q$} (C)
	        (C) edge [above, bend left] node {$q'$} (D)
	        (D) edge [above, bend left] node {$p'$} (Y);
  \path	(D) edge [below, bend left] node {$p$} (C) 
  		(C) edge [below, bend left] node {$q$} (B)
	    (B) edge [below, bend left] node {$q'$} (A)
	    (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\end{center}
If the starting state of the agent is $a$, then the adversary chooses the starting position as the leftmost node and if it is $a'$, then of the middle nodes. Observe that if agent is in one of the outer vertices in state $a$, the agent changes its state to $a'$ and moves via port $p$ to one of the two vertices in the middle. Since $R_3(a',v) = (a',v',q)$ and $R_3(a',v') = (a,\ast,q')$ ($\ast$ takes any possible value), the next time the agent enters to the outer vertex (via port $q'$) will be in state $a$. 
And since $R_2(a,v) = (a',v)$ the states of both outer vertices remain $v$. This means that the agent cannot escape from such a gadget. 
% that agent's state never changes, so there is no possibility to change any of entering states $(a,v)$ and the agent.
 
Therefore $P(a',v)=P(a',v')$. From Lemma \ref{lem:ports} and Fact \ref{wn2} we obtain that $R_2(a,v')=(a,v)$ and $P(a',v)=P(a',v')\neq P(a,v')$.

%CASE 6.2.1.2. 
If we had $R_2(a',v')=(a,v')$, then
by Lemma \ref{lem:vconst}, $A(a,v)\neq A(a,v')=a$, hence, from Fact \ref{wn2}, $R_2(a,v')=(a,v)$. By the symmetry, we conclude that $P(a,v)=P(a,v')\neq P(a',v)=P(a',v')$, hence ports depend only on the agent's state, so we obtain the following algorithm, with simple counterexamples: 
%\subparagraph{1. (6.1,2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-2-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X)
	  (B) edge [above, bend left] node {$p'$} (Y);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X)
	  (B) edge [above, bend left] node {$p$} (Y);
\end{tikzpicture}
\end{minipage}
\end{center}

%CASE 6.2.1.3. 
On the other hand, if $R_2(a',v')\neq (a,v')$, then by Fact~\ref{wn2} we obtain $V(a',v')=v$. Recall that $A(a',v')=a$, so $R_2(a',v')=(a,v)$.
Moreover, from Lemma~\ref{lem:ports}, we get that $A(a,v')=a$, because $A(a,v)=a'$. From Fact~\ref{wn2} we attain $R_2(a,v')=(a,v)$.
%CASE 6.2.1.3.1. Let $A(a,v')=a'$.

%From Fact \ref{fact:1} we obtain $R_2(a',v')=(a,v)$. Moreover, realize that $A(a,v')=A(a,v)$, so from Lemma \ref{lem:vconst}, $V(a,v')=v$.
%From Fact \ref{wn5} we obtain that $P(a',v)\neq P(a',v')$.
%However from CASE 6.2.1.1. we have already known that $P(a',v)=P(a',v')$.\\
%CASE 6.2.1.3.2. Hence
%Recall, that $R_2(a,v')=(a,v)$.\\
%CASE 6.2.1.3.1. 
%If $R_2(a',v')=(a',v)$, then from Lemma \ref{lem:vconst} the algorithm can be easily looped.\\
%CASE 6.2.1.3.2.1. 
Now, if additionally $P(a,v')=p$, then from $P(a',v)=P(a',v')\neq P(a,v')$ %and Conclusion after CASE 6.2.1.1. 
we obtain $R_3(a',v')=(a,v,p')$ and $R_3(a',v)=(a',v',p')$, so we end up with the following algorithm and we present two gadgets for it:
%\subparagraph{2. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p'$} (A) 
 	  (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

%CASE 6.2.1.3.2.2. 
On the other hand, if alternatively $P(a,v')=p'$, %Then from CASE 6.2.1.1. we know and 
then we similarly obtain $R_3(a',v')=(a,v,p)$ and $R_3(a',v)=(a',v',p)$ and the provided algorithm falls into infinite loop on the following gadgets:

%\subparagraph{3. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p'$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path  (AA) edge [above, bend left] node {$p$} (A) 
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p'$} (X) ;
\end{tikzpicture}
\end{minipage}
\end{center}
This completes the analysis of Case A.\\
\noindent
\textbf{Case B: $R_2(a',v)=(a,v')$}.
%CASE 6.2.2. Let $R_2(a',v)=(a,v')$. 
From Lemma \ref{lem:vconst}, $A(a',v)\neq A(a',v')=a'$, so $R_2(a',v')=(a',v)$, due to Fact~\ref{wn2}.
%CASE 6.2.2.1. 
%Assume that $R_2(a,v')=(a',v')$. Then we may swap $v$ with $v'$ in order to obtain
If we had $R_2(a,v')=(a',v')$, then by symmetry we could swap $v$ with $v'$ and obtain Case A. Hence $R_2(a,v') \neq (a',v')$. 
%CASE 6.2.1.3.1., so by CASE 2. $V(a,v')=v$.\\
Again, Fact~\ref{wn2} bears $V(a,v')=v$. 
%--------------------------------------------------------
%Let $P(a,v)=p$ and $P(a',v)=q$. Then, from Lemma \ref{lem:ports} either $P(a,v')=p$ or $q=p \land P(a,v')=p'$. However, in both cases, by the Lemma \ref{lem:ports} once again we may obtain $R_2(a,v')=(a,v)$.\\
%%Hence we provide two possible algorithms in this arrangement:\\
%%I.2.1 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p')$,$R_3(a',v')=(a,v,p')$,$R_3(a,v')=(a,v,p)$\\
%%KONTRPRZYKLAD\\
%%I.2.2 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p)$,$R_3(a',v')=(a,v,p)$,$R_3(a,v')=(a,v,p')$\\
%%KONTRPRZYKLAD\\
%----------------------------
%Let $P(a,v)=p$. Realize that then $(\exists\;(x,v')\in S)(\exists\; y\in Vs)\;R_3(x,v')=(a',y,p')$.\\
%Indeed, if $P(a',v')=p$, then we may arrange
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow}(a',v)~,
%$$
%where after leaving the $(a,v)$ we won't change its vertex' state until we enter it with the agent's state $a'$ through port $p'$, so then $R_3(a,v')=(a',y,p')$ for some $y$.\\
%-----------------------------------------
%CASE 6.2.2.2.

%TEN CASE PRZERZUCONY DO GLOWNEJ CZESCI!!!!!
%Assume that $P(a',v)=P(a',v')=p'$.
%Then $P(a,v')=p$ and $A(a,v')=a$ from Lemma \ref{lem:ports}, so $R_3(a,v')=(a,v,p)$. We obtained the algorithm, in which the agent can be looped by the following gadgets: 
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
  %\matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  %{
    %{$a$ \\ $v$}& {$a'$ \\ $v$} \\
     %{$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     %};
    %\draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    %\draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
    %\draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    %\draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}[->]
 %\node (X) at (0,0) { };
 %\node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 %\node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v'$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  %\node (Y) at (5,0) { };
 %\path (A) edge [above, bend left] node {$p$} (B)
	  %(B) edge [above, bend left] node {$p'$} (C)
	  %(C) edge [above, bend left] node {$p$} (D)
	  %(D) edge [above, bend left] node {$p'$} (Y);
  %\path (D) edge [below, bend left] node {$p$} (C)
	  %(C) edge [below, bend left] node {$p'$} (B)
	  %(B) edge [below, bend left] node {$p$} (A)
	  %(A) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\begin{tikzpicture}[->]
 %\node (X) at (0,0) { };
  %\node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 %\node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 %\node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v'$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  %\node (Y) at (6,0) { };
 %\path  (AA) edge [above, bend left] node {$p'$} (A) 
           %(A) edge [above, bend left] node {$p$} (B)
	  %(B) edge [above, bend left] node {$p'$} (C)
	  %(C) edge [above, bend left] node {$p$} (D)
	  %(D) edge [above, bend left] node {$p'$} (Y);
  %\path (D) edge [below, bend left] node {$p$} (C)
	  %(C) edge [below, bend left] node {$p'$} (B)
	  %(B) edge [below, bend left] node {$p$} (A)
	  %(A) edge [below, bend left] node {$p'$} (AA)
	  %(AA) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}
%\end{minipage}
%\end{center}
Suppose that $P(a',v)=P(a',v')=p'$. Then $P(a,v')=p$ and $A(a,v')=a$ from Lemma \ref{lem:ports}, so $R_3(a,v')=(a,v,p)$, what provides Algorithm Q from Section~\ref{sec:line}, which can be looped by the adversary.
Thence we assume that either $P(a',v)\neq p'$ or $P(a',v')\neq p'$. Moreover, let us denote $P(a',v')=q$.
%Assume for a while that $R_2(a,v')=(a',v)$ and 
%denote $P(a',v)=q$. Due to Fact \ref{wn5}, $P(a',v)\neq P(a',v')$, hence $P(a',v')=q'$.
%CASE 6.2.2.2.1.
%If $P(a,v')=p$, then on the following gadget:
%$$
%(a,v)\stackrel{p\; q}{\leftrightarrow} (a',v)\stackrel{q'\; q'}{\leftrightarrow} (a',v) \stackrel{q\; p}{\leftrightarrow} %(a,v)~,
%$$
Consider the following gadget (if the agent starts in state $a$ it is initialized on one of the outer vertices and otherwise on one of the inner vertices, what is indicated above the nodes):
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] { } (m-2-1);
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-2-2) edge node [right, near start] {$q$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (D) at (4,0) {$v$};
 \path 	(A) edge [above, bend left] node {$p$} (B)
		(B) edge [above, bend left] node {$q$} (C)
	        (C) edge [above, bend left] node {$q'$} (D);
  \path	(D) edge [below, bend left] node {$p$} (C) 
  		(C) edge [below, bend left] node {$q$} (B)
	        (B) edge [below, bend left] node {$q'$} (A);
\end{tikzpicture}
\end{minipage}
\end{center}%\db{moze przy okazji narysowac algorytm}

%In order to escape from this gadget, the agent has to enter to one of the outer vertices in state $a'$, since otherwise it exits via port $p$ without changing the state of the vertex. 
Consider the following three invariants: 
\begin{itemize}
\item[I1] While the agent visits one of the inner vertices in state $a$, then the state of this vertex is always $v$.
\item[I2] The agent visits the outer vertices always in state $a$.
\item[I3] The state of the outer vertices is always $v$.
\end{itemize}
Notice, that as long as the invariants are not violated, the agent cannot escape the gadget because it always exits via port $q'$ from the outer vertices. Observe, that the invariants are initially true and assume that all three invariants were true up to some step $t$. We want to show that the invariants will remain true after this step.

First, we show that the agent cannot violate I3 in step $t+1$. In order to do so, it need to change the state of an outer vertex from $v$ to $v'$, so it has to visit this vertex in state $a'$ while entering to the vertex via port $q'$. Therefore, at the moment $t$, the agent should have internal state $a$, so since the invariant I1 was not violated, the appropriate vertex had state $v$. In consequence, $P(a,v)=q'$, hence $q=p'$. From the assumption, $P(a',v)=p$.
Note that the internal state of the agent cannot be changed to $a$ during the step $t-1$, from outer node to inner node, because it either violates I2 or I3.
Therefore such the move should be between two inner nodes, via port $q$.

Hence, from invariant I1, we may conclude that $P(a',v)=q=p'$, contrary to previous observation.
%Since $R_3(a',v')= (a',v,q')$ and $R_3(a',v) = (a,v',q)$, then if the agent is in state $a'$ in one of the inner vertices, then it either takes port $q'$ (and moves to the other inner vertex) or it changes its state to $a$ and goes to the outer vertex.
The same argument shows that the agent also cannot violate I2 in step $t+1$.
%, because in order to enter to the outer vertices in state $a'$ it had to be in state $a$ in one of the inner vertices thus it had to violate I1 before that.

As long as invariants I2 and I3 are not violated, the agent always enters to inner vertices from outer vertices in state $a'$.
Thence, in order to violate I1, the state of the agent has to be changed to $a$ during the pass between the middle nodes (via port $q$), so $R_3(a',v)=(a,v',q)$ (otherwise the agent had to violate I1 before).
Then, from the assumption, $q$ cannot be $p'$, so from Lemma~\ref{lem:ports}, $P(a,v')=p'$. However, then the only way to go to outer node is via port $p'$, but then the agent violates I1.
%Moreover if the agent is in state $a'$ in the inner vertex it either keeps its state $a'$ or moves to an outer vertex. 
Hence the agent cannot violate any of the invariants hence it cannot escape the gadget.
This completes the proof of Case B.
%In order to do so, the state of the agent has to be in state $a'$ $x$. This means that in the pervious 
% However it can only be obtained from the agent's state $a$, so $p=q$. Now, consider the step $x-1$. Then one of the middle vertices has to be entered either from boundary node $(a,v)$ by port $p$ with agent's state $a'$ or by port $q'=p'$, from the state $(a',v')$, with the agent's state $a'$ as well, what contradictes that agent's state before step $x-1$ is $a$.\\
%CASE 6.2.2.2.2. Hence $P(a,v')=p'$.\\
%CASE 6.2.2.2.2.1 Let $q=p$.\\
%\subparagraph{5A. (6.2.3.2.2)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
%    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p$} (m-2-1);
%    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
%    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
% \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
% \path (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p'$} (C)
%	  (C) edge [above, bend left] node {$p$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p'$} (B)
%	  (B) edge [below, bend left] node {$p$} (A)
%	  (A) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
%  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
%  \node (Y) at (6,0) { };
% \path (AA) edge [above, bend left] node {$p$} (A) 
% 	 (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p'$} (C)
%	  (C) edge [above, bend left] node {$p$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p'$} (B)
%	  (B) edge [below, bend left] node {$p$} (A)
%	  (A) edge [below, bend left] node {$p'$} (AA)
%	  (AA) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\end{minipage}
%\end{center}
%
%CASE 6.2.2.2.2.2. Let $q=p'$.\\
%
%\subparagraph{5B. (6.2.3.2.2)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
%    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
%    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
%    \draw[->] (m-2-2) edge node [right, near start] {$p$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
% \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
% \path (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p$} (C)
%	  (C) edge [above, bend left] node {$p'$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p$} (B)
%	  (B) edge [below, bend left] node {$p'$} (A)
%	  (A) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
%  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
%  \node (Y) at (6,0) { };
% \path (AA) edge [above, bend left] node {$p'$} (A)  
% 	 (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p$} (C)
%	  (C) edge [above, bend left] node {$p'$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p$} (B)
%	  (B) edge [below, bend left] node {$p'$} (A)
%	  (A) edge [below, bend left] node {$p'$} (AA)
%	  (AA) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}
%\end{minipage}
%\end{center}
%
%Let $P(a',v')=p$. Realize that the agent's state $a'$ can be obtained only from the states $(a,v)$ and $(a',v')$, so it can be only obtained via port $p$. Therefore, in the beneath gadget, the agent cannot have the state $a'$ in outer vertices, hence he cannot change the states of outer vertices, so agent falls in an infinite loop:
%\begin{center}
%\begin{tikzpicture}[->]
 %\node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 %\node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 %\node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 %\path 	(Z) edge [above, bend left] node {$p$} (A)
		%(A) edge [above, bend left] node {$p$} (B)
	        %(B) edge [above, bend left] node {$p'$} (C);
  %\path	(C) edge [below, bend left] node {$p$} (B) 
  		%(B) edge [below, bend left] node {$p$} (A)
	        %(A) edge [below, bend left] node {$p'$} (Z);
%\end{tikzpicture}
%\end{center}
%
%
%
%
%
%
%Therefore $P(a',v)=p$.
%%Indeed, in order to change either of the boundary states, the agent needs to use the port $p$ with agent's state $a'$, while entering them. It is only possible, if he goes from the inner vertex of state $(a,v)$. 
%Consider the following gadget:
%\begin{center}
%\begin{tikzpicture}[->]
 %\node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 %\node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 %\node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 %\path 	(Z) edge [above, bend left] node {$p$} (A)
		%(A) edge [above, bend left] node {$p'$} (B)
	        %(B) edge [above, bend left] node {$p$} (C);
  %\path	(C) edge [below, bend left] node {$p$} (B) 
  		%(B) edge [below, bend left] node {$p'$} (A)
	        %(A) edge [below, bend left] node {$p$} (Z);
%\end{tikzpicture}
%\end{center}
%Note that then in order to change the agent state to $a'$ via port $p$, the agent has to have internal state $a$ and vertex state $v$. \db{to poprawic na niezmienniki}
%Note that the agent cannot enter to the one of the middle vertices via port $p$ with agent state $a$ (because $A(a,v)=a'$), so the agent has to enter to it via $p'$.
%Therefore $P(a,v')=p'$ and the agent$(a,v')$ had to be a state of the other middle vertex. Recursively, we may prove that at least one of the middle states has to be initated with agent's state $a$, which is not true.
\end{proof}
\input{sections/twoalgs.tex}

%
%\subparagraph{8. (7.1.1.2.2)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
%    \draw[->,bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
%    \draw[->,bend left] (m-2-1) edge node [right, very near start] {$p$} (m-1-2);
%    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%TODO
%\end{minipage}
%\end{center}

\input{sections/line_end}

==> sections/counterexamples.tex <==
% !TEX root = ../dual_memory.tex
\paragraph{Counterexamples}
\subparagraph{4A. (6.2,3.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p$} (m-2-1);
    \draw[->] (m-2-1) edge node [below, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v'$};
  \node (Y) at (6,0) { };
 \path  (AA) edge [above, bend left] node {$p$} (A)
 	  (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

\subparagraph{4B. (6.2,3.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
    \draw[->] (m-2-1) edge node [below, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (Y);
  \path (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p'$} (A)
 	  (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (Y);
  \path (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

\subparagraph{9. (7.2.2.2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->,bend left] (m-1-1) edge node [right, near start] {$p$} (m-2-1);
    \draw[->] (m-1-2) edge node [left, near start] {$p'$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [left, very near start] {$p'$} (m-1-1);
    \draw[->] (m-2-2) edge node [right, near start] {$p$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
Rotor-router
\end{minipage}
\end{center}

\subparagraph{11. (7.2.4)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[bend left] (m-1-1) edge node [right, near start] {$p$} (m-2-1);
    \draw[bend left] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[bend left] (m-2-1) edge node [left,near start] {$p'$} (m-1-1);
    \draw[bend left] (m-2-2) edge node [left, near start] {$p$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
Rotor-router
\end{minipage}
\end{center}

\subparagraph{12. (7.2.5)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw (m-1-1) edge node [left, near start] {$p$} (m-2-1);
    \draw[bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
    \draw[bend left] (m-2-1) edge node [right, very near start] {$p'$} (m-1-2);
    \draw (m-2-2) edge node [right, near start] {$p$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X)
	  (B) edge [above, bend left] node {$p$} (Y);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X)
	  (B) edge [above, bend left] node {$p$} (Y);
\end{tikzpicture}
\end{minipage}
\end{center}


==> sections/line_1.tex <==
%line.tex
% !TEX root = ../dual_memory.tex
\newcommand{\As}{\mathrm{As}}
\newcommand{\Vs}{\mathrm{Vs}}
\newcommand{\Ps}{\mathrm{Ps}}

\section{Line topology with dirty memory}

\subsection{1 bit per agent, 1 bit per vertex}
A simple round-robin strategy for graph exploration, understood as taking a port different from the previous one on each visit to a vertex of degree $2$, results in exploration time of a path $O(n^2)$. Such a strategy can be clearly implemented with only a single bit at each vertex and zero bits on the agent (if we don't require termination). This strategy can be generalized to arbitrary graphs and such an algorithm, called Rotor-Router works in time $O(mD)$~\cite{YanovskiWB03} for state arbitrary initialization and arbitrary port labelling.
%A classical solution shows that there exists an algorithm, which enables to perform a simple exploration algorithm on a line of size $n$ in $O(n^2)$ steps called Rotor-Router (abbreviated by RR). Every time, when an agent enters a vertex, (excluding two ends of the line) it changes its state to opposite and uses a number of port, which is indicated by this state (every time it enters the opposite port as well).

It is known that adding more bits of memory on the vertices does not help as time $\Omega(n^2)$ is required even in the model with unlimited memory on each node ~\cite{MencPU17}.
In this section  we additionally allow the agent to have $1$ bit of memory and we want to answer the question of whether this single bit allows to break the $\Omega(n^2)$ barrier.

\paragraph{Notation}
In the following lower bound on the line, we take any algorithm working with a single bit at the agent and a single bit at each node. We will focus on the actions of the algorithm in vertices with degree $2$. In such vertices, there are four possible inputs to the algorithm $S = \{(0,0),(0,1),(1,0),(1,1)\}$, where in pair $(a,v)$, $a$ is a bit on the agent and $v$ is a bit saved on the vertex. Let us denote the agent's states by $\As$, vertex' states by $\Vs$ and possible outports by $\Ps$. We use a shorthand notation $'$ to indicate the inverted value of a bit. For example, if $a=0$, then $a'=1$ and vice versa. 


%We denote an entering state as a pair $(a,v)$, where $a$ is a bit on the agent and $v$ is a bit saved on the vertex. At each step at a node with degree $2$, an algorithm has to return some pair $(b,w)$ and port number $p$, depending on the state of the vertex and the state of the agent. Then the agent changes its state to $b$, the state of vertex to $w$ and quits the actual vertex via port $p$. 

%If the vertex is an endpoint of the line, then agent can leave the only by one port. (NIE ANALIZOWALEM JAK SIE ZMIENIA DECYZJA JESLI WIADOMO, ZE TO PUNKT KONCOWY --- TO TRZEBA DODAC)





%The same for vertex' states and ports.

%
%\begin{tikzpicture}[->]
 %\node (X) at (0,0) { };
 %\node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 %\node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    %\node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      %\node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  %\node (Y) at (7,0) { };
 %\path (A) edge [above, bend left] node {$p'$} (B)
	  %(B) edge [above, bend left] node {$p'$} (C)
	  %(C) edge [above, bend left] node {$p'$} (D)
	  %(D) edge [above, bend left] node {$p$} (E)
	  %(E) edge [above, bend left] node {$p$} (F)
	  %(F) edge [above, bend left] node {$p$} (Y);
  %\path (F) edge [below, bend left] node {$p'$} (E)
           %(E) edge [below, bend left] node {$p'$} (D)
  	  %(D) edge [below, bend left] node {$p'$} (C)
	  %(C) edge [below, bend left] node {$p$} (B)
	  %(B) edge [below, bend left] node {$p$} (A)
	  %(A) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}

The goal of this section is to prove the following:
\begin{theorem}
\label{ref:thm}
Any algorithm in the model with one bit at the agent and one bit at each node requires in worst-case time $\Omega(n^2)$ to explore a path.
\end{theorem}
Assume for contradiction, that some algorithm $\mathcal{A}$ explores any path in $o(n^2)$ steps. For algorithm $\mathcal{A}$, for any $s \in S$, by $A(s), V(s), P(s)$ we denote respectively, the returned agent state, vertex state and the chosen outport in each vertex with degree $2$. Moreover, we denote $R_3(s):=(A(s),V(s),P(s))$ and $R_2(s):=(A(s),V(s))$. In the following series of facts we will prove some properties that $\mathcal{A}$ has to satisfy. 

\begin{fact}
\label{wn1}
 $(\forall\; a\in \As)(\exists\; v\in \Vs)\; A(a,v)=a'$.
% or the algorithm reduces to RR.
\end{fact}
\begin{proof}
Assume that $(\exists\; a \in \As)(\forall\; v\in \Vs)\; A(a,v)=a$ and let the starting position be the midpoint of the path. If $a$ is the starting state of the agent, then the agent will never change its state before reaching an endpoint of the path. But before that the exploration is not faster than rotor-router, hence there exists an initialization of port numbers, such that reaching the endpoint takes $\Omega(n^2)$ steps. If $a'$ is the starting state, then either $A(a',w)=a$, for some $w \in \Vs$. In this case, the adversary sets $w$ to be the starting state of the starting vertex and from the second step the algorithm explores not faster than the rotor-router hence needs $\Omega(n^2)$ steps to reach an endpoint. Note that if $A(a',w)=a'$ for each $w\in \Vs$, then this reduces to the first case. The obtained contradiction completes the proof of the fact.
\end{proof}

\begin{fact}
\label{wn2}
For any $a \in \As$ and $v \in \Vs$ we have $R_2(a,v) \neq (a,v)$.
\end{fact}
\begin{proof}
We will show that otherwise algorithm $\mathcal{A}$ falls into infinite loop for some initial state of the path. Assume that $R_3(a,v) = (a,v,p)$ for some entering state $(a,v)$ and port $p \in \Ps$. Then if $a$ is the starting state, it is easy to see that the agent falls into infinite loop on the following gadget (double circle indicates the starting position of the agent):
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}
If $a'$ is the starting state, then we can use Fact~\ref{wn1}, $(\exists\; w\in \Vs)\;A(a',w)=a$. Let $q = P(a',w)$ (it is possible that $p = q$) and observe that the  agent falls into infinite loop in the following gadget:
%$$
%\underline{(a',w)}\stackrel{q\;p'}{\leftrightarrow}(a,v)\stackrel{p\;p}{\leftrightarrow}(a,v)
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (Z) at (1,0) {$w$};
  \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (3,0) {$v$};
  \node (Y) at (4,0) { };
 \path 	(Z) edge [above, bend left] node {$q$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (Z)
		(Z) edge [below, bend left] node {$q'$} (X);
\end{tikzpicture}\\
\end{center}

%which after first step reduces to the CASE 2.1.\\
%Thanks to the CASE 2. we obtain following results:
\end{proof}

\begin{lem}
\label{lem:vconst}
Fix any $a \in \As$ and $v\in \Vs$. Algorithm $\mathcal{A}$ does \textbf{not} satisfy the following:
\[
%(\forall\;a,x\in \As)(\forall\;v,y,z\in Vs)\;R_2(a,v)=(a',v) \land R_2(a',v)=(x,y)\land R_2(a',v')=(x,z).
R_2(a,v)=(a',v) \land A(a',v) = A(a',v').
\]
%Then the adversary can initialize the algorithm in such the way, to either produce infinite loop either reduce the algorithm to RR.

\end{lem}

\begin{proof}
%CASE 3. 
Assume that the formula holds for some $a \in \As$ and $v\in \Vs$ and we will show that in such a case $\mathcal{A}$ would fall into an infinite loop for some initializations of the path. 
From Fact \ref{wn1}, we obtain, that $A(a',v) = A(a',v') = a$. Denote $P(a,v)=p$ and $V(a',v)= y$.\\
%CASE 3.1. 

If $y=v$, then let $P(a',v)=q$, and the following initial state of the path results in an infinite loop: 
%$\underline{(a,v)}\stackrel{p\;q}{\leftrightarrow}(a',v)$ 
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (Y);
  \path	 (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}

%so only two vertices will be visited.\\
%CASE 3.2. 
In the opposite case, where $y = v'$, the agent would fall into an infinite loop on the following gadget:
%$$
%(a,v)\stackrel{p\;p}{\leftrightarrow}(a',v')\stackrel{p'\;p}{\leftrightarrow}(a,v)~,
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v'$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (3,0) {$v$};
  \node (Y) at (4,0) { };
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (Z)
		(Z) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}

%which leads to infinite loop.\\
We have $R_3(a,v) = (a',v,p)$, hence in the first step, the agent moves to the middle vertex, changes its state to $a'$, and keeps $v$ as the state of the first vertex.
At the middle vertex when the agent's state is $a'$, then it always changes its state to $a$ and moves to one of the outer vertices. But since the outer vertices are both in state $v$, the agent returns to the middle vertex, and so on, which is an infinite loop.
%and, hence we always return to the middle vertex from the entering state $(a,v)$, hence the outer vertices' states won't change as well, so we never visit any of the positions excluding these 3.
\end{proof}

The following fact characterises features of an algorithm, in which some state $a$ of the agent is flipped for both states of a vertex.
\begin{fact}
\label{wn3}
Fix any $a\in\As$. %\marginpar{DB: Wybieramy dowolne a. Ale obydwa fakty dotycza tego samego a; Innymi słowy: jak pewne a spełnia warunek ifa, to zachodza dla niego te dwie wlasnosci. Jesli a' tez spelnia analogiczny warunek z ifa, to dla niego tez beda zachodzily analogiczne wlasnosci z primami przy stanach agentow; To wynika z Lematu 1. dla $a'=a$, $x=a'$, raz przy $v=v$, a raz przy $v=v'$.} 
If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then:
%$(\forall\; w\in \Vs)\; R_2(a',w)\neq(a,w)$ and moreover, from Fact \ref{wn2}, then 
%$(\forall\; w\in \Vs)\; V(a',w)=w'$.
\begin{enumerate}[label=\roman*.,ref=\roman*]
\item\label{fct:31} $(\forall\; w\in \Vs)\; R_2(a',w)\neq(a,w)$,
\item\label{fct:32} $(\forall\; w\in \Vs)\; V(a',w)=w'$,
\item\label{fct:33} $(\exists\; w\in \Vs)\; R_2(a',w)=(a,w')$.
\end{enumerate}
\end{fact}
\begin{proof}
For each $w\in\Vs$, claim~\ref{fct:31} follows from Lemma~\ref{lem:vconst} for $a', w$, and Claim~\ref{fct:32} follows from Fact~\ref{wn2}. Claim~\ref{fct:33} follows from Fact~\ref{wn1} and claims~\ref{fct:31},~\ref{fct:32}.
\end{proof}
%\marginpar{DB: dlatego moze wartop rozbic to na 2 fakty}

%\begin{fact}
%\label{wn4}
%Fix any $a\in\As$. If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then, from facts \ref{wn1} and \ref{wn3}, 
%$(\exists\; w\in \Vs)\; R_2(a',w)=(a,w')$.
%\marginpar{DB: tutaj mogloby byc z faktu 3. tylko $R_2(a',w)=(a,w')$ albo $R_2(a',w)=(a',w')$, ale z faktu 1. musi choc raz zmieniac stan agenta.}
%\end{fact}


\begin{fact}
\label{fac:CASE4}
%CASE 4\dpa{CASE 4 -- to jest do któregoś z faktów?}. 
%Assume that for some $v$, $R_3(a,v)=(a',v,p)$ and $R_3(a',v)=(a,v,q)$. Then $(a',v)\stackrel{q\;p}{\leftrightarrow}(a,v)$ gives the 2-loop.
For any $v \in \Vs$, $R_2(a,v) \neq (a',v)$ or $R_2(a',v) \neq (a,v)$. 
\end{fact}
\begin{proof}
Observe that if we had for some $v$, that $R_3(a,v) = (a',v,p)$ and $R_3(a',v) = (a,v,q)$, for any $p,q \in \Ps$, then the agent would fall into an infinite loop on the following gadget:

%Then $(a',v)\stackrel{q\;p}{\leftrightarrow}(a,v)$ gives the 2-loop.

\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$q'$} (Y);
  \path  (B) edge [below, bend left] node {$q$} (A)
	   (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}
If the agent's starting state is $a$ ($a'$), the adversary chooses its starting position as the right (left) vertex and in both cases the agent never exits from the gadget.

\end{proof}


\begin{lem}
\label{lem:ports}
For any $a\in \As$. If $(\forall\; v\in\Vs)\; P(a,v)=p$, then 
$$
(\exists\; w\in \Vs)\; A(a',w)=a' \land P(a',w)=p'~.
$$
\end{lem}

\begin{proof}
First observe that $(\exists\; w\in \Vs) P(a',w)=p'$, since otherwise the algorithm always takes the same port $p$ in every node with degree $2$. 
%Fix $w^*  \in \Vs$ such that $P(a',w^*) = p'$. 

%CASE 5.1. If all the outports are the same, then there is no way to change the direction, hence 2-loop can be trivially obtained.\\
%CASE 5.2.  
Observe that, if $(\forall\;w\in Vs)\;P(a',w)=p' \Rightarrow A(a',w)=a$, then the agent always changes its state to $a$ after taking port $p'$ and always takes port $p$ in state $a$. Consider the following gadget (where $*$ denotes any vertex state, possibly different at each vertex):

\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (1,0) {$*$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$*$};
 \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$*$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$*$};
  \node (Y) at (5,0) { };
 \path 	(X) edge [above, bend left] node {$p'$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	        (B) edge [above, bend left] node {$p$} (C)
	  	(C) edge [above, bend left] node {$p'$} (D)
		(D) edge [above, bend left] node {$p'$} (Y);
  \path	 (Y) edge [below, bend left] node {$p'$} (D)
	         (D) edge [below, bend left] node {$p$} (C)
		(C) edge [below, bend left] node {$p$} (B)
		(B) edge [below, bend left] node {$p'$} (A)
		(A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}
After entering to any of the outer vertices, the agent is certainly in state $a$ because it can only enter via port $p'$. Hence in the next step it takes port $p$. Thus it cannot exit from such a gadget. We obtain a contradiction, hence the implication cannot be true, which completes the proof of the lemma.


%then we can construct the sequence of ports:
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow}B \stackrel{p\; p}{\leftrightarrow}C\stackrel{p'\; p}{\leftrightarrow} (a,v)~,
%$$
%which blocks the opportunity to change the direction both in A and D.
%Indeed, in order to get to those vertices, we have to use port $p'$, but then the agent's bit changes to $a$. However the adversary initializes terminal positions with vertex's state $v$, then the agent has to use $P(a,v)=p$, so it goes always either to B or C.
\end{proof}
The following Fact is a direct conclusion of Lemma~\ref{lem:ports}.
\begin{fact}
\label{wn5}
If $(\forall\; v\in\Vs)\; A(a',v)=a$, then $P(a,v)\neq P(a,v')$.
\end{fact}

%\paragraph{CASE 6. Assume that 
%$$
%(\forall\; a\in\As)(\forall\; v\in\Vs) A(a,v)=a' \lor (\exists\;a\in\As)\; V(a,v)=v~.
%$$}

% \marginpar{DB: ewentualnie to mozna rozbic na osobne przypadki 6. i 7. zamiast 6.1 i 6.2}
The next lemma shows that the agent does not change its internal state in every step.

\begin{lem}
\label{fact:1}
Fix any $a\in \As$. If $(\forall\;v\in \Vs)\;A(a,v)=a'$, then $(\exists\; w\in \Vs)\;R_2(a',w)=(a,w') \land R_2(a',w')=(a',w)$. % or the algorithm is equivalent with RR.
\end{lem}
\begin{proof}
%CASE 6.1.
By Fact \ref{wn3} we know that $(\exists\; w\in \Vs)\;R_2(a',w)=(a,w')$ and that either $R_2(a',w')=(a',w)$ or $R_2(a',w')=(a,w')$. If the statement of this fact is not correct, then $R_2(a',w')=(a,w')$, which means, that the agent changes its internal state in each step (i.e., $(\forall\; a\in\As)(\forall\; v\in\Vs)\; A(a,v)=a'$).
  By the symmetry and Fact \ref{wn3} we obtain that $(\forall\; a\in\As)(\forall\; v\in\Vs)\; R_2(a,v)=(a',v')$, which means that the vertices' states are changed upon each visit of the agent. We want to show that for such an algorithm:
  \begin{equation}
  \label{eqn:differences}
   (\forall\; a\in\As)(\forall\; v\in\Vs) P(a,v)\neq P(a,v'). 
   \end{equation}
   Assume for contrary that for some $a_1 \in \As,v_1 \in \Vs$ we have $P(a_1,v_1) = P(a_1,v_1') = p$, for some $p \in \Ps$. Observe that in this case, since in every step at a node with degree $2$, the agent changes its state, then out of every two consecutive steps at nodes with degree $2$, at least one is via port $p$. This shows, that on a path, where port $p$ always points towards the starting position of the agent, the agent cannot reach more than $2$ steps away from its starting position, hence it cannot explore the whole path. This completes the proof of Equation~\ref{eqn:differences}.

%Since we are not able to change the agent's bit at entering state of any particular position, then $(\forall\; a\in\As)(\forall\; v\in\Vs) P(a,v)\neq P(a,v')$, because otherwise there won't be possibility to change the direction at some positions, because of parity argument, which blocks the possibility to visit all the vertices.\\


Consider the following two cases:
%CASE 6.1.1. 
if $P(a,v)=P(a',v)$, then, by Equation~\ref{eqn:differences}, $P(a,v')=P(a',v')$, and the outports chosen by the agent depend only on states of vertices (the agent does not use its internal state), hence this algorithm is equivalent to Rotor-Router on vertices with degree $2$, hence it requires $\Omega(n^2)$ steps to explore a path, starting from a vertex in the middle of the path (at distance at least $\lfloor n/2 \rfloor$ from each endpoint).\\
%CASE 6.1.2. 
Otherwise, again from Equation~\ref{eqn:differences} $P(a',v)=P(a,v')$ and $P(a,v)=P(a',v')$. We may think of an equivalence relation, where $(a,v)\equiv(a',v')=W$ and $(a,v')\equiv(a',v)=W'$. Then the outports of $W$ and $W'$ are different. Now, observe, that since the agent changes its internal state at each step, then after an even number of steps on nodes with degree $2$, the agent is always in the same state. Notice, that to return to a some vertex, the agent has to make an even number of steps. Consider an agent starting in the middle of a path and analyze its walk until it reaches some of the endpoints. Between succesive visits to any of the vertices $x$, the agent makes an even number of steps hence the agent always visits $x$ in the same state. Thus upon consecituve visits, it choses different outports. Hence the walk performed by the agent is equivalent to Rotor-Router and for some initialization of port labels it takes $\Omega(n^2)$ steps to reach any endpoint of the path.


We obtained a contradiction in both cases, which proves the fact. 

%Realize that after exit of some position, the vertex state changes, but the future agent's state cannot be another, so it may  be seen as changing the state from $W$ to $W'$ and viceversa. Hence this algorithm is isomorphic with RR.\\
%CASE 6.1 provides the following result:
\end{proof}
The following lemma shows that the agent changes the state of the vertex in each step at a node of degree $2$.
\begin{lem}
\label{lem:vchange}
$(\forall\; a\in\As)(\forall\; v\in\Vs) V(a,v)=v'$.
\end{lem}
\begin{proof}
%CASE 6.2. 
Assume, that the algorithm does not satisfy the claim and fix such $a,v$, that $V(a,v) = v$. Then from Fact~\ref{wn2} we get $R_2(a,v) = (a',v)$. Moreover from Fact~\ref{fac:CASE4}, $R_2(a',v) \neq (a,v)$ and again from Fact~\ref{wn2} $R_2(a',v) \neq (a',v)$, hence $V(a',v) = v'$.
%. Moreover, from CASE 4. and CASE 2. we know that $(\exists\; a\in \As)\; R_2(a,v)=(a',v) \land V(a',v)=v'$.\\

We consider two cases:\\
\textbf{Case A: $R_2(a',v)=(a',v')$}. Observe that in this case Lemma \ref{lem:vconst} we obtain $A(a',v')=a$. Observe that if we had $q = P(a',v) \neq P(a',v')=q'$, then on the following gadget:


%CASE 6.2.1. Assume that $R_2(a',v)=(a',v')$. From .\\
%CASE 6.2.1.1. Realize that if $P(a,v)=p$, $P(a',v)=q$ and $P(a',v')=q'$, then we can construct a sequence:
%$$
%(a,v)\stackrel{p\; q'}{\leftrightarrow}(a',v)\stackrel{q\; q}{\leftrightarrow}(a',v)\stackrel{q'\; p}{\leftrightarrow}(a,v)~,
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (B) at (2,0) {$*$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (C) at (3,0) {$*$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$ $] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
		(B) edge [above, bend left] node {$q$} (C)
	        (C) edge [above, bend left] node {$q'$} (D)
	        (D) edge [above, bend left] node {$p'$} (Y);
  \path	(D) edge [below, bend left] node {$p$} (C) 
  		(C) edge [below, bend left] node {$q$} (B)
	    (B) edge [below, bend left] node {$q'$} (A)
	    (A) edge [below, bend left] node {$p'$} (X);
  		

\end{tikzpicture}\\
\end{center}
If the starting state of the agent is $a$, then the adversary chooses the starting position as the leftmost node and if it is $a'$, then of the middle nodes. Oberve that if agent is in one of the outer vertices in state $a$, the agent changes its state to $a'$ and moves via port $p$ to one of the two vertices in the middle. Since $R_2(a',v) = (a',v')$ and $R_3(a',v') = (a,*,q')$, the next time the agent enters to the outer vertices (via port $q' \neq q$) it will be in state $a$. And since $R_2(a,v) = (a',v)$ the state of the outer vertices remains $v$. This means that the agent cannot escape from such a gadget. 
% that agent's state never changes, so there is no possibility to change any of entering states $(a,v)$ and the agent. 
This shows that $P(a',v)=P(a',v')$. Moreover, from Lemma \ref{lem:ports} we obtain that $R_2(a,v')=(a,v)$ and $P(a',v)=P(a',v')\neq P(a,v')$.

%CASE 6.2.1.2. 
If we had $R_2(a',v')=(a,v')$, then by Lemma \ref{lem:vconst},  $A(a,v')=a$, hence, from Fact \ref{wn2}, $R_2(a,v')=(a,v)$. By the same argument as above, we conclude that $P(a,v)=P(a,v')$, hence ports depend only on the agent's state, so by Lemma \ref{lem:ports} we obtain the following algorithm, with simple counterexamples: 

%\subparagraph{1. (6.1,2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-2-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X)
	  (B) edge [above, bend left] node {$p'$} (Y);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X)
	  (B) edge [above, bend left] node {$p$} (Y);
\end{tikzpicture}
\end{minipage}
\end{center}

%CASE 6.2.1.3. 
If on the other hand $R_2(a',v')\neq (a,v')$, then by Fact~\ref{wn2} we obtain $V(a',v')=v$ and by Lemma \ref{lem:vconst} we get $R_2(a',v')=(a,v)$.
%CASE 6.2.1.3.1. Let $A(a,v')=a'$.

%From Fact \ref{fact:1} we obtain $R_2(a',v')=(a,v)$. Moreover, realize that $A(a,v')=A(a,v)$, so from Lemma \ref{lem:vconst}, $V(a,v')=v$.
%From Fact \ref{wn5} we obtain that $P(a',v)\neq P(a',v')$.
%However from CASE 6.2.1.1. we have already known that $P(a',v)=P(a',v')$.\\
%CASE 6.2.1.3.2. Hence
%Recall, that $R_2(a,v')=(a,v)$.\\
%CASE 6.2.1.3.1. 
%If $R_2(a',v')=(a',v)$, then from Lemma \ref{lem:vconst} the algorithm can be easily looped.\\
%CASE 6.2.1.3.2.1. 
If $R_3(a,v')=(a,v,p)$, then from Lemma \ref{lem:ports} %and Conclusion after CASE 6.2.1.1. 
we obtain $R_3(a',v')=(a,v,p')$ and $R_3(a',v)=(a',v',p')$ and we obtain the following algorithm with counterexamples:

%\subparagraph{2. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-1-1);
\end{tikzpicture}

\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p'$} (A) 
 	  (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}

\end{minipage}
\end{center}


%CASE 6.2.1.3.2.2. 
On the other hand if $R_3(a,v')=(a,v,p')$. %Then from CASE 6.2.1.1. we know and 
Then by Lemma \ref{lem:ports} we obtain $R_3(a',v')=(a,v,p)$ and $R_3(a',v)=(a',v',p)$ and the obtained algorithm falls into infinite loop on the following gadget:

%\subparagraph{3. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p'$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path  (AA) edge [above, bend left] node {$p$} (A) 
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p'$} (X) ;
\end{tikzpicture}
\end{minipage}
\end{center}
This completes the analysis of Case A.\\
\noindent
\textbf{Case B: $R_2(a',v)=(a,v')$}
%CASE 6.2.2. Let $R_2(a',v)=(a,v')$. 
from Lemma \ref{lem:vconst} $A(a',v')=a'$, so $R_2(a',v')=(a',v)$, due to Fact~\ref{wn2}.
%CASE 6.2.2.1. 
%Assume that $R_2(a,v')=(a',v')$. Then we may swap $v$ with $v'$ in order to obtain 
If we had $R_2(a,v')=(a',v')$, then by symmetry we could swap $v$ with $v'$ and obtain Case A. Hence $R_2(a,v')  \neq (a',v')$. 
%CASE 6.2.1.3.1., so by CASE 2. $V(a,v')=v$.\\
Due to Fact~\ref{wn2}, we get $V(a,v')=v$. 
%--------------------------------------------------------
%Let $P(a,v)=p$ and $P(a',v)=q$. Then, from Lemma \ref{lem:ports} either $P(a,v')=p$ or $q=p \land P(a,v')=p'$. However, in both cases, by the Lemma \ref{lem:ports} once again we may obtain $R_2(a,v')=(a,v)$.\\
%%Hence we provide two possible algorithms in this arrangement:\\
%%I.2.1 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p')$,$R_3(a',v')=(a,v,p')$,$R_3(a,v')=(a,v,p)$\\
%%KONTRPRZYKLAD\\
%%I.2.2 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p)$,$R_3(a',v')=(a,v,p)$,$R_3(a,v')=(a,v,p')$\\
%%KONTRPRZYKLAD\\
%----------------------------
%Let $P(a,v)=p$. Realize that then $(\exists\;(x,v')\in S)(\exists\; y\in Vs)\;R_3(x,v')=(a',y,p')$.\\
%Indeed, if $P(a',v')=p$, then we may arrange
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow}(a',v)~,
%$$
%where after leaving the $(a,v)$ we won't change its vertex' state until we enter it with the agent's state $a'$ through port $p'$, so then $R_3(a,v')=(a',y,p')$ for some $y$.\\
%-----------------------------------------
%CASE 6.2.2.2. 
%Assume that we have $R_2(a,v')=(a',v)$ and 
Denote $P(a,v)=p$ and $P(a',v)=q$ and due to Fact \ref{wn5} $P(a',v)\neq P(a',v')$ hence $P(a',v')=q'$.
%CASE 6.2.2.2.1.
%If $P(a,v')=p$, then on the following gadget:
%$$
%(a,v)\stackrel{p\; q}{\leftrightarrow} (a',v)\stackrel{q'\; q'}{\leftrightarrow} (a',v) \stackrel{q\; p}{\leftrightarrow} %(a,v)~,
%$$
Consider the following gadget:
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (2,0) {$*$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (C) at (3,0) {$*$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (D) at (4,0) {$v$};
 \path 	(A) edge [above, bend left] node {$p$} (B)
		(B) edge [above, bend left] node {$q'$} (C)
	        (C) edge [above, bend left] node {$q$} (D);
  \path	(D) edge [below, bend left] node {$p$} (C) 
  		(C) edge [below, bend left] node {$q'$} (B)
	        (B) edge [below, bend left] node {$q$} (A);
\end{tikzpicture}\\
\end{center}
If the agent starts in state $a$ it is initialized on one of the outer vertices and otherwise on one of the inner vertices. 
%In order to escape from this gadget, the agent has to enter to one of the outer vertices in state $a'$, since otherwise it exits via port $p$ without changing the state of the vertex. 
Consider the following three invariants: 
\begin{itemize}
\item[I1] The agent visits the inner vertices always in state $a'$.
\item[I2] The agent visits the outer vertices always in state $a$.
\item[I3] The state of the outer vertices is always $v$.
\end{itemize}
Notice, that as long as the invariants are not violated, the agent cannot escape the gadget because it always exits via port $p$ from the outer vertices. Observe, that the invariants are initially true and assume that all three invariants were true up to some step $t$. We want to show that the invariants will remain true after this step. The agent cannot violate I3 in step $t+1$ because to change the state of an outer vertex from $v$ to $v'$, it has to visit this vertex in state $a'$ so it has to violate I2 before. But since $R_3(a',v')= (a',v,q')$ and $R_3(a',v) = (a,v',q)$ hence if the agent is in state $a'$ in one of the inner vertices it either takes port $q'$ (and moves to the other inner vertex) or it changes its state to $a$. Hence the agent also cannot violate I2 in step $t+1$ because in order to enter to the outer vertices in state $a'$ it had to be in state $a$ in one of the inner vertices thus it had to violate I1 before that. As long as invariants I2 and I3 are not violated, the agent always enters to inner vertices from outer vertices in state $a'$. Moreover if the agent is in state $a'$ in the inner vertex it either keeps its state $a'$ or moves to an outer vertex. Hence the agent cannot violate I1 before I2 and I3. This means that the agent cannot violate any of the invariants hence it cannot escape the gadget. This completes the proof of Case B.


%In order to do so, the state of the agent has to be in state $a'$ $x$. This means that in the pervious 
% However it can only be obtained from the agent's state $a$, so $p=q$. Now, consider the step $x-1$. Then one of the middle vertices has to be entered either from boundary node $(a,v)$ by port $p$ with agent's state $a'$ or by port $q'=p'$, from the state $(a',v')$, with the agent's state $a'$ as well, what contradictes that agent's state before step $x-1$ is $a$.\\
%CASE 6.2.2.2.2. Hence $P(a,v')=p'$.\\
%CASE 6.2.2.2.2.1 Let $q=p$.\\

%\subparagraph{5A. (6.2.3.2.2)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
%    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p$} (m-2-1);
%    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
%    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
% \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
% \path (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p'$} (C)
%	  (C) edge [above, bend left] node {$p$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p'$} (B)
%	  (B) edge [below, bend left] node {$p$} (A)
%	  (A) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
%  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
%  \node (Y) at (6,0) { };
% \path (AA) edge [above, bend left] node {$p$} (A) 
% 	 (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p'$} (C)
%	  (C) edge [above, bend left] node {$p$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p'$} (B)
%	  (B) edge [below, bend left] node {$p$} (A)
%	  (A) edge [below, bend left] node {$p'$} (AA)
%	  (AA) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\end{minipage}
%\end{center}
%
%CASE 6.2.2.2.2.2. Let $q=p'$.\\
%
%\subparagraph{5B. (6.2.3.2.2)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
%    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
%    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
%    \draw[->] (m-2-2) edge node [right, near start] {$p$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
% \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
% \path (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p$} (C)
%	  (C) edge [above, bend left] node {$p'$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p$} (B)
%	  (B) edge [below, bend left] node {$p'$} (A)
%	  (A) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
%  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
%  \node (Y) at (6,0) { };
% \path (AA) edge [above, bend left] node {$p'$} (A)  
% 	 (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p$} (C)
%	  (C) edge [above, bend left] node {$p'$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p$} (B)
%	  (B) edge [below, bend left] node {$p'$} (A)
%	  (A) edge [below, bend left] node {$p'$} (AA)
%	  (AA) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}
%\end{minipage}
%\end{center}
%
%CASE 6.2.2.3. Let $R_2(a,v')=(a,v)$. \\
%CASE 6.2.2.3.1. Let $P(a',v')=p$. Realize that the agent's state $a'$ can be obtained only from the states $(a,v)$ and $(a',v')$, so it can be only obtained via port $p$. Then the sequence
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow} (a',v)\stackrel{p\; p}{\leftrightarrow} (a',v) \stackrel{p'\; p}{\leftrightarrow} (a,v)~
%$$
%\begin{center}
%\begin{tikzpicture}[->]
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
% \path 	(Z) edge [above, bend left] node {$p$} (A)
%		(A) edge [above, bend left] node {$p$} (B)
%	        (B) edge [above, bend left] node {$p'$} (C);
%  \path	(C) edge [below, bend left] node {$p$} (B) 
%  		(B) edge [below, bend left] node {$p$} (A)
%	        (A) edge [below, bend left] node {$p'$} (Z);
%\end{tikzpicture}\\
%\end{center}
%
%provides a loop, because agent cannot change neither agent's state nor vertex' states at both ends.\\
%CASE 6.2.2.3.2. Hence $P(a',v')=p'$.\\
%CASE 6.2.2.3.2.1. If $P(a',v)=p'$, then $P(a,v')=p$ from Lemma \ref{lem:ports}\\
%
%\subparagraph{6. (6.2.4.2.1)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
%    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
%    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
%    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
% \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
% \path (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p'$} (C)
%	  (C) edge [above, bend left] node {$p$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p'$} (B)
%	  (B) edge [below, bend left] node {$p$} (A)
%	  (A) edge [below, bend left] node {$p'$} (X);
%\end{tikzpicture}
%\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
%  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v'$};
%  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
%  \node (Y) at (6,0) { };
% \path  (AA) edge [above, bend left] node {$p'$} (A) 
%           (A) edge [above, bend left] node {$p$} (B)
%	  (B) edge [above, bend left] node {$p'$} (C)
%	  (C) edge [above, bend left] node {$p$} (D)
%	  (D) edge [above, bend left] node {$p'$} (Y);
%  \path (D) edge [below, bend left] node {$p$} (C)
%	  (C) edge [below, bend left] node {$p'$} (B)
%	  (B) edge [below, bend left] node {$p$} (A)
%	  (A) edge [below, bend left] node {$p'$} (AA)
%	  (AA) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}
%\end{minipage}
%\end{center}
%
%CASE 6.2.2.3.2.2. Let $P(a',v)=p$.
%Then the sequence
%$$
%(a,v)\stackrel{p\; p}{\leftrightarrow} (a',v)\stackrel{p'\; p'}{\leftrightarrow} (a',v) \stackrel{p\; p}{\leftrightarrow} (a,v)~
%$$ 
%\begin{center}
%\begin{tikzpicture}[->]
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
% \path 	(Z) edge [above, bend left] node {$p$} (A)
%		(A) edge [above, bend left] node {$p'$} (B)
%	        (B) edge [above, bend left] node {$p$} (C);
%  \path	(C) edge [below, bend left] node {$p$} (B) 
%  		(B) edge [below, bend left] node {$p'$} (A)
%	        (A) edge [below, bend left] node {$p$} (Z);
%\end{tikzpicture}\\
%\end{center}
%
%
%provides the loop. Indeed, in order to change either of the boundary states, the agent needs to use the port $p$ with agent's state $a'$, while entering them. It is only possible, if he goes from the inner vertex of state $(a,v)$. As soon as, he cannot enter the middle vertex by port $p$ with agent's state $a$ (because $A(a,v)=a'$), so the agent has to enter it via $p'$, so $P(a,v')=p'$ and $(a,v')$ had to be a state of the other middle vertex. Recursively, we may prove that at least one of the middle states has to be initated with agent's state $a$, which is not true.\\
\end{proof}
\paragraph{Algorithms $X$ and $Y$}
Consider the following two algorithms:

\begin{center}
\begin{minipage}{.4\textwidth}
\textbf{Algorithm\hspace*{1mm}$X$}
\linebreak
%\subparagraph{7. (7.1.1.1)}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\textbf{Algorithm\hspace*{1mm}$Y$}
\linebreak
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
    \draw[->,bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [right, very near start] {$p$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\end{center}

\begin{lem}
Algorithms $X$ and $Y$ require time $\Omega(n^2)$ to explore a path.
\end{lem}
\begin{proof}

To wytlumaczenie jest dobre dla algorytmow 7. i 8.\\
---------------------------------------------------\\
Realize that agent's state determines the outport, because $P(a,.)=p$ and $P(a',.)=p'$ and moreover
\begin{equation}
\label{prop2}
(\forall\; v\in\Vs)(\forall\; a\in\As)(\exists\; b\in\As)\; R_2(a,v)=(b,v')\land R_2(a,v')=(b',v)~.
\end{equation}
We will show that the adversary is able to force the agent to move according to a sequence decomposed into blocks LR, RL, LRL and RLR where L denotes a move via the left port and R --- a move through the right port. Moreover, assume that after executing the block RL, the next move is L and that after LR, the next block starts with R.\\
Realize that the adversary can establish any starting port (we assume that both ports are available, so the node is not an endpoint of the line structure), so without a loss of generality, let us assume that it will be R. The algorithm is deterministic, so the adversary can choose a vertex' state and outports at the moment of the first visit of a node.
Moreover, assume that adversary established the outports and initial vertices in such the arrangement, that after the agent enters a new node (not yet visited), he has to use the move in the opposite direction in next two consecutive moves (so he uses either RL or LR block).
It is always possible. Indeed, consider a situation that the agent uses R (or alternatively L) with the state $(b,w)$ and enters the new node, with some agent's state $c$. The vertex' state of the left node is then $w'$. The next move will be performed via port determined by $c$ (let $r=P(c,.)$). We wants the agent to go L, so adversary defines the left outport as $r$. Because the agent's state determines the outport and the adversary wants the agent to go L again, so the next time the agent will be in the left node, it should have the opposite agent's state, i.e. $b'$. However, by (\ref{prop2}), there exists such $u$ that $R_3(c,u)=(b',u',r)$. Hence the RL is possible in such the situation. Hence, in this situation RL changes the states from
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (?,u)~
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw,double, circle, text width=.5em, text height=0.5em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$?$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}

to
$$
\stackrel{?\;\;q'}{\leftrightarrow}\underline{(b',w')}\stackrel{q\;\;r}{\leftrightarrow} (c,u')~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=0.6em, label=$ $] (Z) at (1,0) {$ $};
 \node [draw, double, circle, text width=.5em, text height=0.6em, label=$b'$] (A) at (2,0) {$w'$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$c$] (B) at (3,0) {$u'$};
 \path 	(Z) edge [above, bend left] node {$?$} (A)
		(A) edge [above, bend left] node {$q$} (B);
  \path	(B) edge [below, bend left] node {$r$} (A) 
  		(A) edge [below, bend left] node {$q'$} (Z);
\end{tikzpicture}\\
\end{center}

If the new node is discovered by L move, then by the symmetry gives the same possibility by the block LR. Obviously either RL or LR is the starting block of the algorithm (there is only one visited node).\\
Now consider a situation that at some moment the agent performs a block RLR as beneath:
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (c,u)~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw,double, circle, text width=.6em, text height=.6em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.6em, text height=.6em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
Realize that both R moves are performed via outport $q$ and agent's state determines the outport, so after move L, the agent's state has to be $b$ as well.\\
Note that the right node have been visited, because otherwise the block RL should be performed. Let $c$ be the last agent's state used in the right node. Thence $P(c,.)=r$ and $P(c',.)=r'$.
Realize that $A(b,w)=c$, because otherwise $P(c',.)=r$. Before the last move of block RLR, the state of left node will be thence $(b,w')$ and the vertex state of the right node will be $u'$, because after the first move of the block RLR, a situation will be as follows:
$$
(b,w')\stackrel{q\;\;r}{\leftrightarrow} \underline{(c,u)}~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=.6em, label=$b$] (Z) at (1,0) {$w'$};
 \node [draw, double, circle, text width=.6em, text height=.6em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
However we know that $A(b,w)=c$, so by (\ref{prop2}), $A(b,w')=c'$. Moreover $P(c',.)=r'$, so after the block RLR, the states will be as follows:
$$
(b,w)\stackrel{q\;\;r}{\leftrightarrow} \underline{(c',u')}\stackrel{r'\;\;?}{\leftrightarrow}~.
$$
That proves that after the block RLR, the next move will be R as well. Symmetrically for LRL.\\

Consider that we only use blocks from the set $Bl:=\{RL, LR, RLR, LRL\}$.
Note that if the block ends by some move, then the next will starts with the same move. Moreover the ending node of any of theses blocks was visited before the execution of this block. We are able to determine the last agent's state for any visited node. Realize that both the last agent's state and vertex state of ending node of any block change. Moreover, both RLR and LRL do not change states of any other nodes. However, RL and LR changes the vertex' state of new node and determines the last agent's state used of this new node and do not change states of any other nodes. Nevertheless, as the vertex state of the new node is used for a first time, we may think that it is determined by this block as well.
It also worth to mention that moves from the block RL change the states in the same way as the two last moves of the block LRL (symmetrically for LR and two last steps of RLR).  

Now we would like to show that the algorithm can be decomposed in blocks from the set $Bl$ (exluding the last block which will be a single move), i.e. the new block cannot start with the same two moves (RR or LL). As said before, the first block of the algorithm is either RL or LR. Assume that agent performed only some number of blocks from the set $Bl$ and
assume that after these moves we have the situation as beneath:
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (c,u)\stackrel{r'\;\;s}{\leftrightarrow}(d,x)
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, double, circle, text width=.6em, text height=0.6em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.5em, text height=0.6em, label=$c$] (A) at (2,0) {$u$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$d$] (B) at (3,0) {$x$};
 \path 	(Z) edge [above, bend left] node {$q$} (A)
		(A) edge [above, bend left] node {$r'$} (B);
  \path	(B) edge [below, bend left] node {$s$} (A) 
  		(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}

and moreover the agent wants to take two consecutive moves R. As this is the beginning of the new block, thence the last move had to be R as well, so the previous block ended with the sequence LR (either block LR or RLR was used). Realize that $(c,u)$ had to be visited yet, because otherwise RL will be performed. Moreover $P(c,.)=r$ and $P(c',.)=r'$, so $A(b,w)=c'$. Two moves before the potential new block, the situation was as follows:
$$
(e,y)\stackrel{t\;\;q'}{\leftrightarrow}\underline{(b',w')}\stackrel{q\;\;r}{\leftrightarrow} (c,u)\stackrel{r'\;\;s}{\leftrightarrow}(d,x)~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=0.6em, label=$e$] (Z) at (1,0) {$y$};
 \node [draw, double, circle, text width=.5em, text height=0.6em, label=$b'$] (A) at (2,0) {$w'$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$c'$] (B) at (3,0) {$u$};
  \node [draw, circle, text width=.6em, text height=0.6em, label=$d$] (C) at (4,0) {$x$};
 \path 	(Z) edge [above, bend left] node {$t$} (A)
		(A) edge [above, bend left] node {$q$} (B)
	        (B) edge [above, bend left] node {$r'$} (C);
  \path	(C) edge [below, bend left] node {$s$} (B) 
  		(B) edge [below, bend left] node {$r$} (A)
	        (A) edge [below, bend left] node {$q'$} (Z);
\end{tikzpicture}\\
\end{center}

That means that the highlighted node was visited before. However the last visit of this node was not be the first one, because both $(e,y)$ and $(c,u)$ were visited and if the not visited node has two neighbours, then at least one of them is unvisted as well. Hence the last change of the states of highlighted node was when it was an end node of some block. This block ended with L (because $P(b',.)=q'$). This block was not be RL, because $(c,u)$ was visited before, so it was LRL. However before this block we had  the beneath situation:
$$
(b,w)\stackrel{q\;\;r}{\leftrightarrow} \underline{(c,u)}~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
A block LRL does not change the last agent's state of the left node, so $A(c,u)=b$. and $A(b,w)=c$, The last move of the block LRL has to be via outport $r$ and $P(c,.)=r$, so $A(b,w)=c$, contrary to the previous observation.\\
A symmetric situation holds if the agent wants to start a new block by LL.\\

Now we would like to estimate the number of moves needed to explore the graph by this algorithm.
Realize that after RL, LRL is performed until the next new node is found by a block LR. Symmetrically with swapped R and L.
Let say that the line has $n$ nodes. Then the adversary may put the agent in the middle of the line in such the way that, so the agent has to performs $n-2$ RL or LR blocks. After every block RL (or LR), there is one more visited node, so the number of RLR (or LRL) blocks that has to be executed before performing the next RL (or LR) block increases by $1$. The last number of consecutive LRL or RLR blocks is $n-2$ (because the last move is a single one), so the agent has to perform at least
$$
2(n-2)+1+\sum_{i=1}^{n-2}3i=\frac{(n-2)(3n+1)}{2}+1=\Omega(n^2)
$$
moves in order to explore the graph. It worths to note that it is approximately $3$ times longer than RR algorithm.
%Realize that when the agent enters a new node, then we use blocks RL and LR, which works the same as when visiting a new node in RR algorithm. When RR is used when agent enters the already visited node, then 

%The vertex' state change every step, thence after the first R, $(b,w)$ changes to $(b,w')$ and $P(b,w)=q$.\\
%After L we may either have agent's state $b$ or $b'$, but the vertex state will be $w'$ and we have to use the outport $q$.
%
%There exists an automorphism of the transition graph is that swaps $a$ and $a'$, so we may assume that the initial agent's state is $a$. Realize that for any $a_1,a_2$, there exists $v$ such that $A(a_1,v)=a_2$.  Imagine that the agent enters some node for the first time, with the agent's state $a_1$. Assume that the agent's state in the previous move was $a_2'$. The adversary wants to turn back the agent and let him go the opposite direction. However the agent's state determines the outport, so he has to change the agent's state to $a_2$. From the previous observation, we are able to do so, by choosing the appropriate vertex' state. Realize that $a_1$ determines the outport, so the appropriate port should be directed to the previous node. Hence, when the agent is entering a new node, he has to turn around, so he goes one step forward turn around and go back with the opposite orientation --- denote this sequence of moves by FB.
%Assume that otherwise (when he does not enter a new node), the agent make a sequence of moves: forward, back and forward (call it FBF).
%Assume that all the nodes are indexed with consecutive natural numbers from left to right and the starting position has the index $x$.
%We may say, that the virtual state of agent is the tuple (node index, the orientation ($L$ or $R$), leftmost visited node, rightmost visited node). Hence for $c<y<d$, $(y,L,y,d)\stackrel{FB}{\rightarrow}(y,R,y-1,d)$, $(y,R,c,y)\stackrel{FB}{\rightarrow}(y,L,c,y+1)$, $(y,R,c,d)\stackrel{FBF}{\rightarrow}(y+1,R,c,d)$ and $(y,L,c,d)\stackrel{FBF}{\rightarrow}(y-1,L,c,d)$.
%Realize that the definition of the chosen vertices' states and direction of ports approves the virtual states transitions for the move FB. We have to prove that the virtual states transitions are also true for moves of FBF type.
%POKAZAC, ze gdy uzywamy ktoregos portu po raz drugi(w danym nodzie), to musielismy byc w tym samym stanie.
%Assume that the agent moved according to FB and FBF moves to some virtual state $(y,L,c,d)$, for $c<y<d$. If $y=c+1$, then the agent has to move to the node $c$, which is visited again. Realize that, when we visit 
%After the first step, agent meets a new node with state $v'$ and with agent's state $a'$, but $P(a',v')=p'$, so he rotates and goes the step forward. Realize that the vertices' states in $x$ and $x+1$ has been already changed.\\
-------------------------------------\\

\end{proof}
%
%\subparagraph{8. (7.1.1.2.2)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
%    \draw[->,bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
%    \draw[->,bend left] (m-2-1) edge node [right, very near start] {$p$} (m-1-2);
%    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%TODO
%\end{minipage}
%\end{center}


\begin{lem}
\label{lem:threeports}
Assume we have:
\begin{enumerate}
\item $\forall a \in \As$ $V(a,v) = v'$ and $V(a,v') = v$,
\item function $P(s) = P(s') = P(s'')$ for three different state values $s, s',s'' \in S$,
\end{enumerate}
then such an algorithm requires in the worst case $\Omega(n^2)$ steps to explore a path.
\end{lem}
\begin{proof}
Set $S$ has $4$ values so if function $P$ returns the same port for all of them then the algorithm cannot explore all paths of length $>2$. 

Assume that for some $a \in \As$, $v\in \Vs$ and $p\in \Ps$, we have $P(a,v) = p$ and $P(s) = p'$ for $s \neq (a,v)$. Let us construct a path $\mathcal{P} = (v_1,v_2,\dots, v_n)$ of length $n$ such that a port from $v_i$ to $v_{i+1}$ is always $p$ (and port from $v_{i}$ to $v_{i-1}$ is $p'$). Let $v_1$ be the starting position of the agent and let $v'$ be the initial state of each vertex and consider the exploration time of such an agent on such a path.

To prove the time complexity, we show the following: \\
\textit{Claim: For any $i \in 2,3,\dots n-1$, between first visit to $v_i$ and $v_{i+1}$, the agent visits node $v_1$. }\\
To prove the claim observe that, when entering $v_i$ for the first time, the last exit from each vertex $v_2,v_3,\dots,v_{i-1}$ was  via port $p$.  This means that the state of each of these nodes is $v'$ (it is because $V(a,v) = v'$). Since the state of $v_i,v_{i-1},\dots,v_2$ is $v'$, and the agent is at $v_i$, the agent leaves each of these vertices via port $p'$ and walks straight to node $v_1$. This completes the proof of the claim. \\

The lemma is a direct consequence of the claim, because time to explore the whole path is at least $2 \cdot \sum_{i=1}^{n-2} i \in \Omega(n^2)$.

\end{proof}


We are ready to complete the proof of Theorem~\ref{ref:thm}
\begin{proof}{(of Theorem~\ref{ref:thm})}
From Lemma~\ref{fact:1} we know that the state of the agent is not changed during every step at the nodes with degree $2$. By Lemma~\ref{lem:vchange} the state of a vertex is flipped by the agent upon each visit to the vertex. If the ouport chosen by the agent is determined solely based on the state of the vertex then such algorithm would be equivalentto Rotor-Router (on vertices with degree $2$) hence would require time $\Omega(n^2)$. Consider the remaining possible algorithms.
%CASE 7. Assume that the state of vertex changes on every step, but state of agent is not and the outport is not defined only by vertex' state. \\
%Then either exists $a$ such that $P(a,v)=P(a,v')$ or $P(a,v)=P(a',v')$ and $P(a',v)=P(a,v')$.\\
%TO JEST CALY DUZY PRZYPADEK DO ROZPATRZENIA

%CASE 7.1. 

Assume that the outport is defined by the state of the agent i.e.
$$
(\exists\; p \in \Ps)(\forall\; v\in \Vs)\; P(a,v)=p \land P(a',v)=p'~.
$$
CASE 7.1.1. Let $A(a,v)=a$. Then $R_3(a,v)=(a,v',p)$ and because of CASE 4. we obtain $R_3(a,v')=(a',v,p)$.\\
CASE 7.1.1.1. Let $A(a',v)=a'$. Then similarily $R_3(a',v)=(a',v',p')$ and $R_3(a',v')=(a,v,p')$.\\


CASE 7.1.1.2. If $A(a',v)=a$, then $R_3(a',v)=(a,v',p')$.\\
CASE 7.1.1.2.1. Let $A(a',v')=a$. Then $R_3(a',v')=(a,v,p')$, so everytime the agent's state is $a'$, the outport $p'$ is used and the state is changed to $a$, so the outport during the next step will be $p$, so
$$
A\stackrel{p\; p'}{\leftrightarrow}(a,.)\stackrel{p\; p}{\leftrightarrow}(a',.)\stackrel{p'\; p}{\leftrightarrow}B
$$
provides a loop.\\
CASE 7.1.1.2.2. If $A(a',v')=a'$, then $R_3(a',v')=(a',v,p')$.\\
%
%\subparagraph{8. (7.1.1.2.2)}
%\begin{center}
%\begin{minipage}{.4\textwidth}
%\begin{tikzpicture}
%  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
%  {
%    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
%     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
%     };
%    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
%    \draw[->,bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
%    \draw[->,bend left] (m-2-1) edge node [right, very near start] {$p$} (m-1-2);
%    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
%\end{tikzpicture}
%\end{minipage}
%\begin{minipage}{.4\textwidth}
%TODO
%\end{minipage}
%\end{center}


CASE 7.1.2. If $(\forall\; (a,v)\in S)\; A(a,v)=a'$, then we obtain CASE 6.1.\\
%$A(a,v)=a'$. Then $R_2(a,v)=(a',v')$.
%Case II.1. $A(a',v')=a$. Then $R_2(a',v')=(a,v)$. Realize that the actual situation is symmetric with respect to agent's state, so we are going to consider two cases:
%Case II.1.1. If $A(a,v')\neq A(a',v)$, then the transition graph is equivalent with this from the case I.2.2.
%Case II.1.2. If $A(a,v')=A(a',v)$, then the transition graph is equivalent with this from the case I.2.1.
%Case II.2. $A(a',v')=a'$, so $R_2(a',v')=(a',v)$. Then $R_2(a',v)=(a,v')$, because otherwise $a'=A(a',v)=A(a',v')$.
%Case II.2.1 If $A(a,v')=a$, then the transition graph is equivalent with this from the case I.1.
%Case II.2.2 If $A(a,v')=a'$, then the transition graph is equivalent with this from the case I.2.1.
CASE 7.2. Assume that 
\begin{equation}
\label{property}
(\forall\; p\in\Ps)(\forall\; a\in \As)(\exists\; v\in\Vs)\; P(a,v)=p~.
\end{equation}
Due to Fact \ref{wn1} we may assume that $R_3(a,v)=(a',v',p)$.\\
CASE 7.2.1. Let $A(a',v)=a'$, so because the vertex state does not determines the outport and (\ref{property}), we attain $R_3(a',v)=(a',v',p')$. Then also $R_3(a',v')=(a,v,p)$, because of (\ref{property})and CASE 4. Moreover, the agent's state is not determined by the vertex state, so again from (\ref{property}) we get $R_3(a,v')=(a',v,p')$.\\

\subparagraph{10. (7.2.3)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[bend left] (m-1-1) edge node [above, very near start] {$p$} (m-2-2);
    \draw (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw (m-2-1) edge node [left,near start] {$p'$} (m-1-2);
    \draw[bend left] (m-2-2) edge node [below, very near start] {$p$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    \node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      \node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  \node (Y) at (7,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (E)
	  (E) edge [above, bend left] node {$p$} (F)
	  (F) edge [above, bend left] node {$p$} (Y);
  \path (F) edge [below, bend left] node {$p'$} (E)
           (E) edge [below, bend left] node {$p'$} (D)
  	  (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    \node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      \node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  \node (Y) at (7,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (E)
	  (E) edge [above, bend left] node {$p$} (F)
	  (F) edge [above, bend left] node {$p$} (Y);
  \path (F) edge [below, bend left] node {$p'$} (E)
           (E) edge [below, bend left] node {$p'$} (D)
  	  (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 7.2.2. Assume that $A(a',v)=a$, so $R_3(a',v)=(a,v',p')$ from (\ref{property}).\\
CASE 7.2.2.1. Let $A(a',v')=a$. Then $R_3(a',v')=(a,v,p)$ by (\ref{property}). However, if we swap $v$ with $v'$, then we will get CASE 7.2.1.\\
CASE 7.2.2.2. Hence from (\ref{property}), $R_3(a',v')=(a',v,p)$.\\
Note that $R_3(a',v)=(a,v',p')$, so if we swap all the vertex states, agent's states and outports, then we obtain CASE 7.2. However, $A(a,v)=a'$, so we get CASE 7.2.2. But from CASE 7.2.2.1. $A(a,v')\neq a'$, so together with (ref{property}) we finally get $R_3(a,v')=(a,v,p')$.\\

\subparagraph{13. (7.2.6)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw  (m-2-1) edge node [left, near start] {$p'$} (m-1-1);
    \draw (m-2-2) edge node [right, near start] {$p$} (m-1-2);
    \draw (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
    \draw (m-1-1) edge node [below, near start] {$p$} (m-2-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
Algorithm 3 = Rotor-Router
\end{minipage}
\end{center}
 
Realize that the outport of this algorithm determines the agent's state. hence if the adversary put the outports in such a way that only one type of port directs to a node, then the agent will always have the same agent's state in this node. If the adversary do this for all the nodes, then at each node the same will be true. Thence we may think of it as the algorithm without the agent's memory. However the vertex' state change every time it is used, so it is then isomorphic with RR algorithm. Indeed, note that in this case the direction is given not only by vertices' states, but also by the fixed agents' states , which are deteremined by the outports given a priori. Hence for every node, $v$ directs to one direction and $v'$ leads to another, however for different nodes, the same type of vertex may indice different direction.

Thence we only need to show that it is possible to arrange the outports in such the way, that for every node, there is only one type of ports which indice there. However it is simple to realize, that this condition guarantees that if the outports are established  for one node, then the node, which is two places apart has to have the outports defined in opposite way, because it has to indice the opposite direction with the same outport. Moreover there is no possiblity to define the other outports using this restriciton, so me may define outports separately for the nodes which are even places apart the left end of the line and separately for the odd ones.
%If the state of vertex changes on every step and the outport is not defined only by vertex' state and for any port $p$ and any $a\in As$, there exists $v\in Vs$, such that $P(a,v)=p$ and $R_2$ is iniective function, then the algorithm can be reduced to SEA.

%Indeed, assume that $P(a,v)=p$ and $P(a',v)=q$. By the assumptions, then $P(a,v')=p'$ and $P(a',v')=q'$. Assume for a while that $R_2$ is a permutation that consists of one cycle.
%Without a loss of generality we may assume that the agent starts with agent's state $a$ in a $k$-th node, initialized with a state $v$ and that port $p$ directs to $k+1$-th node of the line. The adversary should initialize all vertices as follows:
%the node with index $k+c$ should be initialized by $v$, if $2\not| c$ and by $v'$ for $2|c$; the node with index $k-c$ should be initialize by $v$ if $2|c$ and by $v'$ for $2\not| c$.
%Moreover all the ports should be directed in such the way, that during the first visit, the agent is directed to the previous node.
%TROCHE INACZEJ TO BEDZIE
%NIE WIEM NA ILE TERAZ TO MA SENS

%%%%%%%


CASE 7.3. Assume that
$$
(\exists\; p\in\Ps)(\exists\; a\in \As)(\forall\; v\in \Vs)\; P(a,v)=p~.
$$
Agent's states does not determine the outports and vertex' states always change, so Lemma \ref{lem:ports} guarantees the assumptions of Lemma \ref{lem:threeports} and hence in this case, the algorithm requires $\Omega(n^2)$ steps to explore a path.

\end{proof}
\input{sections/counterexamples}


%%%%%%%

\subsection{unlimited memory}
We consider a model, where $1$ agent tries to explore line topology, where every vertex has some states and number of OutPorts defined by adversary, with no identificators. InPorts and OutPorts does not need to be the same. Also the agent does not have any token that he may take through edges and leave at vertices.

We would like to find some lower bound for complexity of exploration of line graph using a deterministic algorithm. In order to do so, we assume that we are able to save any information in vertices and agent can remember everything he has seen.

For descriptive purpose, let us numerate consecutive vertices by consecutive numbers from $1$ to $n$. Assume that the agent starts the exploration at vertex $1$, so there is only one OutPort, so he can change a state of vertex $1$ to $1$ ($S(1)=1$) and simply traverse to vertex $2$.

Now assume that after some number of steps, the agent is in vertex $k$ and he is aware of all the OutPorts, which can transport him from vertex $1$ to vertex $k$ in $k-1$ consecutive steps and for all $i\leq k$, $S(i)=i$. In such the situation, we say that agent has $k$-progress. Let $OL(i)$ be the number of OutPort, which directs from vertex $i$ to vertex $i-1$, for $i=2,\ldots,n$. Let $OP(i)$ be the number of OutPort, which directs from vertex $i$ to vertex $i+1$, for $i=1,\ldots,n-1$. Realize that, if the agent knows $OL(i)$, then he knows $OP(i)$ and vice versa (if $i\neq 1$ and $i\neq n$).
If he has no $(k+1)$-progress, then he cannot guess $OL(k)$, so we may assume that at vertex $k$ he chooses a port with smaller id. If he will use $OL(k)$, then the state of the next vertex is $k-1$. If the state of the successor is another, then he knows that he went forward to vertex $k+1$ and hence after changing $S(k+1)=k+1$ he has $k+1$-progress.
Further, the agent wants to make a sequence of $\lfloor\sqrt{k}-1\rfloor$ steps using $OL(k-i)$ port at step $i$. If for $i=1,2,\ldots,j-1$, after step $i$, the agent has seen state $k-i-1$ and after step $j$, he sees the state different from $k-j-1$, then that means that, starting from vertex $k$, he has just made $j+1$ steps forward. Hence he can change $S(k+j+1)=k+j+1$ and establish $OL(i)$ for $i=k,k+1,\ldots,k+j$.
 



==> sections/line_intro__Kopia_powoduja__ca_konflikty__uz__ytkownik_Dominik_B__2021-07-05_.tex <==
%line.tex
% !TEX root = ../dual_memory.tex
\newcommand{\As}{\mathrm{As}}
\newcommand{\Vs}{\mathrm{Vs}}
\newcommand{\Ps}{\mathrm{Ps}}

\section{Line topology with dirty memory}

%\subsection{1 bit per agent, 1 bit per vertex}


%It is known that adding more bits of memory on the vertices does not help as time $\Omega(n^2)$ is required even in the model with unlimited memory on each node ~\cite{MencPU17}.
%When exploring a line with a single bit of memory at each node, one use employ the Rotor-router algorithm and achieve exploration time of $O(n^2)$. 
In this section we analyze exploration of a line topology with one bit of memory at each node and one bit of memory at the agent. We show that in this setting, in the \dirtymem model, the exploration of the line requires sometimes $\Omega(n^2)$ steps.

%We want to verify the hypothesis that both types of memory allow for linear time exploration. In this section we provide a partial argument for the contrary -- we show that without additional assumptions such exploration of the line requires in the worst case $\Omega(n^2)$ steps.
%allow the agent to have $1$ bit of memory and we want to answer the question of whether this single bit allows to break the $\Omega(n^2)$ barrier.
\vspace*{2mm}
\customparagraph{Notation}
In the following lower bound on the line, we consider any algorithm working with a single bit at the agent and a single bit at each node. 
We will focus on the actions of the algorithm performed in vertices with degree $2$.
In such vertices, there are four possible inputs to the algorithm $S = \{(0,0),(0,1),(1,0),(1,1)\}$, where in a pair $(a,v)$, $a$ denotes a bit on the agent and $v$ is a bit saved on the vertex. 
Let us denote the agent states by $\As$ and vertex states by $\Vs$. We also use elements from $\Ps=\{0,1\}$ to denote ports in vertices of degree $2$. Morevoer, a shorthand notation $'$ indicates the inverted value of a bit. For example, if $a=0$, then $a'=1$ and vice versa. 

%We denote an entering state as a pair $(a,v)$, where $a$ is a bit on the agent and $v$ is a bit saved on the vertex. At each step at a node with degree $2$, an algorithm has to return some pair $(b,w)$ and port number $p$, depending on the state of the vertex and the state of the agent. Then the agent changes its state to $b$, the state of vertex to $w$ and quits the actual vertex via port $p$. 

%If the vertex is an endpoint of the line, then agent can leave the only by one port. (NIE ANALIZOWALEM JAK SIE ZMIENIA DECYZJA JESLI WIADOMO, ZE TO PUNKT KONCOWY --- TO TRZEBA DODAC)





%The same for vertex' states and ports.

%
%\begin{tikzpicture}[->]
 %\node (X) at (0,0) { };
 %\node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 %\node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    %\node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      %\node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  %\node (Y) at (7,0) { };
 %\path (A) edge [above, bend left] node {$p'$} (B)
	  %(B) edge [above, bend left] node {$p'$} (C)
	  %(C) edge [above, bend left] node {$p'$} (D)
	  %(D) edge [above, bend left] node {$p$} (E)
	  %(E) edge [above, bend left] node {$p$} (F)
	  %(F) edge [above, bend left] node {$p$} (Y);
  %\path (F) edge [below, bend left] node {$p'$} (E)
           %(E) edge [below, bend left] node {$p'$} (D)
  	  %(D) edge [below, bend left] node {$p'$} (C)
	  %(C) edge [below, bend left] node {$p$} (B)
	  %(B) edge [below, bend left] node {$p$} (A)
	  %(A) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}

The goal of this section is to prove the following:
\begin{theorem}
\label{ref:thm}
Any algorithm in the \dirtymem model with one bit at the agent and one bit at each node requires in worst-case time $\Omega(n^2)$ to explore a path.
\end{theorem}

Assume for contradiction, that there exists algorithm $\mathcal{A}$, which explores any path in $o(n^2)$ steps. Without a loss of generality, we may assume that the adversary always sets the agent in the middle point of the path.
For algorithm $\mathcal{A}$, for any $s \in S$, by $A(s), V(s), P(s)$ we denote respectively, the returned agent state, vertex state and the chosen outport in each vertex with degree $2$.
Moreover, we denote $R_3(s):=(A(s),V(s),P(s))$ and $R_2(s):=(A(s),V(s))$.
We will show that $\mathcal{A}$ either falls into infinite loop, works like Rotor-Router algorithm or performs even slower.

A proof of \autoref{ref:thm} is divided naturally in several parts.
In the first one, we concern we provide several properties of potential algorithms $\mathcal{A}$. 
They will be utilized, among others, in the second part, where we will show that the agent does not change its internal state (Lemma~\ref{lem:fact1}), however it has to change the state of the vertex in each step (Lemma~\ref{lem:vchange}).
Further we check two unusual algorithms (called X and Y), which occur to explore the path even slower than the Rotor-Router algorithm (Lemma~\ref{lem:twoAlgs}).
After this we will show that three states of $\mathcal{A}$ cannot return the same outport. 
In the latter part we consider the rest of amenable algorithms, which can either be reduced to previous counterexamples or be fallen into infinite loop.
The proof is very technical, so for the sake of clarity, it is moved to Appendix~\ref{app_line}. 

==> sections/line_old.tex <==
%line.tex
% !TEX root = ../dual_memory.tex
\newcommand{\As}{\mathrm{As}}
\newcommand{\Vs}{\mathrm{Vs}}
\newcommand{\Ps}{\mathrm{Ps}}

\section{Line topology with dirty memory}

\subsection{1 bit per agent, 1 bit per vertex}
A simple round-robin strategy for graph exploration, understood as taking a port different from the previous one on each visit to a vertex of degree $2$, results in exploration time of a path $O(n^2)$. Such a strategy can be clearly implemented with only a single bit at each vertex and zero bits on the agent (if we don't require termination). This strategy can be generalized to arbitrary graphs and such an algorithm, called Rotor-Router works in time $O(mD)$~\cite{YanovskiWB03} for state arbitrary initialization and arbitrary port labelling.
%A classical solution shows that there exists an algorithm, which enables to perform a simple exploration algorithm on a line of size $n$ in $O(n^2)$ steps called Rotor-Router (abbreviated by RR). Every time, when an agent enters a vertex, (excluding two ends of the line) it changes its state to opposite and uses a number of port, which is indicated by this state (every time it enters the opposite port as well).

It is known that adding more bits of memory on the vertices does not help as time $\Omega(n^2)$ is required even in the model with unlimited memory on each node ~\cite{MencPU17}.
In this section  we additionally allow the agent to have $1$ bit of memory and we want to answer the question of whether this single bit allows to break the $\Omega(n^2)$ barrier.

\paragraph{Notation}
In the following lower bound on the line, we take any algorithm working with a single bit at the agent and a single bit at each node. We will focus on the actions of the algorithm in vertices with degree $2$. In such vertices, there are four possible inputs to the algorithm $S = \{(0,0),(0,1),(1,0),(1,1)\}$, where in pair $(a,v)$, $a$ is a bit on the agent and $v$ is a bit saved on the vertex. Let us denote the agent's states by $\As$, vertex' states by $\Vs$ and possible outports by $\Ps$. We use a shorthand notation $'$ to indicate the inverted value of a bit. For example, if $a=0$, then $a'=1$ and vice versa. 


%We denote an entering state as a pair $(a,v)$, where $a$ is a bit on the agent and $v$ is a bit saved on the vertex. At each step at a node with degree $2$, an algorithm has to return some pair $(b,w)$ and port number $p$, depending on the state of the vertex and the state of the agent. Then the agent changes its state to $b$, the state of vertex to $w$ and quits the actual vertex via port $p$. 

%If the vertex is an endpoint of the line, then agent can leave the only by one port. (NIE ANALIZOWALEM JAK SIE ZMIENIA DECYZJA JESLI WIADOMO, ZE TO PUNKT KONCOWY --- TO TRZEBA DODAC)





%The same for vertex' states and ports.

%
%\begin{tikzpicture}[->]
 %\node (X) at (0,0) { };
 %\node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 %\node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    %\node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      %\node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  %\node (Y) at (7,0) { };
 %\path (A) edge [above, bend left] node {$p'$} (B)
	  %(B) edge [above, bend left] node {$p'$} (C)
	  %(C) edge [above, bend left] node {$p'$} (D)
	  %(D) edge [above, bend left] node {$p$} (E)
	  %(E) edge [above, bend left] node {$p$} (F)
	  %(F) edge [above, bend left] node {$p$} (Y);
  %\path (F) edge [below, bend left] node {$p'$} (E)
           %(E) edge [below, bend left] node {$p'$} (D)
  	  %(D) edge [below, bend left] node {$p'$} (C)
	  %(C) edge [below, bend left] node {$p$} (B)
	  %(B) edge [below, bend left] node {$p$} (A)
	  %(A) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}

The goal of this section is to prove the following:
\begin{theorem}
Any algorithm in the model with one bit at the agent and one bit at each node requires in worst-case time $\Omega(n^2)$ to explore a path.
\end{theorem}
Assume for contradiction, that some algorithm $\mathcal{A}$ explores any path in $o(n^2)$ steps. For algorithm $\mathcal{A}$, for any $s \in S$, by $A(s), V(s), P(s)$ we denote respectively, the returned agent state, vertex state and the chosen outport in each vertex with degree $2$. Moreover, we denote $R_3(s):=(A(s),V(s),P(s))$ and $R_2(s):=(A(s),V(s))$. In the following series of facts we will prove some properties that $\mathcal{A}$ has to satisfy. 

\begin{fact}
\label{wn1}
 $(\forall\; a\in \As)(\exists\; v\in \Vs)\; A(a,v)=a'$.
% or the algorithm reduces to RR.
\end{fact}
\begin{proof}
Assume that $(\exists\; a \in \As)(\forall\; v\in \Vs)\; A(a,v)=a$ and let the starting position be the midpoint of the path. If $a$ is the starting state of the agent, then the agent will never change its state before reaching an endpoint of the path. But before that the exploration is not faster than rotor-router, hence there exists an initialization of port numbers, such that reaching the endpoint takes $\Omega(n^2)$ steps. If $a'$ is the starting state, then either $A(a',w)=a$, for some $w \in \Vs$. In this case, the adversary sets $w$ to be the starting state of the starting vertex and from the second step the algorithm explores not faster than the rotor-router hence needs $\Omega(n^2)$ steps to reach an endpoint. Note that if $A(a',w)=a'$ for each $w\in \Vs$, then this reduces to the first case. The obtained contradiction completes the proof of the fact.
\end{proof}

\begin{fact}
\label{wn2}
If $A(a,v)=a$ for some $(a,v) \in S$, then $V(a,v)=v'$.
\end{fact}
\begin{proof}
We will show that otherwise algorithm $\mathcal{A}$ falls into infinite loop for some initial state of the path. Assume that $R_3(a,v) = (a,v,p)$ for some entering state $(a,v)$ and port $p \in \Ps$. Then if $a$ is the starting state, it is easy to see that the agent falls into infinite loop on the following gadget (double circle indicates the starting position of the agent):
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}
If $a'$ is the starting state, then we can use Fact~\ref{wn1}, $(\exists\; w\in \Vs)\;A(a',w)=a$. Let $q = P(a',w)$ (it is possible that $p = q$) and observe that the  agent falls into infinite loop in the following gadget:
%$$
%\underline{(a',w)}\stackrel{q\;p'}{\leftrightarrow}(a,v)\stackrel{p\;p}{\leftrightarrow}(a,v)
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (Z) at (1,0) {$w$};
  \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (3,0) {$v$};
  \node (Y) at (4,0) { };
 \path 	(Z) edge [above, bend left] node {$q$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (Z)
		(Z) edge [below, bend left] node {$q'$} (X);
\end{tikzpicture}\\
\end{center}

%which after first step reduces to the CASE 2.1.\\
%Thanks to the CASE 2. we obtain following results:
\end{proof}

\begin{lem}
\label{lem:vconst}
Fix any $a \in \As$ and $v\in \Vs$. Algorithm $\mathcal{A}$ does \textbf{not} satisfy the following:
\[
%(\forall\;a,x\in \As)(\forall\;v,y,z\in Vs)\;R_2(a,v)=(a',v) \land R_2(a',v)=(x,y)\land R_2(a',v')=(x,z).
R_2(a,v)=(a',v) \land A(a',v) = A(a',v').
\]
%Then the adversary can initialize the algorithm in such the way, to either produce infinite loop either reduce the algorithm to RR.

\end{lem}

\begin{proof}
%CASE 3. 
Assume that the formula holds for some $a \in \As$ and $v\in \Vs$ and we will show that in such a case $\mathcal{A}$ would fall into an infinite loop for some initializations of the path. 
From Fact \ref{wn1}, we obtain, that $A(a',v) = A(a',v') = a$. Denote $P(a,v)=p$ and $V(a',v)= y$.\\
%CASE 3.1. 

If $y=v$, then let $P(a',v)=q$, and the following initial state of the path results in an infinite loop: 
%$\underline{(a,v)}\stackrel{p\;q}{\leftrightarrow}(a',v)$ 
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (Y);
  \path	 (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}

%so only two vertices will be visited.\\
%CASE 3.2. 
In the opposite case, where $y = v'$, the agent would fall into an infinite loop on the following gadget:
%$$
%(a,v)\stackrel{p\;p}{\leftrightarrow}(a',v')\stackrel{p'\;p}{\leftrightarrow}(a,v)~,
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v'$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (3,0) {$v$};
  \node (Y) at (4,0) { };
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (Z)
		(Z) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}

%which leads to infinite loop.\\
We have $R_3(a,v) = (a',v,p)$, hence in the first step, the agent moves to the middle vertex, changes its state to $a'$, and keeps $v$ as the state of the first vertex.
At the middle vertex when the agent's state is $a'$, then it always changes its state to $a$ and moves to one of the outer vertices. But since the outer vertices are both in state $v$, the agent returns to the middle vertex, and so on, which is an infinite loop.
%and, hence we always return to the middle vertex from the entering state $(a,v)$, hence the outer vertices' states won't change as well, so we never visit any of the positions excluding these 3.
\end{proof}

The following fact characterises features of an algorithm, in which some state $a$ of the agent is flipped for both states of a vertex.
\begin{fact}
\label{wn3}
Fix any $a\in\As$. %\marginpar{DB: Wybieramy dowolne a. Ale obydwa fakty dotycza tego samego a; Innymi słowy: jak pewne a spełnia warunek ifa, to zachodza dla niego te dwie wlasnosci. Jesli a' tez spelnia analogiczny warunek z ifa, to dla niego tez beda zachodzily analogiczne wlasnosci z primami przy stanach agentow; To wynika z Lematu 1. dla $a'=a$, $x=a'$, raz przy $v=v$, a raz przy $v=v'$.} 
If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then:
%$(\forall\; w\in \Vs)\; R_2(a',w)\neq(a,w)$ and moreover, from Fact \ref{wn2}, then 
%$(\forall\; w\in \Vs)\; V(a',w)=w'$.
\begin{enumerate}[label=\roman*.,ref=\roman*]
\item\label{fct:31} $(\forall\; w\in \Vs)\; R_2(a',w)\neq(a,w)$,
\item\label{fct:32} $(\forall\; w\in \Vs)\; V(a',w)=w'$,
\item\label{fct:33} $(\exists\; w\in \Vs)\; R_2(a',w)=(a,w')$.
\end{enumerate}
\end{fact}
\begin{proof}
For each $w\in\Vs$, claim~\ref{fct:31} follows from Lemma~\ref{lem:vconst} for $a', w$, and Claim~\ref{fct:32} follows from Fact~\ref{wn2}. Claim~\ref{fct:33} follows from Fact~\ref{wn1} and claims~\ref{fct:31},~\ref{fct:32}.
\end{proof}
%\marginpar{DB: dlatego moze wartop rozbic to na 2 fakty}

%\begin{fact}
%\label{wn4}
%Fix any $a\in\As$. If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then, from facts \ref{wn1} and \ref{wn3}, 
%$(\exists\; w\in \Vs)\; R_2(a',w)=(a,w')$.
%\marginpar{DB: tutaj mogloby byc z faktu 3. tylko $R_2(a',w)=(a,w')$ albo $R_2(a',w)=(a',w')$, ale z faktu 1. musi choc raz zmieniac stan agenta.}
%\end{fact}


\begin{fact}
\label{fac:CASE4}
%CASE 4\dpa{CASE 4 -- to jest do któregoś z faktów?}. 
%Assume that for some $v$, $R_3(a,v)=(a',v,p)$ and $R_3(a',v)=(a,v,q)$. Then $(a',v)\stackrel{q\;p}{\leftrightarrow}(a,v)$ gives the 2-loop.
For any $v \in \Vs$, $R_2(a,v) \neq (a',v)$ or $R_2(a',v) \neq (a,v)$. 
\end{fact}
\begin{proof}
Observe that if we had for some $v$, that $R_3(a,v) = (a',v,p)$ and $R_3(a',v) = (a,v,q)$, for any $p,q \in \Ps$, then the agent would fall into an infinite loop on the following gadget:

%Then $(a',v)\stackrel{q\;p}{\leftrightarrow}(a,v)$ gives the 2-loop.

\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$q'$} (Y);
  \path  (B) edge [below, bend left] node {$q$} (A)
	   (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}
If the agent's starting state is $a$ ($a'$), the adversary chooses its starting position as the right (left) vertex and in both cases the agent never exits from the gadget.

\end{proof}


\begin{lem}
\label{lem:ports}
For any $a\in \As$. If $(\forall\; v\in\Vs)\; P(a,v)=p$, then 
$$
(\exists\; w\in \Vs)\; A(a',w)=a' \land P(a',w)=p'~.
$$
\end{lem}

\begin{proof}
First observe that $(\exists\; w\in \Vs) P(a',w)=p'$, since otherwise the algorithm always takes the same port $p$ in every node with degree $2$. 
%Fix $w^*  \in \Vs$ such that $P(a',w^*) = p'$. 

%CASE 5.1. If all the outports are the same, then there is no way to change the direction, hence 2-loop can be trivially obtained.\\
%CASE 5.2.  
Observe that, if $(\forall\;w\in Vs)\;P(a',w)=p' \Rightarrow A(a',w)=a$, then the agent always changes its state to $a$ after taking port $p'$ and always takes port $p$ in state $a$. Consider the following gadget (where $*$ denotes any vertex state, possibly different at each vertex):

\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (1,0) {$*$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$*$};
 \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$*$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$*$};
  \node (Y) at (5,0) { };
 \path 	(X) edge [above, bend left] node {$p'$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	        (B) edge [above, bend left] node {$p$} (C)
	  	(C) edge [above, bend left] node {$p'$} (D)
		(D) edge [above, bend left] node {$p'$} (Y);
  \path	 (Y) edge [below, bend left] node {$p'$} (D)
	         (D) edge [below, bend left] node {$p$} (C)
		(C) edge [below, bend left] node {$p$} (B)
		(B) edge [below, bend left] node {$p'$} (A)
		(A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}
After entering to any of the outer vertices, the agent is certainly in state $a$ because it can only enter via port $p'$. Hence in the next step it takes port $p$. Thus it cannot exit from such a gadget. We obtain a contradiction, hence the implication cannot be true, which completes the proof of the lemma.


%then we can construct the sequence of ports:
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow}B \stackrel{p\; p}{\leftrightarrow}C\stackrel{p'\; p}{\leftrightarrow} (a,v)~,
%$$
%which blocks the opportunity to change the direction both in A and D.
%Indeed, in order to get to those vertices, we have to use port $p'$, but then the agent's bit changes to $a$. However the adversary initializes terminal positions with vertex's state $v$, then the agent has to use $P(a,v)=p$, so it goes always either to B or C.
\end{proof}
The following Fact is a direct conclusion of Lemma~\ref{lem:ports}.
\begin{fact}
\label{wn5}
If $(\forall\; v\in\Vs)\; A(a',v)=a$, then $P(a,v)\neq P(a,v')$.
\end{fact}
NEW VERSION
--------------------------------------- 
The next two facts ....
\begin{fact}
\label{fact:1}
Fix any $a\in \As$. If $(\forall\;v\in \Vs)\;A(a,v)=a'$, then $(\exists\; w\in \Vs)\;R_2(a',w)=(a,w') \land R_2(a',w')=(a',w)$. % or the algorithm is equivalent with RR.
\end{fact}
\begin{proof}
%CASE 6.1.
By Fact \ref{wn3} we know that $(\exists\; w\in \Vs)\;R_2(a',w)=(a,w')$ and that either $R_2(a',w')=(a',w)$ or $R_2(a',w')=(a,w')$. If the statement of this fact is not correct, then $R_2(a',w')=(a,w')$, which means, that the agent changes its internal state in each step (i.e., $(\forall\; a\in\As)(\forall\; v\in\Vs)\; A(a,v)=a'$).
  By the symmetry and Fact \ref{wn3} we obtain that $(\forall\; a\in\As)(\forall\; v\in\Vs)\; R_2(a,v)=(a',v')$, which means that the vertices' states are changed upon each visit of the agent. We want to show that for such an algorithm:
  \begin{equation}
  \label{eqn:differences}
   (\forall\; a\in\As)(\forall\; v\in\Vs) P(a,v)\neq P(a,v'). 
   \end{equation}
   Assume for contrary that for some $a_1 \in \As,v_1 \in \Vs$ we have $P(a_1,v_1) = P(a_1,v_1') = p$, for some $p \in \Ps$. Observe that in this case, since in every step at a node with degree $2$, the agent changes its state, then out of every two consecutive steps at nodes with degree $2$, at least one is via port $p$. This shows, that on a path, where port $p$ always points towards the starting position of the agent, the agent cannot reach more than $2$ steps away from its starting position, hence it cannot explore the whole path. This completes the proof of Equation~\ref{eqn:differences}.

%Since we are not able to change the agent's bit at entering state of any particular position, then $(\forall\; a\in\As)(\forall\; v\in\Vs) P(a,v)\neq P(a,v')$, because otherwise there won't be possibility to change the direction at some positions, because of parity argument, which blocks the possibility to visit all the vertices.\\


Consider the following two cases:
%CASE 6.1.1. 
if $P(a,v)=P(a',v)$, then, by Equation~\ref{eqn:differences}, $P(a,v')=P(a',v')$, and the outports chosen by the agent depend only on states of vertices (the agent does not use its internal state), hence this algorithm is equivalent to Rotor-Router on vertices with degree $2$, hence it requires $\Omega(n^2)$ steps to explore a path, starting from a vertex in the middle of the path (at distance at least $\lfloor n/2 \rfloor$ from each endpoint).\\
%CASE 6.1.2. 
Otherwise, again from Equation~\ref{eqn:differences} $P(a',v)=P(a,v')$ and $P(a,v)=P(a',v')$. We may think of an equivalence relation, where $(a,v)\equiv(a',v')=W$ and $(a,v')\equiv(a',v)=W'$. Then the outports of $W$ and $W'$ are different. Now, observe, that since the agent changes its internal state at each step, then after an even number of steps on nodes with degree $2$, the agent is always in the same state. Notice, that to return to a some vertex, the agent has to make an even number of steps. Consider an agent starting in the middle of a path and analyze its walk until it reaches some of the endpoints. Between succesive visits to any of the vertices $x$, the agent makes an even number of steps hence the agent always visits $x$ in the same state. Thus upon consecituve visits, it choses different outports. Hence the walk performed by the agent is equivalent to Rotor-Router and for some initialization of port labels it takes $\Omega(n^2)$ steps to reach any endpoint of the path.


We obtained a contradiction in both cases, which proves the fact. 

%Realize that after exit of some position, the vertex state changes, but the future agent's state cannot be another, so it may  be seen as changing the state from $W$ to $W'$ and viceversa. Hence this algorithm is isomorphic with RR.\\
%CASE 6.1 provides the following result:
\end{proof}

\begin{fact}
\label{fact:2}
Fix any $a\in \As$. If $(\exists\;v\in \Vs)\;A(a,v) = a$, then $(\exists\;b\in\As)\; V(b,v)=v$
\end{fact}
\begin{proof}
%CASE 6.2. 
%Assume, that the agent does not change the state of vertex at every step. 



Moreover, from Fact~\ref{fac:CASE4}. and CASE 2. we know that $(\exists\; a\in \As)\; R_2(a,v)=(a',v) \land V(a',v)=v'$.\\
CASE 6.2.1. Assume that $R_2(a',v)=(a',v')$. From Lemma \ref{lem:vconst} we obtain $A(a',v')=a$.\\
CASE 6.2.1.1. Realize that if $P(a,v)=p$, $P(a',v)=q$ and $P(a',v')=q'$, then we can construct a sequence:
$$
(a,v)\stackrel{p\; q'}{\leftrightarrow}(a',v)\stackrel{q\; q}{\leftrightarrow}(a',v)\stackrel{q'\; p}{\leftrightarrow}(a,v)~,
$$

\begin{center}
\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$q$} (B)
	        (B) edge [above, bend left] node {$q'$} (C);
	        %(C) edge [above, bend left] node {$$} (Y);
  \path	(C) edge [below, bend left] node {$q'$} (B) 
  		(B) edge [below, bend left] node {$q$} (A)
	        (A) edge [below, bend left] node {$q'$} (Z);
		%(Z) edge [below, bend left] node {$$} (X);
\end{tikzpicture}\\
\end{center}
so the adversary only has to establish the outports dependent on the initial state of agent. We may briefly realize that agent's states never change in such the arrangement, so there is no possibility to change any of entering states $(a,v)$. \\
\end{proof}

The next lemma is a direct consequence of Facts~\ref{fact:1} and~\ref{fact:2}


%CASE 6. Assume that 
\begin{lem}
$$
(\forall\; a\in\As)\left((\forall\; v\in\Vs) A(a,v)=a' \lor (\exists\;a\in\As)\; V(a,v)=v\right)~.
$$
\end{lem}


% \marginpar{DB: ewentualnie to mozna rozbic na osobne przypadki 6. i 7. zamiast 6.1 i 6.2}

---------------------------OLD VERSION

CASE 6. Assume that 
$$
(\forall\; a\in\As)(\forall\; v\in\Vs) A(a,v)=a' \lor (\exists\;a\in\As)\; V(a,v)=v~.
$$ \marginpar{DB: ewentualnie to mozna rozbic na osobne przypadki 6. i 7. zamiast 6.1 i 6.2}
CASE 6.1. Let the agent changes the agent's bit every round i.e.
$(\forall\; a\in\As)(\forall\; v\in\Vs)\; A(a,v)=a'$. By the symmetry and Fact \ref{wn3} we obtain that $(\forall\; a\in\As)(\forall\; v\in\Vs)\; R_2(a,v)=(a',v')$, so the vertices' states are always changed as well.
Since we are not able to change the agent's bit at entering state of any particular position, then $(\forall\; a\in\As)(\forall\; v\in\Vs) P(a,v)\neq P(a,v')$, because otherewise there won't be possibility to change the direction at some positions, because of parity argument, which blocks the possibility to visit all the vertices.\\
CASE 6.1.1. If $P(a,v)=P(a',v)=p$, then, by Lemma \ref{lem:ports}, $P(a,v')=P(a',v')=p'$, so the outports depends only on vertices and agent's states are useless, hence this algorithm is just RR.\\
CASE 6.1.2. Otherwise, again from Lemma \ref{lem:ports}, $P(a',v)=P(a,v')=p$ and $P(a,v)=P(a',v')=p'$. We may think of an equivalence relation, where $(a,v)\equiv(a',v')=W$ and $(a,v')\equiv(a',v)=W'$. Then the outports of $W$ and $W'$ are different. Realize that after exit of some position, the vertex state changes, but the future agent's state cannot be another, so it may  be seen as changing the state from $W$ to $W'$ and viceversa. Hence this algorithm is isomorphic with RR.\\
CASE 6.1 provides the following result:

\begin{fact}
\label{fact:1}
Let $a\in \As$. If $(\forall\;v\in \Vs)\;A(a,v)=a'$, then either $(\exists\; w\in \Vs)\;R_2(a',w)=(a,w')\land A(a',w')=a'$, so $R_2(a',w')=(a',w)$ or the algorithm is equivalent with RR.
\end{fact}

CASE 6.2. Assume, that the agent does not change the state of vertex at every step. Moreover, from CASE 4. and CASE 2. we know that $(\exists\; a\in \As)\; R_2(a,v)=(a',v) \land V(a',v)=v'$.\\
CASE 6.2.1. Assume that $R_2(a',v)=(a',v')$. From Lemma \ref{lem:vconst} we obtain $A(a',v')=a$.\\
CASE 6.2.1.1. Realize that if $P(a,v)=p$, $P(a',v)=q$ and $P(a',v')=q'$, then we can construct a sequence:
$$
(a,v)\stackrel{p\; q'}{\leftrightarrow}(a',v)\stackrel{q\; q}{\leftrightarrow}(a',v)\stackrel{q'\; p}{\leftrightarrow}(a,v)~,
$$
\begin{center}
\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$q$} (B)
	        (B) edge [above, bend left] node {$q'$} (C);
	        %(C) edge [above, bend left] node {$$} (Y);
  \path	(C) edge [below, bend left] node {$q'$} (B) 
  		(B) edge [below, bend left] node {$q$} (A)
	        (A) edge [below, bend left] node {$q'$} (Z);
		%(Z) edge [below, bend left] node {$$} (X);
\end{tikzpicture}\\
\end{center}
so the adversary only has to establish the outports dependent on the initial state of agent. We may briefly realize that agent's states never change in such the arrangement, so there is no possibility to change any of entering states $(a,v)$. \\

------------------------------------

\paragraph*{Conclusion}
Hence $P(a',v)=P(a',v')$.
Moreover, from Lemma \ref{lem:ports} we obtain that $R_2(a,v')=(a,v)$ and $P(a',v)=P(a',v')\neq P(a,v')$.\\
CASE 6.2.1.2. From Lemma \ref{lem:vconst}, if $R_2(a',v')=(a,v')$, then $A(a,v')=a$, hence, from Fact \ref{wn2}, $R_2(a,v')=(a,v)$. By the same argument as in CASE 6.2. and CASE 6.2.1, we conclude that $P(a,v)=P(a,v')$, hence ports depend only on the agent's state, so by Lemma \ref{lem:ports} we provide the algorithm:\\
$R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p')$,$R_3(a',v')=(a,v',p')$,$R_3(a,v')=(a,v,p)$.\\
\subparagraph{1. (6.1,2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-2-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X)
	  (B) edge [above, bend left] node {$p'$} (Y);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X)
	  (B) edge [above, bend left] node {$p$} (Y);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.1.3. If $R_2(a',v')\neq (a,v')$, then by CASE 2. we obtain $V(a',v')=v$.\\
%CASE 6.2.1.3.1. Let $A(a,v')=a'$.
From the conclusion after CASE 6.2.1.1. we know that 
%From Fact \ref{fact:1} we obtain $R_2(a',v')=(a,v)$. Moreover, realize that $A(a,v')=A(a,v)$, so from Lemma \ref{lem:vconst}, $V(a,v')=v$.
%From Fact \ref{wn5} we obtain that $P(a',v)\neq P(a',v')$.
%However from CASE 6.2.1.1. we have already known that $P(a',v)=P(a',v')$.\\
%CASE 6.2.1.3.2. Hence
$R_2(a,v')=(a,v)$.\\
CASE 6.2.1.3.1. If $R_2(a',v')=(a',v)$, then from Lemma \ref{lem:vconst} the algorithm can be easily looped.\\
CASE 6.2.1.3.2.1. If $R_3(a,v')=(a,v,p)$, then from Lemma \ref{lem:ports} and Conclusion after CASE 6.2.1.1. we attain $R_3(a',v')=(a,v,p')$ and $R_3(a',v)=(a',v',p')$.\\

\subparagraph{2. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-1-1);
\end{tikzpicture}

\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p'$} (A) 
 	  (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}

\end{minipage}
\end{center}

CASE 6.2.1.3.2.2. Let $R_3(a,v')=(a,v,p')$. Then from CASE 6.2.1.1. we know and Lemma \ref{lem:ports} we obtain $R_3(a',v')=(a,v,p)$ and $R_3(a',v)=(a',v',p)$.\\

\subparagraph{3. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p'$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path  (AA) edge [above, bend left] node {$p$} (A) 
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p'$} (X) ;
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2. Let $R_2(a',v)=(a,v')$. From Lemma \ref{lem:vconst} $A(a',v')=a'$, so $R_2(a',v')=(a',v)$, because of CASE 2.\\
CASE 6.2.2.1. Assume that $R_2(a,v')=(a',v')$. Then we may swap $v$ with $v'$ in order to obtain CASE 6.2.1.3.1., so by CASE 2. $V(a,v')=v$.\\
%--------------------------------------------------------
%Let $P(a,v)=p$ and $P(a',v)=q$. Then, from Lemma \ref{lem:ports} either $P(a,v')=p$ or $q=p \land P(a,v')=p'$. However, in both cases, by the Lemma \ref{lem:ports} once again we may obtain $R_2(a,v')=(a,v)$.\\
%%Hence we provide two possible algorithms in this arrangement:\\
%%I.2.1 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p')$,$R_3(a',v')=(a,v,p')$,$R_3(a,v')=(a,v,p)$\\
%%KONTRPRZYKLAD\\
%%I.2.2 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p)$,$R_3(a',v')=(a,v,p)$,$R_3(a,v')=(a,v,p')$\\
%%KONTRPRZYKLAD\\
%----------------------------
%Let $P(a,v)=p$. Realize that then $(\exists\;(x,v')\in S)(\exists\; y\in Vs)\;R_3(x,v')=(a',y,p')$.\\
%Indeed, if $P(a',v')=p$, then we may arrange
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow}(a',v)~,
%$$
%where after leaving the $(a,v)$ we won't change its vertex' state until we enter it with the agent's state $a'$ through port $p'$, so then $R_3(a,v')=(a',y,p')$ for some $y$.\\
%-----------------------------------------
CASE 6.2.2.2. Assume that $R_2(a,v')=(a',v)$ and $P(a,v)=p$.\\
From Fact \ref{wn5} $P(a',v)\neq P(a',v')$. Hence $P(a',v)=q$ and $P(a',v')=q'$.\\
CASE 6.2.2.2.1.
If $P(a,v')=p$, then there is a sequence:
$$
(a,v)\stackrel{p\; q}{\leftrightarrow} (a',v)\stackrel{q'\; q'}{\leftrightarrow} (a',v) \stackrel{q\; p}{\leftrightarrow} (a,v)~,
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$q'$} (B)
	        (B) edge [above, bend left] node {$q$} (C);
  \path	(C) edge [below, bend left] node {$p$} (B) 
  		(B) edge [below, bend left] node {$q'$} (A)
	        (A) edge [below, bend left] node {$q$} (Z);
\end{tikzpicture}\\
\end{center}
where in order to get to one of the bounds, an agent has to use port $q$ at some move $x$. In order to use $p'$ at step $x+1$, he needs to change the agent's state  to $a'$ at step $x$. However it can only be obtained from the agent's state $a$, so $p=q$. Now, consider the step $x-1$. Then one of the middle vertices has to be entered either from boundary node $(a,v)$ by port $p$ with agent's state $a'$ or by port $q'=p'$, from the state $(a',v')$, with the agent's state $a'$ as well, what contradictes that agent's state before step $x-1$ is $a$.\\
CASE 6.2.2.2.2. Hence $P(a,v')=p'$.\\
CASE 6.2.2.2.2.1 Let $q=p$.\\

\subparagraph{5A. (6.2.3.2.2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p$} (A) 
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2.2.2.2. Let $q=p'$.\\

\subparagraph{5B. (6.2.3.2.2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p'$} (A)  
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2.3. Let $R_2(a,v')=(a,v)$. \\
CASE 6.2.2.3.1. Let $P(a',v')=p$. Realize that the agent's state $a'$ can be obtained only from the states $(a,v)$ and $(a',v')$, so it can be only obtained via port $p$. Then the sequence
$$
(a,v)\stackrel{p\; p'}{\leftrightarrow} (a',v)\stackrel{p\; p}{\leftrightarrow} (a',v) \stackrel{p'\; p}{\leftrightarrow} (a,v)~
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	        (B) edge [above, bend left] node {$p'$} (C);
  \path	(C) edge [below, bend left] node {$p$} (B) 
  		(B) edge [below, bend left] node {$p$} (A)
	        (A) edge [below, bend left] node {$p'$} (Z);
\end{tikzpicture}\\
\end{center}

provides a loop, because agent cannot change neither agent's state nor vertex' states at both ends.\\
CASE 6.2.2.3.2. Hence $P(a',v')=p'$.\\
CASE 6.2.2.3.2.1. If $P(a',v)=p'$, then $P(a,v')=p$ from Lemma \ref{lem:ports}\\

\subparagraph{6. (6.2.4.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path  (AA) edge [above, bend left] node {$p'$} (A) 
           (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2.3.2.2. Let $P(a',v)=p$.
Then the sequence
$$
(a,v)\stackrel{p\; p}{\leftrightarrow} (a',v)\stackrel{p'\; p'}{\leftrightarrow} (a',v) \stackrel{p\; p}{\leftrightarrow} (a,v)~
$$ 
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p'$} (B)
	        (B) edge [above, bend left] node {$p$} (C);
  \path	(C) edge [below, bend left] node {$p$} (B) 
  		(B) edge [below, bend left] node {$p'$} (A)
	        (A) edge [below, bend left] node {$p$} (Z);
\end{tikzpicture}\\
\end{center}


provides the loop. Indeed, in order to change either of the boundary states, the agent needs to use the port $p$ with agent's state $a'$, while entering them. It is only possible, if he goes from the inner vertex of state $(a,v)$. As soon as, he cannot enter the middle vertex by port $p$ with agent's state $a$ (because $A(a,v)=a'$), so the agent has to enter it via $p'$, so $P(a,v')=p'$ and $(a,v')$ had to be a state of the other middle vertex. Recursively, we may prove that at least one of the middle states has to be initated with agent's state $a$, which is not true.\\
CASE 7. Assume that the state of vertex changes on every step, but state of agent is not and the outport is not defined only by vertex' state. \\
%Then either exists $a$ such that $P(a,v)=P(a,v')$ or $P(a,v)=P(a',v')$ and $P(a',v)=P(a,v')$.\\
%TO JEST CALY DUZY PRZYPADEK DO ROZPATRZENIA
CASE 7.1. Assume that the outport is defined by the state of the agent i.e.
$$
(\forall\; v\in \Vs)\; P(a,v)=p \land P(a',v)=p'~.
$$
CASE 7.1.1. Let $A(a,v)=a$. Then $R_3(a,v)=(a,v',p)$ and because of CASE 4. we obtain $R_3(a,v')=(a',v,p)$.\\
CASE 7.1.1.1. Let $A(a',v)=a'$. Then similarily $R_3(a',v)=(a',v',p')$ and $R_3(a',v')=(a,v,p')$.\\

\subparagraph{7. (7.1.1.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
Algorithm 2
\end{minipage}
\end{center}

CASE 7.1.1.2. If $A(a',v)=a$, then $R_3(a',v)=(a,v',p')$.\\
CASE 7.1.1.2.1. Let $A(a',v')=a$. Then $R_3(a',v')=(a,v,p')$, so everytime the agent's state is $a'$, the outport $p'$ is used and the state is changed to $a$, so the outport during the next step will be $p$, so
$$
A\stackrel{p\; p'}{\leftrightarrow}(a,.)\stackrel{p\; p}{\leftrightarrow}(a',.)\stackrel{p'\; p}{\leftrightarrow}B
$$
provides a loop.\\
CASE 7.1.1.2.2. If $A(a',v')=a'$, then $R_3(a',v')=(a',v,p')$.\\

\subparagraph{8. (7.1.1.2.2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
    \draw[->,bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [right, very near start] {$p$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
TODO
\end{minipage}
\end{center}

To wytlumaczenie jest dobre dla algorytmow 7. i 8.\\
---------------------------------------------------\\
Realize that agent's state determines the outport, because $P(a,.)=p$ and $P(a',.)=p'$ and moreover
\begin{equation}
\label{prop2}
(\forall\; v\in\Vs)(\forall\; a\in\As)(\exists\; b\in\As)\; R_2(a,v)=(b,v')\land R_2(a,v')=(b',v)~.
\end{equation}
We will show that the adversary is able to force the agent to move according to a sequence decomposed into blocks LR, RL, LRL and RLR where L denotes a move via the left port and R --- a move through the right port. Moreover, assume that after executing the block RL, the next move is L and that after LR, the next block starts with R.\\
Realize that the adversary can establish any starting port (we assume that both ports are available, so the node is not an endpoint of the line structure), so without a loss of generality, let us assume that it will be R. The algorithm is deterministic, so the adversary can choose a vertex' state and outports at the moment of the first visit of a node.
Moreover, assume that adversary established the outports and initial vertices in such the arrangement, that after the agent enters a new node (not yet visited), he has to use the move in the opposite direction in next two consecutive moves (so he uses either RL or LR block).
It is always possible. Indeed, consider a situation that the agent uses R (or alternatively L) with the state $(b,w)$ and enters the new node, with some agent's state $c$. The vertex' state of the left node is then $w'$. The next move will be performed via port determined by $c$ (let $r=P(c,.)$). We wants the agent to go L, so adversary defines the left outport as $r$. Because the agent's state determines the outport and the adversary wants the agent to go L again, so the next time the agent will be in the left node, it should have the opposite agent's state, i.e. $b'$. However, by (\ref{prop2}), there exists such $u$ that $R_3(c,u)=(b',u',r)$. Hence the RL is possible in such the situation. Hence, in this situation RL changes the states from
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (?,u)~
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw,double, circle, text width=.5em, text height=0.5em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$?$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}

to
$$
\stackrel{?\;\;q'}{\leftrightarrow}\underline{(b',w')}\stackrel{q\;\;r}{\leftrightarrow} (c,u')~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=0.6em, label=$$] (Z) at (1,0) {$ $};
 \node [draw, double, circle, text width=.5em, text height=0.6em, label=$b'$] (A) at (2,0) {$w'$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$c$] (B) at (3,0) {$u'$};
 \path 	(Z) edge [above, bend left] node {$?$} (A)
		(A) edge [above, bend left] node {$q$} (B);
  \path	(B) edge [below, bend left] node {$r$} (A) 
  		(A) edge [below, bend left] node {$q'$} (Z);
\end{tikzpicture}\\
\end{center}

If the new node is discovered by L move, then by the symmetry gives the same possibility by the block LR. Obviously either RL or LR is the starting block of the algorithm (there is only one visited node).\\
Now consider a situation that at some moment the agent performs a block RLR as beneath:
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (c,u)~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw,double, circle, text width=.6em, text height=.6em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.6em, text height=.6em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
Realize that both R moves are performed via outport $q$ and agent's state determines the outport, so after move L, the agent's state has to be $b$ as well.\\
Note that the right node have been visited, because otherwise the block RL should be performed. Let $c$ be the last agent's state used in the right node. Thence $P(c,.)=r$ and $P(c',.)=r'$.
Realize that $A(b,w)=c$, because otherwise $P(c',.)=r$. Before the last move of block RLR, the state of left node will be thence $(b,w')$ and the vertex state of the right node will be $u'$, because after the first move of the block RLR, a situation will be as follows:
$$
(b,w')\stackrel{q\;\;r}{\leftrightarrow} \underline{(c,u)}~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=.6em, label=$b$] (Z) at (1,0) {$w'$};
 \node [draw, double, circle, text width=.6em, text height=.6em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
However we know that $A(b,w)=c$, so by (\ref{prop2}), $A(b,w')=c'$. Moreover $P(c',.)=r'$, so after the block RLR, the states will be as follows:
$$
(b,w)\stackrel{q\;\;r}{\leftrightarrow} \underline{(c',u')}\stackrel{r'\;\;?}{\leftrightarrow}~.
$$
That proves that after the block RLR, the next move will be R as well. Symmetrically for LRL.\\

Consider that we only use blocks from the set $Bl:=\{RL, LR, RLR, LRL\}$.
Note that if the block ends by some move, then the next will starts with the same move. Moreover the ending node of any of theses blocks was visited before the execution of this block. We are able to determine the last agent's state for any visited node. Realize that both the last agent's state and vertex state of ending node of any block change. Moreover, both RLR and LRL do not change states of any other nodes. However, RL and LR changes the vertex' state of new node and determines the last agent's state used of this new node and do not change states of any other nodes. Nevertheless, as the vertex state of the new node is used for a first time, we may think that it is determined by this block as well.
It also worth to mention that moves from the block RL change the states in the same way as the two last moves of the block LRL (symmetrically for LR and two last steps of RLR).  

Now we would like to show that the algorithm can be decomposed in blocks from the set $Bl$ (exluding the last block which will be a single move), i.e. the new block cannot start with the same two moves (RR or LL). As said before, the first block of the algorithm is either RL or LR. Assume that agent performed only some number of blocks from the set $Bl$ and
assume that after these moves we have the situation as beneath:
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (c,u)\stackrel{r'\;\;s}{\leftrightarrow}(d,x)
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, double, circle, text width=.6em, text height=0.6em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.5em, text height=0.6em, label=$c$] (A) at (2,0) {$u$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$d$] (B) at (3,0) {$x$};
 \path 	(Z) edge [above, bend left] node {$q$} (A)
		(A) edge [above, bend left] node {$r'$} (B);
  \path	(B) edge [below, bend left] node {$s$} (A) 
  		(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}

and moreover the agent wants to take two consecutive moves R. As this is the beginning of the new block, thence the last move had to be R as well, so the previous block ended with the sequence LR (either block LR or RLR was used). Realize that $(c,u)$ had to be visited yet, because otherwise RL will be performed. Moreover $P(c,.)=r$ and $P(c',.)=r'$, so $A(b,w)=c'$. Two moves before the potential new block, the situation was as follows:
$$
(e,y)\stackrel{t\;\;q'}{\leftrightarrow}\underline{(b',w')}\stackrel{q\;\;r}{\leftrightarrow} (c,u)\stackrel{r'\;\;s}{\leftrightarrow}(d,x)~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=0.6em, label=$e$] (Z) at (1,0) {$y$};
 \node [draw, double, circle, text width=.5em, text height=0.6em, label=$b'$] (A) at (2,0) {$w'$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$c'$] (B) at (3,0) {$u$};
  \node [draw, circle, text width=.6em, text height=0.6em, label=$d$] (C) at (4,0) {$x$};
 \path 	(Z) edge [above, bend left] node {$t$} (A)
		(A) edge [above, bend left] node {$q$} (B)
	        (B) edge [above, bend left] node {$r'$} (C);
  \path	(C) edge [below, bend left] node {$s$} (B) 
  		(B) edge [below, bend left] node {$r$} (A)
	        (A) edge [below, bend left] node {$q'$} (Z);
\end{tikzpicture}\\
\end{center}

That means that the highlighted node was visited before. However the last visit of this node was not be the first one, because both $(e,y)$ and $(c,u)$ were visited and if the not visited node has two neighbours, then at least one of them is unvisted as well. Hence the last change of the states of highlighted node was when it was an end node of some block. This block ended with L (because $P(b',.)=q'$). This block was not be RL, because $(c,u)$ was visited before, so it was LRL. However before this block we had  the beneath situation:
$$
(b,w)\stackrel{q\;\;r}{\leftrightarrow} \underline{(c,u)}~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
A block LRL does not change the last agent's state of the left node, so $A(c,u)=b$. and $A(b,w)=c$, The last move of the block LRL has to be via outport $r$ and $P(c,.)=r$, so $A(b,w)=c$, contrary to the previous observation.\\
A symmetric situation holds if the agent wants to start a new block by LL.\\

Now we would like to estimate the number of moves needed to explore the graph by this algorithm.
Realize that after RL, LRL is performed until the next new node is found by a block LR. Symmetrically with swapped R and L.
Let say that the line has $n$ nodes. Then the adversary may put the agent in the middle of the line in such the way that, so the agent has to performs $n-2$ RL or LR blocks. After every block RL (or LR), there is one more visited node, so the number of RLR (or LRL) blocks that has to be executed before performing the next RL (or LR) block increases by $1$. The last number of consecutive LRL or RLR blocks is $n-2$ (because the last move is a single one), so the agent has to perform at least
$$
2(n-2)+1+\sum_{i=1}^{n-2}3i=\frac{(n-2)(3n+1)}{2}+1=\Omega(n^2)
$$
moves in order to explore the graph. It worths to note that it is approximately $3$ times longer than RR algorithm.
%Realize that when the agent enters a new node, then we use blocks RL and LR, which works the same as when visiting a new node in RR algorithm. When RR is used when agent enters the already visited node, then 

%The vertex' state change every step, thence after the first R, $(b,w)$ changes to $(b,w')$ and $P(b,w)=q$.\\
%After L we may either have agent's state $b$ or $b'$, but the vertex state will be $w'$ and we have to use the outport $q$.
%
%There exists an automorphism of the transition graph is that swaps $a$ and $a'$, so we may assume that the initial agent's state is $a$. Realize that for any $a_1,a_2$, there exists $v$ such that $A(a_1,v)=a_2$.  Imagine that the agent enters some node for the first time, with the agent's state $a_1$. Assume that the agent's state in the previous move was $a_2'$. The adversary wants to turn back the agent and let him go the opposite direction. However the agent's state determines the outport, so he has to change the agent's state to $a_2$. From the previous observation, we are able to do so, by choosing the appropriate vertex' state. Realize that $a_1$ determines the outport, so the appropriate port should be directed to the previous node. Hence, when the agent is entering a new node, he has to turn around, so he goes one step forward turn around and go back with the opposite orientation --- denote this sequence of moves by FB.
%Assume that otherwise (when he does not enter a new node), the agent make a sequence of moves: forward, back and forward (call it FBF).
%Assume that all the nodes are indexed with consecutive natural numbers from left to right and the starting position has the index $x$.
%We may say, that the virtual state of agent is the tuple (node index, the orientation ($L$ or $R$), leftmost visited node, rightmost visited node). Hence for $c<y<d$, $(y,L,y,d)\stackrel{FB}{\rightarrow}(y,R,y-1,d)$, $(y,R,c,y)\stackrel{FB}{\rightarrow}(y,L,c,y+1)$, $(y,R,c,d)\stackrel{FBF}{\rightarrow}(y+1,R,c,d)$ and $(y,L,c,d)\stackrel{FBF}{\rightarrow}(y-1,L,c,d)$.
%Realize that the definition of the chosen vertices' states and direction of ports approves the virtual states transitions for the move FB. We have to prove that the virtual states transitions are also true for moves of FBF type.
%POKAZAC, ze gdy uzywamy ktoregos portu po raz drugi(w danym nodzie), to musielismy byc w tym samym stanie.
%Assume that the agent moved according to FB and FBF moves to some virtual state $(y,L,c,d)$, for $c<y<d$. If $y=c+1$, then the agent has to move to the node $c$, which is visited again. Realize that, when we visit 
%After the first step, agent meets a new node with state $v'$ and with agent's state $a'$, but $P(a',v')=p'$, so he rotates and goes the step forward. Realize that the vertices' states in $x$ and $x+1$ has been already changed.\\
-------------------------------------\\


CASE 7.1.2. If $(\forall\; (a,v)\in S)\; A(a,v)=a'$, then we obtain CASE 6.1.\\
%$A(a,v)=a'$. Then $R_2(a,v)=(a',v')$.
%Case II.1. $A(a',v')=a$. Then $R_2(a',v')=(a,v)$. Realize that the actual situation is symmetric with respect to agent's state, so we are going to consider two cases:
%Case II.1.1. If $A(a,v')\neq A(a',v)$, then the transition graph is equivalent with this from the case I.2.2.
%Case II.1.2. If $A(a,v')=A(a',v)$, then the transition graph is equivalent with this from the case I.2.1.
%Case II.2. $A(a',v')=a'$, so $R_2(a',v')=(a',v)$. Then $R_2(a',v)=(a,v')$, because otherwise $a'=A(a',v)=A(a',v')$.
%Case II.2.1 If $A(a,v')=a$, then the transition graph is equivalent with this from the case I.1.
%Case II.2.2 If $A(a,v')=a'$, then the transition graph is equivalent with this from the case I.2.1.
CASE 7.2. Assume that 
\begin{equation}
\label{property}
(\forall\; p\in\Ps)(\forall\; a\in \As)(\exists\; v\in\Vs)\; P(a,v)=p~.
\end{equation}
Due to Fact \ref{wn1} we may assume that $R_3(a,v)=(a',v',p)$.\\
CASE 7.2.1. Let $A(a',v)=a'$, so because the vertex state does not determines the outport and (\ref{property}), we attain $R_3(a',v)=(a',v',p')$. Then also $R_3(a',v')=(a,v,p)$, because of (\ref{property})and CASE 4. Moreover, the agent's state is not determined by the vertex state, so again from (\ref{property}) we get $R_3(a,v')=(a',v,p')$.\\

\subparagraph{10. (7.2.3)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[bend left] (m-1-1) edge node [above, very near start] {$p$} (m-2-2);
    \draw (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw (m-2-1) edge node [left,near start] {$p'$} (m-1-2);
    \draw[bend left] (m-2-2) edge node [below, very near start] {$p$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    \node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      \node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  \node (Y) at (7,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (E)
	  (E) edge [above, bend left] node {$p$} (F)
	  (F) edge [above, bend left] node {$p$} (Y);
  \path (F) edge [below, bend left] node {$p'$} (E)
           (E) edge [below, bend left] node {$p'$} (D)
  	  (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    \node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      \node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  \node (Y) at (7,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (E)
	  (E) edge [above, bend left] node {$p$} (F)
	  (F) edge [above, bend left] node {$p$} (Y);
  \path (F) edge [below, bend left] node {$p'$} (E)
           (E) edge [below, bend left] node {$p'$} (D)
  	  (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 7.2.2. Assume that $A(a',v)=a$, so $R_3(a',v)=(a,v',p')$ from (\ref{property}).\\
CASE 7.2.2.1. Let $A(a',v')=a$. Then $R_3(a',v')=(a,v,p)$ by (\ref{property}). However, if we swap $v$ with $v'$, then we will get CASE 7.2.1.\\
CASE 7.2.2.2. Hence from (\ref{property}), $R_3(a',v')=(a',v,p)$.\\
Note that $R_3(a',v)=(a,v',p')$, so if we swap all the vertex states, agent's states and outports, then we obtain CASE 7.2. However, $A(a,v)=a'$, so we get CASE 7.2.2. But from CASE 7.2.2.1. $A(a,v')\neq a'$, so together with (ref{property}) we finally get $R_3(a,v')=(a,v,p')$.\\

\subparagraph{13. (7.2.6)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw  (m-2-1) edge node [left, near start] {$p'$} (m-1-1);
    \draw (m-2-2) edge node [right, near start] {$p$} (m-1-2);
    \draw (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
    \draw (m-1-1) edge node [below, near start] {$p$} (m-2-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
Algorithm 3 = Rotor-Router
\end{minipage}
\end{center}
 
Realize that the outport of this algorithm determines the agent's state. hence if the adversary put the outports in such a way that only one type of port directs to a node, then the agent will always have the same agent's state in this node. If the adversary do this for all the nodes, then at each node the same will be true. Thence we may think of it as the algorithm without the agent's memory. However the vertex' state change every time it is used, so it is then isomorphic with RR algorithm. Indeed, note that in this case the direction is given not only by vertices' states, but also by the fixed agents' states , which are deteremined by the outports given a priori. Hence for every node, $v$ directs to one direction and $v'$ leads to another, however for different nodes, the same type of vertex may indice different direction.

Thence we only need to show that it is possible to arrange the outports in such the way, that for every node, there is only one type of ports which indice there. However it is simple to realize, that this condition guarantees that if the outports are established  for one node, then the node, which is two places apart has to have the outports defined in opposite way, because it has to indice the opposite direction with the same outport. Moreover there is no possiblity to define the other outports using this restriciton, so me may define outports separately for the nodes which are even places apart the left end of the line and separately for the odd ones.

%If the state of vertex changes on every step and the outport is not defined only by vertex' state and for any port $p$ and any $a\in As$, there exists $v\in Vs$, such that $P(a,v)=p$ and $R_2$ is iniective function, then the algorithm can be reduced to SEA.

%Indeed, assume that $P(a,v)=p$ and $P(a',v)=q$. By the assumptions, then $P(a,v')=p'$ and $P(a',v')=q'$. Assume for a while that $R_2$ is a permutation that consists of one cycle.
%Without a loss of generality we may assume that the agent starts with agent's state $a$ in a $k$-th node, initialized with a state $v$ and that port $p$ directs to $k+1$-th node of the line. The adversary should initialize all vertices as follows:
%the node with index $k+c$ should be initialized by $v$, if $2\not| c$ and by $v'$ for $2|c$; the node with index $k-c$ should be initialize by $v$ if $2|c$ and by $v'$ for $2\not| c$.
%Moreover all the ports should be directed in such the way, that during the first visit, the agent is directed to the previous node.
%TROCHE INACZEJ TO BEDZIE
%NIE WIEM NA ILE TERAZ TO MA SENS

%%%%%%%
\begin{lem}
\label{lem:threeports}
Assume we have:
\begin{enumerate}
\item $\forall a \in \As$ $V(a,v) = v'$ and $V(a,v') = v$,
\item function $P(s) = P(s') = P(s'')$ for three different state values $s, s',s'' \in S$,
\end{enumerate}
then such an algorithm requires in the worst case $\Omega(n^2)$ steps to explore a path.
\end{lem}
\begin{proof}
Set $S$ has $4$ values so if function $P$ returns the same port for all of them then the algorithm cannot explore all paths of length $>2$. 

Assume that for some $a \in \As$, $v\in \Vs$ and $p\in \Ps$, we have $P(a,v) = p$ and $P(s) = p'$ for $s \neq (a,v)$. Let us construct a path $\mathcal{P} = (v_1,v_2,\dots, v_n)$ of length $n$ such that a port from $v_i$ to $v_{i+1}$ is always $p$ (and port from $v_{i}$ to $v_{i-1}$ is $p'$). Let $v_1$ be the starting position of the agent and let $v'$ be the initial state of each vertex and consider the exploration time of such an agent on such a path.

To prove the time complexity, we show the following: \\
\textit{Claim: For any $i \in 2,3,\dots n-1$, between first visit to $v_i$ and $v_{i+1}$, the agent visits node $v_1$. }\\
To prove the claim observe that, when entering $v_i$ for the first time, the last exit from each vertex $v_2,v_3,\dots,v_{i-1}$ was  via port $p$.  This means that the state of each of these nodes is $v'$ (it is because $V(a,v) = v'$). Since the state of $v_i,v_{i-1},\dots,v_2$ is $v'$, and the agent is at $v_i$, the agent leaves each of these vertices via port $p'$ and walks straight to node $v_1$. This completes the proof of the claim. \\

The lemma is a direct consequence of the claim, because time to explore the whole path is at least $2 \cdot \sum_{i=1}^{n-2} i \in \Omega(n^2)$.

\end{proof}

CASE 7.3. Assume that
$$
(\exists\; p\in\Ps)(\exists\; a\in \As)(\forall\; v\in \Vs)\; P(a,v)=p~.
$$
Agent's states does not determine the outports and vertex' states always change, so Lemma \ref{lem:ports} guarantees the assumptions of Lemma \ref{lem:threeports} and hence in this case, the algorithm requires $\Omega(n^2)$ steps to explore a path.
 
\input{sections/counterexamples}


%%%%%%%

\subsection{unlimited memory}
We consider a model, where $1$ agent tries to explore line topology, where every vertex has some states and number of OutPorts defined by adversary, with no identificators. InPorts and OutPorts does not need to be the same. Also the agent does not have any token that he may take through edges and leave at vertices.

We would like to find some lower bound for complexity of exploration of line graph using a deterministic algorithm. In order to do so, we assume that we are able to save any information in vertices and agent can remember everything he has seen.

For descriptive purpose, let us numerate consecutive vertices by consecutive numbers from $1$ to $n$. Assume that the agent starts the exploration at vertex $1$, so there is only one OutPort, so he can change a state of vertex $1$ to $1$ ($S(1)=1$) and simply traverse to vertex $2$.

Now assume that after some number of steps, the agent is in vertex $k$ and he is aware of all the OutPorts, which can transport him from vertex $1$ to vertex $k$ in $k-1$ consecutive steps and for all $i\leq k$, $S(i)=i$. In such the situation, we say that agent has $k$-progress. Let $OL(i)$ be the number of OutPort, which directs from vertex $i$ to vertex $i-1$, for $i=2,\ldots,n$. Let $OP(i)$ be the number of OutPort, which directs from vertex $i$ to vertex $i+1$, for $i=1,\ldots,n-1$. Realize that, if the agent knows $OL(i)$, then he knows $OP(i)$ and vice versa (if $i\neq 1$ and $i\neq n$).
If he has no $(k+1)$-progress, then he cannot guess $OL(k)$, so we may assume that at vertex $k$ he chooses a port with smaller id. If he will use $OL(k)$, then the state of the next vertex is $k-1$. If the state of the successor is another, then he knows that he went forward to vertex $k+1$ and hence after changing $S(k+1)=k+1$ he has $k+1$-progress.
Further, the agent wants to make a sequence of $\lfloor\sqrt{k}-1\rfloor$ steps using $OL(k-i)$ port at step $i$. If for $i=1,2,\ldots,j-1$, after step $i$, the agent has seen state $k-i-1$ and after step $j$, he sees the state different from $k-j-1$, then that means that, starting from vertex $k$, he has just made $j+1$ steps forward. Hence he can change $S(k+j+1)=k+j+1$ and establish $OL(i)$ for $i=k,k+1,\ldots,k+j$.
 



==> sections/line_very_old.tex <==
%line.tex
% !TEX root = ../dual_memory.tex
\newcommand{\As}{\mathrm{As}}
\newcommand{\Vs}{\mathrm{Vs}}
\newcommand{\Ps}{\mathrm{Ps}}

\section{Line topology with dirty memory}

\subsection{1 bit per agent, 1 bit per vertex}
A simple round-robin strategy for graph exploration, understood as taking a port different from the previous one on each visit to a vertex of degree $2$, results in exploration time of a path $O(n^2)$. Such a strategy can be clearly implemented with only a single bit at each vertex and zero bits on the agent (if we don't require termination). This strategy can be generalized to arbitrary graphs and such an algorithm, called Rotor-Router works in time $O(mD)$~\cite{YanovskiWB03} for state arbitrary initialization and arbitrary port labelling.
%A classical solution shows that there exists an algorithm, which enables to perform a simple exploration algorithm on a line of size $n$ in $O(n^2)$ steps called Rotor-Router (abbreviated by RR). Every time, when an agent enters a vertex, (excluding two ends of the line) it changes its state to opposite and uses a number of port, which is indicated by this state (every time it enters the opposite port as well).

It is known that adding more bits of memory on the vertices does not help as time $\Omega(n^2)$ is required even in the model with unlimited memory on each node ~\cite{MencPU17}.
In this section  we additionally allow the agent to have $1$ bit of memory and we want to answer the question of whether this single bit allows to break the $\Omega(n^2)$ barrier.

\paragraph{Notation}
In the following lower bound on the line, we take any algorithm working with a single bit at the agent and a single bit at each node. We will focus on the actions of the algorithm in vertices with degree $2$. In such vertices, there are four possible inputs to the algorithm $S = \{(0,0),(0,1),(1,0),(1,1)\}$, where in pair $(a,v)$, $a$ is a bit on the agent and $v$ is a bit saved on the vertex. Let us denote the agent's states by $\As$, vertex' states by $\Vs$ and possible outports by $\Ps$. We use a shorthand notation $'$ to indicate the inverted value of a bit. For example, if $a=0$, then $a'=1$ and vice versa. 


%We denote an entering state as a pair $(a,v)$, where $a$ is a bit on the agent and $v$ is a bit saved on the vertex. At each step at a node with degree $2$, an algorithm has to return some pair $(b,w)$ and port number $p$, depending on the state of the vertex and the state of the agent. Then the agent changes its state to $b$, the state of vertex to $w$ and quits the actual vertex via port $p$. 

%If the vertex is an endpoint of the line, then agent can leave the only by one port. (NIE ANALIZOWALEM JAK SIE ZMIENIA DECYZJA JESLI WIADOMO, ZE TO PUNKT KONCOWY --- TO TRZEBA DODAC)





%The same for vertex' states and ports.

%
%\begin{tikzpicture}[->]
 %\node (X) at (0,0) { };
 %\node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 %\node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  %\node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    %\node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      %\node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  %\node (Y) at (7,0) { };
 %\path (A) edge [above, bend left] node {$p'$} (B)
	  %(B) edge [above, bend left] node {$p'$} (C)
	  %(C) edge [above, bend left] node {$p'$} (D)
	  %(D) edge [above, bend left] node {$p$} (E)
	  %(E) edge [above, bend left] node {$p$} (F)
	  %(F) edge [above, bend left] node {$p$} (Y);
  %\path (F) edge [below, bend left] node {$p'$} (E)
           %(E) edge [below, bend left] node {$p'$} (D)
  	  %(D) edge [below, bend left] node {$p'$} (C)
	  %(C) edge [below, bend left] node {$p$} (B)
	  %(B) edge [below, bend left] node {$p$} (A)
	  %(A) edge [below, bend left] node {$p$} (X);
%\end{tikzpicture}

The goal of this section is to prove the following:
\begin{theorem}
Any algorithm in the model with one bit at the agent and one bit at each node requires in worst-case time $\Omega(n^2)$ to explore a path.
\end{theorem}
Assume for contradiction, that some algorithm $\mathcal{A}$ explores any path in $o(n^2)$ steps. For algorithm $\mathcal{A}$, for any $s \in S$, by $A(s), V(s), P(s)$ we denote respectively, the returned agent state, vertex state and the chosen outport in each vertex with degree $2$. Moreover, we denote $R_3(s):=(A(s),V(s),P(s))$ and $R_2(s):=(A(s),V(s))$. In the following series of facts we will prove some properties that $\mathcal{A}$ has to satisfy. 

\begin{fact}
\label{wn1}
 $(\forall\; a\in \As)(\exists\; v\in \Vs)\; A(a,v)=a'$.
% or the algorithm reduces to RR.
\end{fact}
\begin{proof}
Assume that $(\exists\; a \in \As)(\forall\; v\in \Vs)\; A(a,v)=a$ and let the starting position be the midpoint of the path. If $a$ is the starting state of the agent, then the agent will never change its state before reaching an endpoint of the path. But before that the exploration is not faster than rotor-router, hence there exists an initialization of port numbers, such that reaching the endpoint takes $\Omega(n^2)$ steps. If $a'$ is the starting state, then either $A(a',w)=a$, for some $w \in \Vs$. In this case, the adversary sets $w$ to be the starting state of the starting vertex and from the second step the algorithm explores not faster than the rotor-router hence needs $\Omega(n^2)$ steps to reach an endpoint. Note that if $A(a',w)=a'$ for each $w\in \Vs$, then this reduces to the first case. The obtained contradiction completes the proof of the fact.
\end{proof}

\begin{fact}
\label{wn2}
If $A(a,v)=a$ for some $(a,v) \in S$, then $V(a,v)=v'$.
\end{fact}
\begin{proof}
We will show that otherwise algorithm $\mathcal{A}$ falls into infinite loop for some initial state of the path. Assume that $R_3(a,v) = (a,v,p)$ for some entering state $(a,v)$ and port $p \in \Ps$. Then if $a$ is the starting state, it is easy to see that the agent falls into infinite loop on the following gadget (double circle indicates the starting position of the agent):
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
%  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}
If $a'$ is the starting state, then we can use Fact~\ref{wn1}, $(\exists\; w\in \Vs)\;A(a',w)=a$, so if the agent's initial state is $a'$. Let $q = P(a',w)$ (it is possible that $p = q$) and observe that the  agent falls into infinite loop in the following gadget:
%$$
%\underline{(a',w)}\stackrel{q\;p'}{\leftrightarrow}(a,v)\stackrel{p\;p}{\leftrightarrow}(a,v)
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (Z) at (1,0) {$w$};
  \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (3,0) {$v$};
  \node (Y) at (4,0) { };
 \path 	(Z) edge [above, bend left] node {$q$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (Z)
		(Z) edge [below, bend left] node {$q'$} (X);
\end{tikzpicture}\\
\end{center}

%which after first step reduces to the CASE 2.1.\\
%Thanks to the CASE 2. we obtain following results:
\end{proof}

\begin{lem}
\label{lem:vconst}
Algorithm $\mathcal{A}$ does \textbf{not} satisfy the following:
\[
(\forall\;a,x\in \As)(\forall\;v,y,z\in Vs)\;R_2(a,v)=(a',v) \land R_2(a',v)=(x,y)\land R_2(a',v')=(x,z).
\]
%Then the adversary can initialize the algorithm in such the way, to either produce infinite loop either reduce the algorithm to RR.

\end{lem}

\begin{proof}
%CASE 3. 
Assume that the formula holds and we will show that in such a case $\mathcal{A}$ would fall into an infinite loop for some initializations of the path. 
From Fact \ref{wn1}, we obtain, that $x = a$. Denote $P(a,v)=p$.\\
%CASE 3.1. 

If $y=v$, then let $P(a',v)=q$, and the following initial state of the path results in an infinite loop: 
%$\underline{(a,v)}\stackrel{p\;q}{\leftrightarrow}(a',v)$ 
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path 	(A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (Y);
  \path	 (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}

%so only two vertices will be visited.\\
%CASE 3.2. 
In the opposite case, where $y = v'$, the agent would fall into an infinite loop on the following gadget:
%$$
%(a,v)\stackrel{p\;p}{\leftrightarrow}(a',v')\stackrel{p'\;p}{\leftrightarrow}(a,v)~,
%$$
\begin{center}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v'$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
% \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (B) at (3,0) {$v$};
  \node (Y) at (4,0) { };
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (Y);
  \path	 (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (Z)
		(Z) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}\\
\end{center}

%which leads to infinite loop.\\
We have $R_3(a,v) = (a',v,p)$, hence in the first step, the agent moves to the middle vertex, changes its state to $a'$, and keeps $v$ as the state of the first vertex.
At the middle vertex when the agent's state is $a'$, then it always changes its state to $a$ and moves to one of the outer vertices. But since the outer vertices are both in state $v$, the agent returns to the middle vertex, and so on, which is an infinite loop.
%and, hence we always return to the middle vertex from the entering state $(a,v)$, hence the outer vertices' states won't change as well, so we never visit any of the positions excluding these 3.
\end{proof}

We may conclude the following results:
\begin{fact}
\label{wn3}
Let $a\in\As$. If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then $(\forall\; w\in \Vs)\; R_2(a',w)\neq(a,w)$ and moreover, from Fact \ref{wn2}, then $(\forall\; w\in \Vs)\; V(a',w)=w'$.
\end{fact}
\marginpar{DB:moze rozbic na 2 fakty}

\begin{fact}
\label{wn4}
Let $a\in\As$. If $(\forall\; v\in \Vs)\; A(a,v)=a'$, then, from facts \ref{wn1} and \ref{wn3}, $(\exists\; w\in \Vs)\; R_2(a',w)=(a,w')$.
\end{fact}

CASE 4. Assume that for some $v$, $R_3(a,v)=(a',v,p)$ and $R_3(a',v)=(a,v,q)$. Then $(a',v)\stackrel{q\;p}{\leftrightarrow}(a,v)$ gives the 2-loop.

\begin{lem}
\label{lem:ports}
Let $a\in \As$. If $(\forall\; v\in\Vs)\; P(a,v)=p$, then 
$$
(\exists\; w\in \Vs)\; A(a',w)=a' \land P(a',w)=p'~.
$$
\end{lem}

\begin{proof}
CASE 5.1. If all the outports are the same, then there is no way to change the direction, hence 2-loop can be trivially obtained.\\
CASE 5.2. However, if $(\forall\;w\in Vs)\;P(a',w)=p' \Rightarrow A(a',w)=a$, then we can construct the sequence of ports:
$$
(a,v)\stackrel{p\; p'}{\leftrightarrow}B \stackrel{p\; p}{\leftrightarrow}C\stackrel{p'\; p}{\leftrightarrow} (a,v)~,
$$
which blocks the opportunity to change the direction both in A and D.
Indeed, in order to get to those vertices, we have to use port $p'$, but then the agent's bit changes to $a$. However the adversary initializes terminal positions with vertex's state $v$, then the agent has to use $P(a,v)=p$, so it goes always either to B or C.
\end{proof}

\begin{fact}
\label{wn5}
If $(\forall\; v\in\Vs)\; A(a',v)=a$, then $P(a,v)\neq P(a,v')$.
\end{fact}

CASE 6. Assume that 
$$
(\forall\; a\in\As)(\forall\; v\in\Vs) A(a,v)=a' \lor (\exists\;a\in\As)\; V(a,v)=v~.
$$ \marginpar{DB: ewentualnie to mozna rozbic na osobne przypadki 6. i 7. zamiast 6.1 i 6.2}
CASE 6.1. Let the agent changes the agent's bit every round i.e.
$(\forall\; a\in\As)(\forall\; v\in\Vs)\; A(a,v)=a'$. By the symmetry and Fact \ref{wn3} we obtain that $(\forall\; a\in\As)(\forall\; v\in\Vs)\; R_2(a,v)=(a',v')$, so the vertices' states are always changed as well.
Since we are not able to change the agent's bit at entering state of any particular position, then $(\forall\; a\in\As)(\forall\; v\in\Vs) P(a,v)\neq P(a,v')$, because otherewise there won't be possibility to change the direction at some positions, because of parity argument, which blocks the possibility to visit all the vertices.\\
CASE 6.1.1. If $P(a,v)=P(a',v)=p$, then, by Lemma \ref{lem:ports}, $P(a,v')=P(a',v')=p'$, so the outports depends only on vertices and agent's states are useless, hence this algorithm is just RR.\\
CASE 6.1.2. Otherwise, again from Lemma \ref{lem:ports}, $P(a',v)=P(a,v')=p$ and $P(a,v)=P(a',v')=p'$. We may think of an equivalence relation, where $(a,v)\equiv(a',v')=W$ and $(a,v')\equiv(a',v)=W'$. Then the outports of $W$ and $W'$ are different. Realize that after exit of some position, the vertex state changes, but the future agent's state cannot be another, so it may  be seen as changing the state from $W$ to $W'$ and viceversa. Hence this algorithm is isomorphic with RR.\\
CASE 6.1 provides the following result:

\begin{fact}
\label{fact:1}
Let $a\in \As$. If $(\forall\;v\in \Vs)\;A(a,v)=a'$, then either $(\exists\; w\in \Vs)\;R_2(a',w)=(a,w')\land A(a',w')=a'$, so $R_2(a',w')=(a',w)$ or the algorithm is equivalent with RR.
\end{fact}

CASE 6.2. Assume, that the agent does not change the state of vertex at every step. Moreover, from CASE 4. and CASE 2. we know that $(\exists\; a\in \As)\; R_2(a,v)=(a',v) \land V(a',v)=v'$.\\
CASE 6.2.1. Assume that $R_2(a',v)=(a',v')$. From Lemma \ref{lem:vconst} we obtain $A(a',v')=a$.\\
CASE 6.2.1.1. Realize that if $P(a,v)=p$, $P(a',v)=q$ and $P(a',v')=q'$, then we can construct a sequence:
$$
(a,v)\stackrel{p\; q'}{\leftrightarrow}(a',v)\stackrel{q\; q}{\leftrightarrow}(a',v)\stackrel{q'\; p}{\leftrightarrow}(a,v)~,
$$
\begin{center}
\begin{tikzpicture}[->]
% \node (X) at (0,0) { };
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
%  \node (Y) at (5,0) { };
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$q$} (B)
	        (B) edge [above, bend left] node {$q'$} (C);
	        %(C) edge [above, bend left] node {$$} (Y);
  \path	(C) edge [below, bend left] node {$q'$} (B) 
  		(B) edge [below, bend left] node {$q$} (A)
	        (A) edge [below, bend left] node {$q'$} (Z);
		%(Z) edge [below, bend left] node {$$} (X);
\end{tikzpicture}\\
\end{center}
so the adversary only has to establish the outports dependent on the initial state of agent. We may briefly realize that agent's states never change in such the arrangement, so there is no possibility to change any of entering states $(a,v)$. \\
\paragraph*{Conclusion}
Hence $P(a',v)=P(a',v')$.
Moreover, from Lemma \ref{lem:ports} we obtain that $R_2(a,v')=(a,v)$ and $P(a',v)=P(a',v')\neq P(a,v')$.\\
CASE 6.2.1.2. From Lemma \ref{lem:vconst}, if $R_2(a',v')=(a,v')$, then $A(a,v')=a$, hence, from Fact \ref{wn2}, $R_2(a,v')=(a,v)$. By the same argument as in CASE 6.2. and CASE 6.2.1, we conclude that $P(a,v)=P(a,v')$, hence ports depend only on the agent's state, so by Lemma \ref{lem:ports} we provide the algorithm:\\
$R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p')$,$R_3(a',v')=(a,v',p')$,$R_3(a,v')=(a,v,p)$.\\
\subparagraph{1. (6.1,2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-2-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X)
	  (B) edge [above, bend left] node {$p'$} (Y);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node (Y) at (3,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X)
	  (B) edge [above, bend left] node {$p$} (Y);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.1.3. If $R_2(a',v')\neq (a,v')$, then by CASE 2. we obtain $V(a',v')=v$.\\
%CASE 6.2.1.3.1. Let $A(a,v')=a'$.
From the conclusion after CASE 6.2.1.1. we know that 
%From Fact \ref{fact:1} we obtain $R_2(a',v')=(a,v)$. Moreover, realize that $A(a,v')=A(a,v)$, so from Lemma \ref{lem:vconst}, $V(a,v')=v$.
%From Fact \ref{wn5} we obtain that $P(a',v)\neq P(a',v')$.
%However from CASE 6.2.1.1. we have already known that $P(a',v)=P(a',v')$.\\
%CASE 6.2.1.3.2. Hence
$R_2(a,v')=(a,v)$.\\
CASE 6.2.1.3.1. If $R_2(a',v')=(a',v)$, then from Lemma \ref{lem:vconst} the algorithm can be easily looped.\\
CASE 6.2.1.3.2.1. If $R_3(a,v')=(a,v,p)$, then from Lemma \ref{lem:ports} and Conclusion after CASE 6.2.1.1. we attain $R_3(a',v')=(a,v,p')$ and $R_3(a',v)=(a',v',p')$.\\

\subparagraph{2. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p'$} (m-1-1);
\end{tikzpicture}

\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p'$} (A) 
 	  (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}

\end{minipage}
\end{center}

CASE 6.2.1.3.2.2. Let $R_3(a,v')=(a,v,p')$. Then from CASE 6.2.1.1. we know and Lemma \ref{lem:ports} we obtain $R_3(a',v')=(a,v,p)$ and $R_3(a',v)=(a',v',p)$.\\

\subparagraph{3. (6.1,3.2.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-2-1) edge node [left, near start] {$p'$} (m-1-1);
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p$} (m-2-2);
    \draw[->] (m-2-2) edge node [below, near start] {$p$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path  (AA) edge [above, bend left] node {$p$} (A) 
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p'$} (X) ;
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2. Let $R_2(a',v)=(a,v')$. From Lemma \ref{lem:vconst} $A(a',v')=a'$, so $R_2(a',v')=(a',v)$, because of CASE 2.\\
CASE 6.2.2.1. Assume that $R_2(a,v')=(a',v')$. Then we may swap $v$ with $v'$ in order to obtain CASE 6.2.1.3.1., so by CASE 2. $V(a,v')=v$.\\
%--------------------------------------------------------
%Let $P(a,v)=p$ and $P(a',v)=q$. Then, from Lemma \ref{lem:ports} either $P(a,v')=p$ or $q=p \land P(a,v')=p'$. However, in both cases, by the Lemma \ref{lem:ports} once again we may obtain $R_2(a,v')=(a,v)$.\\
%%Hence we provide two possible algorithms in this arrangement:\\
%%I.2.1 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p')$,$R_3(a',v')=(a,v,p')$,$R_3(a,v')=(a,v,p)$\\
%%KONTRPRZYKLAD\\
%%I.2.2 $R_3(a,v)=(a',v,p)$,$R_3(a',v)=(a',v',p)$,$R_3(a',v')=(a,v,p)$,$R_3(a,v')=(a,v,p')$\\
%%KONTRPRZYKLAD\\
%----------------------------
%Let $P(a,v)=p$. Realize that then $(\exists\;(x,v')\in S)(\exists\; y\in Vs)\;R_3(x,v')=(a',y,p')$.\\
%Indeed, if $P(a',v')=p$, then we may arrange
%$$
%(a,v)\stackrel{p\; p'}{\leftrightarrow}(a',v)~,
%$$
%where after leaving the $(a,v)$ we won't change its vertex' state until we enter it with the agent's state $a'$ through port $p'$, so then $R_3(a,v')=(a',y,p')$ for some $y$.\\
%-----------------------------------------
CASE 6.2.2.2. Assume that $R_2(a,v')=(a',v)$ and $P(a,v)=p$.\\
From Fact \ref{wn5} $P(a',v)\neq P(a',v')$. Hence $P(a',v)=q$ and $P(a',v')=q'$.\\
CASE 6.2.2.2.1.
If $P(a,v')=p$, then there is a sequence:
$$
(a,v)\stackrel{p\; q}{\leftrightarrow} (a',v)\stackrel{q'\; q'}{\leftrightarrow} (a',v) \stackrel{q\; p}{\leftrightarrow} (a,v)~,
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$q'$} (B)
	        (B) edge [above, bend left] node {$q$} (C);
  \path	(C) edge [below, bend left] node {$p$} (B) 
  		(B) edge [below, bend left] node {$q'$} (A)
	        (A) edge [below, bend left] node {$q$} (Z);
\end{tikzpicture}\\
\end{center}
where in order to get to one of the bounds, an agent has to use port $q$ at some move $x$. In order to use $p'$ at step $x+1$, he needs to change the agent's state  to $a'$ at step $x$. However it can only be obtained from the agent's state $a$, so $p=q$. Now, consider the step $x-1$. Then one of the middle vertices has to be entered either from boundary node $(a,v)$ by port $p$ with agent's state $a'$ or by port $q'=p'$, from the state $(a',v')$, with the agent's state $a'$ as well, what contradictes that agent's state before step $x-1$ is $a$.\\
CASE 6.2.2.2.2. Hence $P(a,v')=p'$.\\
CASE 6.2.2.2.2.1 Let $q=p$.\\

\subparagraph{5A. (6.2.3.2.2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p$} (A) 
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2.2.2.2. Let $q=p'$.\\

\subparagraph{5B. (6.2.3.2.2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->, bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [left, near start] {$p'$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path (AA) edge [above, bend left] node {$p'$} (A)  
 	 (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p'$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2.3. Let $R_2(a,v')=(a,v)$. \\
CASE 6.2.2.3.1. Let $P(a',v')=p$. Realize that the agent's state $a'$ can be obtained only from the states $(a,v)$ and $(a',v')$, so it can be only obtained via port $p$. Then the sequence
$$
(a,v)\stackrel{p\; p'}{\leftrightarrow} (a',v)\stackrel{p\; p}{\leftrightarrow} (a',v) \stackrel{p'\; p}{\leftrightarrow} (a,v)~
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p$} (B)
	        (B) edge [above, bend left] node {$p'$} (C);
  \path	(C) edge [below, bend left] node {$p$} (B) 
  		(B) edge [below, bend left] node {$p$} (A)
	        (A) edge [below, bend left] node {$p'$} (Z);
\end{tikzpicture}\\
\end{center}

provides a loop, because agent cannot change neither agent's state nor vertex' states at both ends.\\
CASE 6.2.2.3.2. Hence $P(a',v')=p'$.\\
CASE 6.2.2.3.2.1. If $P(a',v)=p'$, then $P(a,v')=p$ from Lemma \ref{lem:ports}\\

\subparagraph{6. (6.2.4.2.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [above, near start] {$p$} (m-1-2);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-1);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v$};
  \node (Y) at (5,0) { };
 \path (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
  \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (AA) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (4,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (5,0) {$v$};
  \node (Y) at (6,0) { };
 \path  (AA) edge [above, bend left] node {$p'$} (A) 
           (A) edge [above, bend left] node {$p$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p$} (D)
	  (D) edge [above, bend left] node {$p'$} (Y);
  \path (D) edge [below, bend left] node {$p$} (C)
	  (C) edge [below, bend left] node {$p'$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p'$} (AA)
	  (AA) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 6.2.2.3.2.2. Let $P(a',v)=p$.
Then the sequence
$$
(a,v)\stackrel{p\; p}{\leftrightarrow} (a',v)\stackrel{p'\; p'}{\leftrightarrow} (a',v) \stackrel{p\; p}{\leftrightarrow} (a,v)~
$$ 
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (Z) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (2,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$a'$] (B) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em, label=$a$] (C) at (4,0) {$v$};
 \path 	(Z) edge [above, bend left] node {$p$} (A)
		(A) edge [above, bend left] node {$p'$} (B)
	        (B) edge [above, bend left] node {$p$} (C);
  \path	(C) edge [below, bend left] node {$p$} (B) 
  		(B) edge [below, bend left] node {$p'$} (A)
	        (A) edge [below, bend left] node {$p$} (Z);
\end{tikzpicture}\\
\end{center}


provides the loop. Indeed, in order to change either of the boundary states, the agent needs to use the port $p$ with agent's state $a'$, while entering them. It is only possible, if he goes from the inner vertex of state $(a,v)$. As soon as, he cannot enter the middle vertex by port $p$ with agent's state $a$ (because $A(a,v)=a'$), so the agent has to enter it via $p'$, so $P(a,v')=p'$ and $(a,v')$ had to be a state of the other middle vertex. Recursively, we may prove that at least one of the middle states has to be initated with agent's state $a$, which is not true.\\
CASE 7. Assume that the state of vertex changes on every step, but state of agent is not and the outport is not defined only by vertex' state. \\
%Then either exists $a$ such that $P(a,v)=P(a,v')$ or $P(a,v)=P(a',v')$ and $P(a',v)=P(a,v')$.\\
%TO JEST CALY DUZY PRZYPADEK DO ROZPATRZENIA
CASE 7.1. Assume that the outport is defined by the state of the agent i.e.
$$
(\forall\; v\in \Vs)\; P(a,v)=p \land P(a',v)=p'~.
$$
CASE 7.1.1. Let $A(a,v)=a$. Then $R_3(a,v)=(a,v',p)$ and because of CASE 4. we obtain $R_3(a,v')=(a',v,p)$.\\
CASE 7.1.1.1. Let $A(a',v)=a'$. Then similarily $R_3(a',v)=(a',v',p')$ and $R_3(a',v')=(a,v,p')$.\\

\subparagraph{7. (7.1.1.1)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
    \draw[->] (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw[->] (m-2-1) edge node [left, near start] {$p$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
Algorithm 2
\end{minipage}
\end{center}

CASE 7.1.1.2. If $A(a',v)=a$, then $R_3(a',v)=(a,v',p')$.\\
CASE 7.1.1.2.1. Let $A(a',v')=a$. Then $R_3(a',v')=(a,v,p')$, so everytime the agent's state is $a'$, the outport $p'$ is used and the state is changed to $a$, so the outport during the next step will be $p$, so
$$
A\stackrel{p\; p'}{\leftrightarrow}(a,.)\stackrel{p\; p}{\leftrightarrow}(a',.)\stackrel{p'\; p}{\leftrightarrow}B
$$
provides a loop.\\
CASE 7.1.1.2.2. If $A(a',v')=a'$, then $R_3(a',v')=(a',v,p')$.\\

\subparagraph{8. (7.1.1.2.2)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[->] (m-1-1) edge node [left, near start] {$p$} (m-2-1);
    \draw[->,bend left] (m-1-2) edge node [left, very near start] {$p'$} (m-2-1);
    \draw[->,bend left] (m-2-1) edge node [right, very near start] {$p$} (m-1-2);
    \draw[->] (m-2-2) edge node [right, near start] {$p'$} (m-1-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
TODO
\end{minipage}
\end{center}

To wytlumaczenie jest dobre dla algorytmow 7. i 8.\\
---------------------------------------------------\\
Realize that agent's state determines the outport, because $P(a,.)=p$ and $P(a',.)=p'$ and moreover
\begin{equation}
\label{prop2}
(\forall\; v\in\Vs)(\forall\; a\in\As)(\exists\; b\in\As)\; R_2(a,v)=(b,v')\land R_2(a,v')=(b',v)~.
\end{equation}
We will show that the adversary is able to force the agent to move according to a sequence decomposed into blocks LR, RL, LRL and RLR where L denotes a move via the left port and R --- a move through the right port. Moreover, assume that after executing the block RL, the next move is L and that after LR, the next block starts with R.\\
Realize that the adversary can establish any starting port (we assume that both ports are available, so the node is not an endpoint of the line structure), so without a loss of generality, let us assume that it will be R. The algorithm is deterministic, so the adversary can choose a vertex' state and outports at the moment of the first visit of a node.
Moreover, assume that adversary established the outports and initial vertices in such the arrangement, that after the agent enters a new node (not yet visited), he has to use the move in the opposite direction in next two consecutive moves (so he uses either RL or LR block).
It is always possible. Indeed, consider a situation that the agent uses R (or alternatively L) with the state $(b,w)$ and enters the new node, with some agent's state $c$. The vertex' state of the left node is then $w'$. The next move will be performed via port determined by $c$ (let $r=P(c,.)$). We wants the agent to go L, so adversary defines the left outport as $r$. Because the agent's state determines the outport and the adversary wants the agent to go L again, so the next time the agent will be in the left node, it should have the opposite agent's state, i.e. $b'$. However, by (\ref{prop2}), there exists such $u$ that $R_3(c,u)=(b',u',r)$. Hence the RL is possible in such the situation. Hence, in this situation RL changes the states from
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (?,u)~
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw,double, circle, text width=.5em, text height=0.5em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.5em, text height=0.5em, label=$?$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}

to
$$
\stackrel{?\;\;q'}{\leftrightarrow}\underline{(b',w')}\stackrel{q\;\;r}{\leftrightarrow} (c,u')~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=0.6em, label=$$] (Z) at (1,0) {$ $};
 \node [draw, double, circle, text width=.5em, text height=0.6em, label=$b'$] (A) at (2,0) {$w'$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$c$] (B) at (3,0) {$u'$};
 \path 	(Z) edge [above, bend left] node {$?$} (A)
		(A) edge [above, bend left] node {$q$} (B);
  \path	(B) edge [below, bend left] node {$r$} (A) 
  		(A) edge [below, bend left] node {$q'$} (Z);
\end{tikzpicture}\\
\end{center}

If the new node is discovered by L move, then by the symmetry gives the same possibility by the block LR. Obviously either RL or LR is the starting block of the algorithm (there is only one visited node).\\
Now consider a situation that at some moment the agent performs a block RLR as beneath:
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (c,u)~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw,double, circle, text width=.6em, text height=.6em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.6em, text height=.6em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
Realize that both R moves are performed via outport $q$ and agent's state determines the outport, so after move L, the agent's state has to be $b$ as well.\\
Note that the right node have been visited, because otherwise the block RL should be performed. Let $c$ be the last agent's state used in the right node. Thence $P(c,.)=r$ and $P(c',.)=r'$.
Realize that $A(b,w)=c$, because otherwise $P(c',.)=r$. Before the last move of block RLR, the state of left node will be thence $(b,w')$ and the vertex state of the right node will be $u'$, because after the first move of the block RLR, a situation will be as follows:
$$
(b,w')\stackrel{q\;\;r}{\leftrightarrow} \underline{(c,u)}~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=.6em, label=$b$] (Z) at (1,0) {$w'$};
 \node [draw, double, circle, text width=.6em, text height=.6em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
However we know that $A(b,w)=c$, so by (\ref{prop2}), $A(b,w')=c'$. Moreover $P(c',.)=r'$, so after the block RLR, the states will be as follows:
$$
(b,w)\stackrel{q\;\;r}{\leftrightarrow} \underline{(c',u')}\stackrel{r'\;\;?}{\leftrightarrow}~.
$$
That proves that after the block RLR, the next move will be R as well. Symmetrically for LRL.\\

Consider that we only use blocks from the set $Bl:=\{RL, LR, RLR, LRL\}$.
Note that if the block ends by some move, then the next will starts with the same move. Moreover the ending node of any of theses blocks was visited before the execution of this block. We are able to determine the last agent's state for any visited node. Realize that both the last agent's state and vertex state of ending node of any block change. Moreover, both RLR and LRL do not change states of any other nodes. However, RL and LR changes the vertex' state of new node and determines the last agent's state used of this new node and do not change states of any other nodes. Nevertheless, as the vertex state of the new node is used for a first time, we may think that it is determined by this block as well.
It also worth to mention that moves from the block RL change the states in the same way as the two last moves of the block LRL (symmetrically for LR and two last steps of RLR).  

Now we would like to show that the algorithm can be decomposed in blocks from the set $Bl$ (exluding the last block which will be a single move), i.e. the new block cannot start with the same two moves (RR or LL). As said before, the first block of the algorithm is either RL or LR. Assume that agent performed only some number of blocks from the set $Bl$ and
assume that after these moves we have the situation as beneath:
$$
\underline{(b,w)}\stackrel{q\;\;r}{\leftrightarrow} (c,u)\stackrel{r'\;\;s}{\leftrightarrow}(d,x)
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, double, circle, text width=.6em, text height=0.6em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, circle, text width=.5em, text height=0.6em, label=$c$] (A) at (2,0) {$u$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$d$] (B) at (3,0) {$x$};
 \path 	(Z) edge [above, bend left] node {$q$} (A)
		(A) edge [above, bend left] node {$r'$} (B);
  \path	(B) edge [below, bend left] node {$s$} (A) 
  		(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}

and moreover the agent wants to take two consecutive moves R. As this is the beginning of the new block, thence the last move had to be R as well, so the previous block ended with the sequence LR (either block LR or RLR was used). Realize that $(c,u)$ had to be visited yet, because otherwise RL will be performed. Moreover $P(c,.)=r$ and $P(c',.)=r'$, so $A(b,w)=c'$. Two moves before the potential new block, the situation was as follows:
$$
(e,y)\stackrel{t\;\;q'}{\leftrightarrow}\underline{(b',w')}\stackrel{q\;\;r}{\leftrightarrow} (c,u)\stackrel{r'\;\;s}{\leftrightarrow}(d,x)~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.6em, text height=0.6em, label=$e$] (Z) at (1,0) {$y$};
 \node [draw, double, circle, text width=.5em, text height=0.6em, label=$b'$] (A) at (2,0) {$w'$};
 \node [draw, circle, text width=.6em, text height=0.6em, label=$c'$] (B) at (3,0) {$u$};
  \node [draw, circle, text width=.6em, text height=0.6em, label=$d$] (C) at (4,0) {$x$};
 \path 	(Z) edge [above, bend left] node {$t$} (A)
		(A) edge [above, bend left] node {$q$} (B)
	        (B) edge [above, bend left] node {$r'$} (C);
  \path	(C) edge [below, bend left] node {$s$} (B) 
  		(B) edge [below, bend left] node {$r$} (A)
	        (A) edge [below, bend left] node {$q'$} (Z);
\end{tikzpicture}\\
\end{center}

That means that the highlighted node was visited before. However the last visit of this node was not be the first one, because both $(e,y)$ and $(c,u)$ were visited and if the not visited node has two neighbours, then at least one of them is unvisted as well. Hence the last change of the states of highlighted node was when it was an end node of some block. This block ended with L (because $P(b',.)=q'$). This block was not be RL, because $(c,u)$ was visited before, so it was LRL. However before this block we had  the beneath situation:
$$
(b,w)\stackrel{q\;\;r}{\leftrightarrow} \underline{(c,u)}~.
$$
\begin{center}
\begin{tikzpicture}[->]
 \node [draw, circle, text width=.5em, text height=0.5em, label=$b$] (Z) at (1,0) {$w$};
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$c$] (A) at (2,0) {$u$};
 \path 	(Z) edge [above, bend left] node {$q$} (A);
  \path	(A) edge [below, bend left] node {$r$} (Z);
\end{tikzpicture}\\
\end{center}
A block LRL does not change the last agent's state of the left node, so $A(c,u)=b$. and $A(b,w)=c$, The last move of the block LRL has to be via outport $r$ and $P(c,.)=r$, so $A(b,w)=c$, contrary to the previous observation.\\
A symmetric situation holds if the agent wants to start a new block by LL.\\

Now we would like to estimate the number of moves needed to explore the graph by this algorithm.
Realize that after RL, LRL is performed until the next new node is found by a block LR. Symmetrically with swapped R and L.
Let say that the line has $n$ nodes. Then the adversary may put the agent in the middle of the line in such the way that, so the agent has to performs $n-2$ RL or LR blocks. After every block RL (or LR), there is one more visited node, so the number of RLR (or LRL) blocks that has to be executed before performing the next RL (or LR) block increases by $1$. The last number of consecutive LRL or RLR blocks is $n-2$ (because the last move is a single one), so the agent has to perform at least
$$
2(n-2)+1+\sum_{i=1}^{n-2}3i=\frac{(n-2)(3n+1)}{2}+1=\Omega(n^2)
$$
moves in order to explore the graph. It worths to note that it is approximately $3$ times longer than RR algorithm.
%Realize that when the agent enters a new node, then we use blocks RL and LR, which works the same as when visiting a new node in RR algorithm. When RR is used when agent enters the already visited node, then 

%The vertex' state change every step, thence after the first R, $(b,w)$ changes to $(b,w')$ and $P(b,w)=q$.\\
%After L we may either have agent's state $b$ or $b'$, but the vertex state will be $w'$ and we have to use the outport $q$.
%
%There exists an automorphism of the transition graph is that swaps $a$ and $a'$, so we may assume that the initial agent's state is $a$. Realize that for any $a_1,a_2$, there exists $v$ such that $A(a_1,v)=a_2$.  Imagine that the agent enters some node for the first time, with the agent's state $a_1$. Assume that the agent's state in the previous move was $a_2'$. The adversary wants to turn back the agent and let him go the opposite direction. However the agent's state determines the outport, so he has to change the agent's state to $a_2$. From the previous observation, we are able to do so, by choosing the appropriate vertex' state. Realize that $a_1$ determines the outport, so the appropriate port should be directed to the previous node. Hence, when the agent is entering a new node, he has to turn around, so he goes one step forward turn around and go back with the opposite orientation --- denote this sequence of moves by FB.
%Assume that otherwise (when he does not enter a new node), the agent make a sequence of moves: forward, back and forward (call it FBF).
%Assume that all the nodes are indexed with consecutive natural numbers from left to right and the starting position has the index $x$.
%We may say, that the virtual state of agent is the tuple (node index, the orientation ($L$ or $R$), leftmost visited node, rightmost visited node). Hence for $c<y<d$, $(y,L,y,d)\stackrel{FB}{\rightarrow}(y,R,y-1,d)$, $(y,R,c,y)\stackrel{FB}{\rightarrow}(y,L,c,y+1)$, $(y,R,c,d)\stackrel{FBF}{\rightarrow}(y+1,R,c,d)$ and $(y,L,c,d)\stackrel{FBF}{\rightarrow}(y-1,L,c,d)$.
%Realize that the definition of the chosen vertices' states and direction of ports approves the virtual states transitions for the move FB. We have to prove that the virtual states transitions are also true for moves of FBF type.
%POKAZAC, ze gdy uzywamy ktoregos portu po raz drugi(w danym nodzie), to musielismy byc w tym samym stanie.
%Assume that the agent moved according to FB and FBF moves to some virtual state $(y,L,c,d)$, for $c<y<d$. If $y=c+1$, then the agent has to move to the node $c$, which is visited again. Realize that, when we visit 
%After the first step, agent meets a new node with state $v'$ and with agent's state $a'$, but $P(a',v')=p'$, so he rotates and goes the step forward. Realize that the vertices' states in $x$ and $x+1$ has been already changed.\\
-------------------------------------\\


CASE 7.1.2. If $(\forall\; (a,v)\in S)\; A(a,v)=a'$, then we obtain CASE 6.1.\\
%$A(a,v)=a'$. Then $R_2(a,v)=(a',v')$.
%Case II.1. $A(a',v')=a$. Then $R_2(a',v')=(a,v)$. Realize that the actual situation is symmetric with respect to agent's state, so we are going to consider two cases:
%Case II.1.1. If $A(a,v')\neq A(a',v)$, then the transition graph is equivalent with this from the case I.2.2.
%Case II.1.2. If $A(a,v')=A(a',v)$, then the transition graph is equivalent with this from the case I.2.1.
%Case II.2. $A(a',v')=a'$, so $R_2(a',v')=(a',v)$. Then $R_2(a',v)=(a,v')$, because otherwise $a'=A(a',v)=A(a',v')$.
%Case II.2.1 If $A(a,v')=a$, then the transition graph is equivalent with this from the case I.1.
%Case II.2.2 If $A(a,v')=a'$, then the transition graph is equivalent with this from the case I.2.1.
CASE 7.2. Assume that 
\begin{equation}
\label{property}
(\forall\; p\in\Ps)(\forall\; a\in \As)(\exists\; v\in\Vs)\; P(a,v)=p~.
\end{equation}
Due to Fact \ref{wn1} we may assume that $R_3(a,v)=(a',v',p)$.\\
CASE 7.2.1. Let $A(a',v)=a'$, so because the vertex state does not determines the outport and (\ref{property}), we attain $R_3(a',v)=(a',v',p')$. Then also $R_3(a',v')=(a,v,p)$, because of (\ref{property})and CASE 4. Moreover, the agent's state is not determined by the vertex state, so again from (\ref{property}) we get $R_3(a,v')=(a',v,p')$.\\

\subparagraph{10. (7.2.3)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw[bend left] (m-1-1) edge node [above, very near start] {$p$} (m-2-2);
    \draw (m-1-2) edge node [right, near start] {$p'$} (m-2-2);
    \draw (m-2-1) edge node [left,near start] {$p'$} (m-1-2);
    \draw[bend left] (m-2-2) edge node [below, very near start] {$p$} (m-1-1);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a'$] (A) at (1,0) {$v$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v'$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    \node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      \node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  \node (Y) at (7,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (E)
	  (E) edge [above, bend left] node {$p$} (F)
	  (F) edge [above, bend left] node {$p$} (Y);
  \path (F) edge [below, bend left] node {$p'$} (E)
           (E) edge [below, bend left] node {$p'$} (D)
  	  (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\begin{tikzpicture}[->]
 \node (X) at (0,0) { };
 \node [draw, double, circle, text width=.5em, text height=0.5em, label=$a$] (A) at (1,0) {$v'$};
 \node [draw, circle, text width=.5em, text height=0.5em] (B) at (2,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (C) at (3,0) {$v$};
  \node [draw, circle, text width=.5em, text height=0.5em] (D) at (4,0) {$v'$};
    \node [draw, circle, text width=.5em, text height=0.5em] (E) at (5,0) {$v'$};
      \node [draw, circle, text width=.5em, text height=0.5em] (F) at (6,0) {$v$};
  \node (Y) at (7,0) { };
 \path (A) edge [above, bend left] node {$p'$} (B)
	  (B) edge [above, bend left] node {$p'$} (C)
	  (C) edge [above, bend left] node {$p'$} (D)
	  (D) edge [above, bend left] node {$p$} (E)
	  (E) edge [above, bend left] node {$p$} (F)
	  (F) edge [above, bend left] node {$p$} (Y);
  \path (F) edge [below, bend left] node {$p'$} (E)
           (E) edge [below, bend left] node {$p'$} (D)
  	  (D) edge [below, bend left] node {$p'$} (C)
	  (C) edge [below, bend left] node {$p$} (B)
	  (B) edge [below, bend left] node {$p$} (A)
	  (A) edge [below, bend left] node {$p$} (X);
\end{tikzpicture}
\end{minipage}
\end{center}

CASE 7.2.2. Assume that $A(a',v)=a$, so $R_3(a',v)=(a,v',p')$ from (\ref{property}).\\
CASE 7.2.2.1. Let $A(a',v')=a$. Then $R_3(a',v')=(a,v,p)$ by (\ref{property}). However, if we swap $v$ with $v'$, then we will get CASE 7.2.1.\\
CASE 7.2.2.2. Hence from (\ref{property}), $R_3(a',v')=(a',v,p)$.\\
Note that $R_3(a',v)=(a,v',p')$, so if we swap all the vertex states, agent's states and outports, then we obtain CASE 7.2. However, $A(a,v)=a'$, so we get CASE 7.2.2. But from CASE 7.2.2.1. $A(a,v')\neq a'$, so together with (ref{property}) we finally get $R_3(a,v')=(a,v,p')$.\\

\subparagraph{13. (7.2.6)}
\begin{center}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}[->]
  \matrix (m) [matrix of nodes, row sep=3em, column sep=4em, minimum width=2em, nodes={draw, align=left, text width=.5em, text height=0.5em}]
  {
    {$a$ \\ $v$}& {$a'$ \\ $v$} \\
     {$a$ \\ $v'$} & {$a'$ \\ $v'$} \\
     };
    \draw  (m-2-1) edge node [left, near start] {$p'$} (m-1-1);
    \draw (m-2-2) edge node [right, near start] {$p$} (m-1-2);
    \draw (m-1-2) edge node [right, near start] {$p'$} (m-2-1);
    \draw (m-1-1) edge node [below, near start] {$p$} (m-2-2);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
Algorithm 3 = Rotor-Router
\end{minipage}
\end{center}
 
Realize that the outport of this algorithm determines the agent's state. hence if the adversary put the outports in such a way that only one type of port directs to a node, then the agent will always have the same agent's state in this node. If the adversary do this for all the nodes, then at each node the same will be true. Thence we may think of it as the algorithm without the agent's memory. However the vertex' state change every time it is used, so it is then isomorphic with RR algorithm. Indeed, note that in this case the direction is given not only by vertices' states, but also by the fixed agents' states , which are deteremined by the outports given a priori. Hence for every node, $v$ directs to one direction and $v'$ leads to another, however for different nodes, the same type of vertex may indice different direction.

Thence we only need to show that it is possible to arrange the outports in such the way, that for every node, there is only one type of ports which indice there. However it is simple to realize, that this condition guarantees that if the outports are established  for one node, then the node, which is two places apart has to have the outports defined in opposite way, because it has to indice the opposite direction with the same outport. Moreover there is no possiblity to define the other outports using this restriciton, so me may define outports separately for the nodes which are even places apart the left end of the line and separately for the odd ones.

%If the state of vertex changes on every step and the outport is not defined only by vertex' state and for any port $p$ and any $a\in As$, there exists $v\in Vs$, such that $P(a,v)=p$ and $R_2$ is iniective function, then the algorithm can be reduced to SEA.

%Indeed, assume that $P(a,v)=p$ and $P(a',v)=q$. By the assumptions, then $P(a,v')=p'$ and $P(a',v')=q'$. Assume for a while that $R_2$ is a permutation that consists of one cycle.
%Without a loss of generality we may assume that the agent starts with agent's state $a$ in a $k$-th node, initialized with a state $v$ and that port $p$ directs to $k+1$-th node of the line. The adversary should initialize all vertices as follows:
%the node with index $k+c$ should be initialized by $v$, if $2\not| c$ and by $v'$ for $2|c$; the node with index $k-c$ should be initialize by $v$ if $2|c$ and by $v'$ for $2\not| c$.
%Moreover all the ports should be directed in such the way, that during the first visit, the agent is directed to the previous node.
%TROCHE INACZEJ TO BEDZIE
%NIE WIEM NA ILE TERAZ TO MA SENS

%%%%%%%
\begin{lem}
\label{lem:threeports}
Assume we have:
\begin{enumerate}
\item $\forall a \in \As$ $V(a,v) = v'$ and $V(a,v') = v$,
\item function $P(s) = P(s') = P(s'')$ for three different state values $s, s',s'' \in S$,
\end{enumerate}
then such an algorithm requires in the worst case $\Omega(n^2)$ steps to explore a path.
\end{lem}
\begin{proof}
Set $S$ has $4$ values so if function $P$ returns the same port for all of them then the algorithm cannot explore all paths of length $>2$. 

Assume that for some $a \in \As$, $v\in \Vs$ and $p\in \Ps$, we have $P(a,v) = p$ and $P(s) = p'$ for $s \neq (a,v)$. Let us construct a path $\mathcal{P} = (v_1,v_2,\dots, v_n)$ of length $n$ such that a port from $v_i$ to $v_{i+1}$ is always $p$ (and port from $v_{i}$ to $v_{i-1}$ is $p'$). Let $v_1$ be the starting position of the agent and let $v'$ be the initial state of each vertex and consider the exploration time of such an agent on such a path.

To prove the time complexity, we show the following: \\
\textit{Claim: For any $i \in 2,3,\dots n-1$, between first visit to $v_i$ and $v_{i+1}$, the agent visits node $v_1$. }\\
To prove the claim observe that, when entering $v_i$ for the first time, the last exit from each vertex $v_2,v_3,\dots,v_{i-1}$ was  via port $p$.  This means that the state of each of these nodes is $v'$ (it is because $V(a,v) = v'$). Since the state of $v_i,v_{i-1},\dots,v_2$ is $v'$, and the agent is at $v_i$, the agent leaves each of these vertices via port $p'$ and walks straight to node $v_1$. This completes the proof of the claim. \\

The lemma is a direct consequence of the claim, because time to explore the whole path is at least $2 \cdot \sum_{i=1}^{n-2} i \in \Omega(n^2)$.

\end{proof}

CASE 7.3. Assume that
$$
(\exists\; p\in\Ps)(\exists\; a\in \As)(\forall\; v\in \Vs)\; P(a,v)=p~.
$$
Agent's states does not determine the outports and vertex' states always change, so Lemma \ref{lem:ports} guarantees the assumptions of Lemma \ref{lem:threeports} and hence in this case, the algorithm requires $\Omega(n^2)$ steps to explore a path.
 
\input{sections/counterexamples}


%%%%%%%

\subsection{unlimited memory}
We consider a model, where $1$ agent tries to explore line topology, where every vertex has some states and number of OutPorts defined by adversary, with no identificators. InPorts and OutPorts does not need to be the same. Also the agent does not have any token that he may take through edges and leave at vertices.

We would like to find some lower bound for complexity of exploration of line graph using a deterministic algorithm. In order to do so, we assume that we are able to save any information in vertices and agent can remember everything he has seen.

For descriptive purpose, let us numerate consecutive vertices by consecutive numbers from $1$ to $n$. Assume that the agent starts the exploration at vertex $1$, so there is only one OutPort, so he can change a state of vertex $1$ to $1$ ($S(1)=1$) and simply traverse to vertex $2$.

Now assume that after some number of steps, the agent is in vertex $k$ and he is aware of all the OutPorts, which can transport him from vertex $1$ to vertex $k$ in $k-1$ consecutive steps and for all $i\leq k$, $S(i)=i$. In such the situation, we say that agent has $k$-progress. Let $OL(i)$ be the number of OutPort, which directs from vertex $i$ to vertex $i-1$, for $i=2,\ldots,n$. Let $OP(i)$ be the number of OutPort, which directs from vertex $i$ to vertex $i+1$, for $i=1,\ldots,n-1$. Realize that, if the agent knows $OL(i)$, then he knows $OP(i)$ and vice versa (if $i\neq 1$ and $i\neq n$).
If he has no $(k+1)$-progress, then he cannot guess $OL(k)$, so we may assume that at vertex $k$ he chooses a port with smaller id. If he will use $OL(k)$, then the state of the next vertex is $k-1$. If the state of the successor is another, then he knows that he went forward to vertex $k+1$ and hence after changing $S(k+1)=k+1$ he has $k+1$-progress.
Further, the agent wants to make a sequence of $\lfloor\sqrt{k}-1\rfloor$ steps using $OL(k-i)$ port at step $i$. If for $i=1,2,\ldots,j-1$, after step $i$, the agent has seen state $k-i-1$ and after step $j$, he sees the state different from $k-j-1$, then that means that, starting from vertex $k$, he has just made $j+1$ steps forward. Hence he can change $S(k+j+1)=k+j+1$ and establish $OL(i)$ for $i=k,k+1,\ldots,k+j$.
 



==> sections/path.tex <==
\section{Exploration of a path}
\subsection{One agent on a path without an oracle}
In this subsection we consider a path graph $P_{n-1}(V,E)$, where $V= \{0,1,\ldots,n-1\}$ and $E=\{(k,k+1):k\in V\backslash\{n-1\}\}$.
\mk{Uwaga: warto zaznaczyc, ze agent wie ze jest sam}
\begin{definition}
Let $x<y$. By $[x:y]$ we indicate a subpath $P_{x:y}(V_{x:y},E_{x:y})$, where $V_{x:y}=\{x,x+1,\ldots, y-1,y\}$ and $E_{x:y}=E|_{V_{x:y}^2}$.
\end{definition}
Suppose that an agent $a$ is initially in a vertex $v$ and is awared to be present in $[0:n-1]$ graph.
We search for a optimal strategy for this agent.
Realize that $0$ or $n-1$ are only two nodes of degree $1$, so we call them ends. All others vertices have degree $2$.
In order to explore the path, the agent has to visit both ends. If he is present at one of ends and graph is not explored yet, then he naturally wants to move still in one direction $n-1$ times.
Hence we may assume that agent starts at node $v$ of degree $2$.
Let $V_t$ be a subset of vertices visited by $a$ after $t$ steps, then $(t, v_t, V_t)$ is a state of progress of the agent, where $v_t$ is actual position of the agent after $t$ steps.
Realize that when $a$ chooses one side at start, he should still go in that direction until he reach one of ends of the path.
Indeed, assume that $a$ selected left at start and there exists optimal strategy $S_1(V,v)$, in which after $t$ steps, at some vertex $x\neq 0$, the agent turns right. Then $V_{t+1}=V_{t-1}\cup\{x\}$ and $v_{t+1}=x+1$. Consider a strategy $S_2(V,v)$
\mk{Nie bardzo wiadomo co to jest $S()$ w sensie formalnym } such that $S_2(V_s,v_s)=S_1(V_s,v_s)$ for $s<t-1$ and $S_2(V_s,v_s)=S_1(V_{s+2},v_{s+2})$ for $s\gs t-1$. Let the algorithm $S_1$ stops at $T$. Then $V_T=V$ and $V_{T-1}\neq V$. $S_1$ is optimal, but if $T\gs t+1$, then $V_{T-2}^2=V_T^1$, so the algorithm $S_2$ stops at $T-2$, so it is better than $S_1$, contrary to assumption.
Hence the agent either has to pass through $v+n-1$ edges or $2n-2-v$ edges.
If the agent knows where is ,,left side'', then he can decide to go left at the beginning. But then the adversary chooses $v=n-2$, so the agent has to pass $2n-3$ edges.
If he does not know the sides he may choose randomly to go left with probability $p$ and right with probability $1-p$. Then the expected value of passes is $(n-1)(2-p)+v(2p-1)$.
If $p=\frac{1}{2}$, then the expectation does not depend on a choice of $v$ and it is equal to $1.5(n-1)$. If $p<\frac{1}{2}$ then a choice $v=1$ gives bigger expectation. Symmetrically, if $p>\frac{1}{2}$, then the adversary's choice should be $v=n-2$.
Hence a knowledge of the sides of a path does not give any desired information.
\mk{Zasadniczo w przypadku 1 agenta energia = czas . A tu musi byc klasyczny wynik i chyba warto zacytowac ... }
\subsection{One agent on a path with an oracle}
Now, consider the path graph $P_{n-1}$ and a problem of one agent with an initiative oracle, that gives the information about the number of starting point vertex $v$ of the agent.
Then the agent know whether if he is closer to $0$ or to $n-1$, so he may start to go to the closer end. Then we makes $\min\{n-1+v,2n-2-v\}$ moves. However, if $2\not{|}n$, then the adversary can choose $v=\frac{n-1}{2}$ and the expectation remains $1.5(n-1)$. When $2|n$, then the expectation is $1.5(n-1)-0.5$ 
Hence such an oracle does not bear any useful information.

\subsection{Two agents on a path without an oracle}
\mk{Tu niejawnie zakładamy symetrie (agenty wykonuja ten sam kod) i determinizm }
Consider the path $P_{n-1}$ with two agents $a_1$ and $a_2$, starting in $v_1$ and $v_2$ respectively. %Every agent has to go in the direction he chosed at the start until he reach a point with a sign of the other agent or until he reach the end of a path.
\db{dlaczego nie oplaca sie zawracac przed spotkaniem czyjegos sladu ani przed koncem sciezki? Chyba niekoniecznie tak jest.}
\mk{Chyba tak jest, ale katycznie to musi byc jakos uzasadnione. }
Realize that, if $v_1=v_2=0$, then both agents want to go right until one of them reach $n-1$.
If in any moment any agent want to stop, then the other one is idle due to the adversary. So they will have to go both to $n-1$. Hence the needed energy is $2n-2$. Symetrically, if $v_1=v_2=n-1$, the energy is $2n-2$. If $0<v_1=v_2<n-1$, then one decide to go left until he will reach the end. Then go right. Symetrically the other one start with going right, then revert at the end.
Also there is a case, when They meet once again, but one of them still didn't reach the end of a path. Then they have to reach this end together due to sabotage work of adversary. In this case they have to go through $v_1+(n-1-v_2)+x+(n-1-x)=2n-2$ edges, where $x$ is the end point of theirs voyage.
Although the sum of energy is bigger than for one agent, the average cost is $n-1$, which $\frac{2}{3}$ of the cost for 1 agent.

Consider a situation, when $v_1=0$ and $v_2<n-1$ and $a-2$ decides to go right at start.\db{tutaj dobry opis, zeby wykorzystywac ten schemat poxniej. moze nawet zrobic ogolniej, dla $x\neq v_1$}

Now we assume that agents starts in different vertices, know the sides of the path and use deterministic strategy:
\begin{enumerate}
\item choose direction (somehow).
\item go still this direction.
\item if you reach the end of path, turn aroung and go the opposite direction.
\item if you meet a sign of the other agent (or the agent itself) turn around and go that direction.
\item repeat until the end of procedure.
\end{enumerate}\db{pewnie trzeba pokazac, ze taka procedura sie zakonczy}
Case 1. Imagine that both agents chooses the same direction and $v_1<v_2$. For exapmle, the left one.
There are some number of scenarios.\\
Scenario 1. $a_1$ reaches $0$ before $a_2$ reaches $v_1$.\\
Scenario 1.1. $a_1$ reaches $v_1$ once again until $a_2$ reaches $v_1$.\\
Scenario 1.2 $a_2$ reaches $v_1$ before $a_1$ reaches it again.\\
Scenario 2. $a_1$ reaches $0$ at the same time as $a_2$ reaches $v_1$.\\
Scenario 3. $a_2$ reaches $v_1$ before $a_1$ reaches $0$.\\
Scenario 3.1. $a_2$ reaches $n-1$ before $a_1$ reaches $0$.\\
Scenario 3.2. $a_1$ reaches $0$ before $a_2$ reaches $n-1$. \\
1.1. $a_1$ meets $a_2$ at $x$, where $v_1\leq x\leq v_2$ and they go together to $n-1$.
Energy: $2v_1+(x-v_1)+(v_2-x)+2(n-1-x)=2(n-1)+(v_2+v_1)-2x$, which is the biggest when $x=v_1$, so the maximal energy is $2(n-1)+(v_2-v_1)$.\\
1.2. Both agents are going right until one of them reach $n-1$. Assume that the second one ends in $x$. Hence the energy is:
$v_1+(v_2-v_1)+\max\{n-1+(x-v_1),(n-1-v_1)+x\}=n-1+x+v_2-v_1$, which is the biggest when $x=n-1$, so the maximal energy is $2(n-1)+(v_2-v_1)$.\\
2. The same situation as 1.2.\\
3.2. The same situation as 1.2.\\
3.1. Symetrical scenario to 3.1. Energy is $(v_2-v_1)+(n-1-v_1)+\max\{(n-1-x)+v_1,n-1+(v_1-x)\}=2(n-1)+(v_2-v_1)-x$, which is the biggest when $x=0$.
In all the cases we have the maximal energy of $2(n-1)+(v_2-v_1)$.
The worst case is when $v-1=0$ and $v_2=n-2$, which leads to $3n-4$.\\
Case 2. Symmetricaly, when both agents starts to right, then the maxiamal energy is still $2(n-1)+(v_2-v_1)$ and the worst case of $v_1=1$ and $v_2=n-1$ gives energy of $3n-4$.\\ \db{ten case mozna usunac}
Case 3. If $a_1$ chooses right and $a_2$ chooses left. Then they meet at some $x$ between $v_1$ and $v_2$. After that at least one of them reaches one of the ends of the path. Then the situation is reduced to an old problem. Again we obtain $2(n-1)+(v_2-v_1)$ and $3n-4$.\\
Case 4. $a_1$ chooses left and $a_2$ chooses right.
Then at least one of them reaches the end of the path and we reduced the problemt to old one.
Due to symmetry, assume that the agent $a_1$ was not first at one of the ends. Hence the energy is $(n-1-v_2)+\max\{(v_1-x)+n-1,(n-1-x)+v_1\}=2(n-1)+(v_1-v_2)-x$, which is the biggest when $x=0$, hence the energy is $2(n-1)+(v_1-v_2)$ this time, what gives the maximum for $|v_2-v_1|=2$, so it gives the energy of $2(n-1)-2$.

\paragraph{Remark} If both agents choose the same direction, then the energy needed is $3n-4$.
If one agent chooses left iff the second chooses right, the answer is still $3n-4$.
If the agents know whether the second agent is on the left or right, they can choose the opposite and reach $2n-4$.
If the agents chooses direction unifromly at random, then the solution is $2(n-1)+\frac{1}{2}(v_2-v_1)$, which leads to $2.5n-3$ in the worst case.\db{upewnic sie co do stalej}
If the agents chooses direction from a distribution $\mathrm{Bin}(p)$, then the maximal energy is $2(n-1)+(v_2-v_1)(1-2p(1-p))$ and the optimal one is for $p=\frac{1}{2}$.
If agents chooses the opposite values of probability ($p$ and $r$), then either $1-2p(1-r)$ or $1-2(1-p)r$ is not lower than $\frac{1}{2}$, because either $1-2p(1-r)>1-2p(1-p)$ or $1-2r(1-p)>1-2r(1-r)$.
If we want to optimize the energy for any randomized strategy of this type, we have to find the $\min\{\max\{(v_2-v_1)(1-2p(v_1)(1-p(v_2))):v_1<v_2\}:p:V\rightarrow[0,1]\}$.
In particular, the adversary has to choose $v_2$ and $v_1$ in such a way, that $|v_2-v_1|>\frac{n-1}{2}$, because otherwise the energy would be lower than $2.5n-3$.
So if, an oracle reveals the starting position of the particular agent, then he has to choose the direction that leads to the closer end of a path to obtain the energy of $2(n-1)-|v_1-v_2|$ and the maximum of $2n-4$.

==> sections/token.tex <==
\subsection{Token model with DirtyMem on the line graph}
The agent has a unique token, which can be DROPped, TAKEn and MOVEd through ports of a graph.
Moreover, assume that the agent has constant memory which consist of a State from the set $\{HasToken, SeeToken, None, Terminated\}$, a Progress from the set $\{0,1\}$ and an index ID consisting of $C\geqslant 2$ bits (with values from $1$ to $2^C$).
Each node has one bit of memory, which directs to one of its ports, initially set by the adversary.
If the agent is in the state HasToken, then he can DROP it or MOVE with it. 
If he has the state SeeToken, then he can TAKE it or MOVE without it.
If the agent changes the value of memory at some node, then we write that agent make a SWAP.
The agent starts the algorithm in the $State=HasToken$, with $ID=1$ and $Progress=0$.
The agent can additionally check whether is he at the end of the line. An event End is true if and only if the agent is at one of two ends of the line graph.

Consider the beneath algorithm:
\begin{algorithm}
	\begin{algorithmic}[1]
		\caption{Token alg}
		\IF{$End$}
			\IF{$Progress=1$}
				\STATE{$State\leftarrow Terminated$;}
			\ELSIF{$State=HasToken$;}
				\STATE{$Progress\leftarrow 1$; $MOVE$; $ID\leftarrow 1$;}
			\ENDIF
		\ENDIF
		\IF{$State=HasToken$}
			\STATE{$SWAP$;}
			\IF{$ID=1$}
				\STATE{$DROP$;}
			\ELSE
				\STATE{$ID--$;}
			\ENDIF
		\ELSIF{$State=SeeToken$}
			\STATE{$TAKE$;}
			\IF{$ID=2$}
				\STATE{$ID--$;}
			\ELSE
				\STATE{$ID\leftarrow \lfloor\frac{ID+1}{2}\rfloor$;}
			\ENDIF
		\ELSIF{$State=None$}
			\IF{$ID=1$}
				\STATE{$ID++$;}
			\ELSE
				\STATE{$ID\leftarrow \min\{ID+1,2^C\}$;}
			\ENDIF
		\ENDIF
		\IF{$State\neq Terminated$}
			\STATE{$MOVE$;}
		\ENDIF
	\end{algorithmic}
\end{algorithm}


